A Comparative Study of Long and Short GRBs. I. Overlapping Properties

Gamma ray bursts (GRBs) are classified into long and short categories based on their durations. Broad band studies suggest that these two categories of objects roughly correspond to two different classes of progenitor systems, i.e. compact star mergers (Type I) vs. massive star core collapse (Type II). However, the duration criterion sometimes leads to mis-identification of the progenitor systems. We perform a comprehensive multi-wavelength comparative study between duration-defined long GRBs and short GRBs as well as the so-called "consensus" long GRBs and short GRBs (which are believed to be more closely related to the two types of progenitor systems). The parameters we study include two parts: the prompt emission properties including duration ($T_{90}$), spectral peak energy ($E_{\rm p}$), low energy photon index ($\alpha$), isotropic $\gamma$-ray energy ($E_{\rm \gamma, iso}$), isotropic peak luminosity ($L_{\rm p,iso}$), and the amplitude parameters ($f$ and $f_{\rm eff}$); and the host galaxy properties including stellar mass ($M_*$), star formation rate (SFR), metallicity ([X/H]), half light radius ($R_{50}$), angular and physical ($R_{\rm off}$) offset of the afterglow from the center of the host galaxy, the normalized offset ($r_{\rm off}=R_{\rm off}/R_{50}$), and the brightness fraction $F_{\rm light}$. For most parameters, we find interesting overlapping properties between the two populations in both 1D and 2D distribution plots. The three best parameters for the classification purpose are $T_{90}$, $f_{\rm eff}$, and $F_{\rm light}$. However, no single parameter alone is good enough to place a particular burst into the right physical category, suggesting a need of multiple criteria for physical classification.

==> basic.tex <==
\begin{deluxetable}{llllcllllrr}
\tabletypesize{\scriptsize}
%%\tabcolsep0.1in\footnotesize
\tablecolumns{10}
\tablewidth{0pc}
\tablecaption{prompt \label{table:basic}}
\tablehead {
\colhead{GRB}        &
\colhead{T90(s)} &
\colhead{RA} &
\colhead{Dec}       &
\colhead{uncertainty (")} &
\colhead{Method}      &
\colhead{z} &
\colhead{Method}      &
\colhead{reference}      &\\
}

\startdata

140606B & 23.6 & 21:51:00 & +33:41 & 10800 & ... & $0.384$ & E & 339,349,353 \\
140518A & 60.5 & 15:09:00.60 & 42:25:05.6 & 1.5 & XRT & $4.707$ & A & 337,351,352 \\
140515A & 23.4 & 12:24:15.45 & 15:06:17.0 & 1.5 & XRT & $6.32$ & A & 336,351,352 \\
140512A & 154.8 & 19:17:28.78 & -15:05:39.2 & 0.61 & UVOT & $0.725$ & A & 338,351,352 \\
140509A & 23.20 & 03:06:22.69 & -62:38:21.7 & 0.42 & UVOT & $2.4$ & P & 335,351 \\
140508A & 44.3 & 17:02:31 & +46:45 & 5400 & ... & $1.027$ & A & 333,334,353 \\
140506A & 111.1 & 18:27:06.04 & -55:38:08.7 & 0.43 & UVOT & $0.8893$ & E & 342,351 \\
140430A & 173.6 & 06:51:44.61 & 23:01:25.2 & 0.62 & UVOT & $1.6019$ & E & 342,351 \\
140428A & 17.42 & 12:57:28.45 & 28:23:05.7 & 1.7 & XRT & $4.7$ & A & 332,351,352 \\
140423A & 134 & 13:09:08.54 & 49:50:29.4 & 0.48 & UVOT & $3.26$ & A & 331,351,352 \\
140419A & 94.7 & 08:27:57.56 & 46:14:25.3 & 0.5 & UVOT & $3.956$ & A & 330,351,352 \\
140318A & 8.43 & 12:16:21.42 & 20:12:32.9 & 1.6 & XRT & $1.02$ & E & 345,351,352 \\
140311A & 71.4 & 13:57:13.25 & 00:38:30.8 & 1.5 & XRT & $4.954$ & A & 329,351,352 \\
140304A & 15.6 & 02:02:34.26 & 33:28:25.7 & 1.6 & XRT & $5.283$ & A & 328,351,352 \\
140301A & 31.0 & 04:38:13.81 & -34:15:24.3 & 1.6 & XRT & $1.4155$ & E & 342,351 \\
140226A & ... & 14:45:58 & +15:00 & 0 & ... & $1.98$ & A & 343,353 \\
140213A & 60.0 & 07:00:37.13 & -73:08:13.5 & 0.51 & UVOT & $1.2079$ & E & 342,351 \\
140206A & 93.6 & 09:41:20.26 & 66:45:38.6 & 0.5 & UVOT & $2.739$ & A & 327,351 \\
140114A & 139.7 & 12:34:05.16 & 27:57:02.6 & 1.4 & XRT & $3\pm0.1$ & A & 342,351 \\
131231A & 31 & 5:40:57 & -04:26 & 540 & ... & $0.642$ & E & 325,326,353 \\
131227A & 18.0 & 04:29:30.78 & 28:52:58.9 & 1.4 & XRT & $5.3$ & A & 318,351,352 \\
131117A & 11.00 & 22:09:19.36 & -31:45:44.3 & 0.64 & UVOT & $4.042$ & A & 316,351,352 \\
131108A & 19 & 10:25:53 & +09:54 & 1800 & ... & $2.4$ & A & 314,315,353 \\
131105A & 112.3 & 04:43:52.18 & -62:59:42.7 & 1.4 & XRT & $1.6854$ & E & 342,351 \\
131103A & 17.3 & 23:15:40.55 & -44:38:25.4 & 0.6 & UVOT & $0.596$ & E & 342,351 \\
131030A & 41.1 & 23:00:16.14 & -05:22:05.2 & 0.5 & UVOT & $1.293$ & A & 313,351,352 \\
131011A & 77 & 1:27:41 & +09:33 & 18900 & ... & $1.874$ & A & 311,312,353 \\
131004A & 1.54 & 19:44:27.09 & -02:57:30.4 & 0.55 & UVOT & $0.717$ & E & 310,351,352 \\
130925A & 7000 & 02:44:42.97 & -26:09:11.5 & 1.4 & XRT & $0.3483$ & E & 319,342,351 \\
130907A & 360 & 14:23:34.04 & 45:36:27.1 & 0.5 & UVOT & $1.238$ & A & 309,351,352 \\
130831A & 32.5 & 23:54:29.89 & 29:25:46.2 & 0.74 & UVOT & $0.4791$ & A & 308,351,352 \\
130702A & 59 & 1:09:54 & +00:00 & 24720 & ... & $0.145$ & E & 289,307,353 \\
130701A & 4.38 & 23:48:55.08 & 36:06:01.5 & 1.5 & XRT & $1.1548$ & E & 342,351 \\
130612A & 4.0 & 17:19:10.58 & 16:43:11.9 & 0.53 & UVOT & $2.006$ & A & 306,351,352 \\
130610A & 46.4 & 14:57:40.88 & 28:12:25.8 & 0.51 & UVOT & $2.092$ & A & 305,351,352 \\
130606A & 276.58 & 16:37:35.13 & 29:47:46.8 & 1.4 & XRT & $5.913$ & A & 288,351 \\
130604A & 37.7 & 16:40:44.89 & 68:13:34.9 & 1.6 & XRT & $1.06$ & E & 304,351,352 \\
130528A & 0.18 & 09:18:01.22 & 87:18:04.2 & 1.9 & XRT & $1.25\pm0.001$ & E & 320,351 \\
130518A & 59.4 & 23:43:14 & +47:38 & 1200 & ... & $2.49$ & A & 301,302,352,353 \\
130514A & 48 & 19:45:07.92 & -07:58:34.0 & 1.5 & XRT & $3.6$ & P & 300,351,352 \\
130511A & 204 & 13:06:34.96 & 18:42:36.0 & 0.64 & UVOT & $1.3033$ & A & 299,351,352 \\
130505A & 5.43 & 09:08:14.64 & 17:29:05.2 & 0.5 & UVOT & $2.27$ & A & 298,351,352 \\
130427B & 88 & 20:59:35.64 & -22:32:46.5 & 1.1 & UVOT & $2.78\pm0.02$ & A & 297,351,352 \\
130427A & 27.0 & 11:32:33 & +27:41 & 180 & ... & $0.3399\pm0.0002$ & E & 290,351,353 \\
130420A & 162.83 & 13:04:25.55 & 59:25:27.1 & 0.5 & UVOT & $1.297$ & A & 296,351,352 \\
130418A & 123.5 & 09:56:08.88 & 13:40:02.7 & 0.5 & UVOT & $1.217$ & A & 295,351,352 \\
130408A & 300 & 08:57:37.30 & -32:21:38.9 & 0.5 & UVOT & $3.757$ & A & 294,351,352 \\
130215A & 28 & 2:53:55 & +13:22 & 180 & ... & $0.597$ & A & 292,351,352,353 \\
130131B & 65.7 & 11:35:49.36 & 15:02:17.5 & 1.6 & XRT & $2.539$ & E & 293,351 \\
121229A & 4.30 & 12:40:24.31 & -50:35:38.6 & 1.7 & XRT & $2.707$ & A & 280,281,351,352 \\
121212A & 100 & 11:51:10.30 & 78:02:14.3 & 0.62 & UVOT & $...$ & ... & 351 \\
121211A & 6.8 & 13:02:07.99 & 30:08:54.6 & 0.52 & UVOT & $1.023$ & A & 279,351 \\
121209A & 182 & 21:47:08.93 & -08:14:07.1 & 1.4 & XRT & $2.1\pm0.3$ & A & 342,351 \\
121201A & 42.7 & 00:53:52.16 & -42:56:34.5 & 0.62 & UVOT & $3.383$ & E & 342,351 \\
121128A & 85 & 20:02:24.00 & 54:17:59.1 & 0.5 & UVOT & $2.2$ & A & 278,351,352 \\
121027A & 23.3 & 04:14:23.47 & -58:49:46.8 & 1.4 & XRT & $1.7732$ & E & 342,351 \\
121024A & 62.6 & 04:41:53.28 & -12:17:26.8 & 0.78 & UVOT & $2.3012$ & E & 342,351 \\
120922A & 69 & 15:38:59.60 & -20:10:54.3 & 0.65 & UVOT & $3.1$ & P & 277,351,352 \\
120909A & 173 & 18:22:56.77 & -59:26:55.0 & 1.4 & XRT & $3.93$ & A & 1,276,351,352 \\
120907A & 112 & 04:59:00.00 & -09:18:54.0 & 0.52 & UVOT & $0.97$ & A & 275,351,352 \\
120815A & 16.9 & 18:15:49.88 & -52:07:52.1 & 0.6 & UVOT & $2.3587$ & E & 342,351 \\
120811C & 9.7 & 13:18:43.82 & 62:18:02.8 & 0.52 & UVOT & $2.671$ & A & 274,351,352 \\
120805A & 26.8 & 14:26:08 & +05:48 & 180 & ... & $3.1\pm0.1$ & A & 342,351,353 \\
120802A & 48.00 & 02:59:22.22 & 13:46:06.0 & 1.4 & XRT & $3.796$ & A & 273,351,352 \\
120729A & 50 & 00:52:17.83 & 49:56:23.1 & 0.5 & UVOT & $0.8$ & A & 272,351,352 \\
120724A & 71.5 & 16:20:43.35 & 03:30:27.8 & 0.77 & UVOT & $1.48$ & A & 271,351,352 \\
120722A & 72.8 & 15:21:59.18 & 13:15:03.8 & 1.7 & XRT & $0.959$ & E & 342,351 \\
120716A & 42.4 & 20:52:21 & +09:33 & 7260 & ... & $2.486$ & A & 269,270,353 \\
120714B & 234 & 23:41:38.1 & -46:11:02 & 0.58 & UVOT & $0.3985$ & E & 342,351 \\
120712A & 159 & 11:18:21.25 & -20:02:01.7 & 0.5 & UVOT & $4.1745$ & A & 268,351,352 \\
120711A & 14.7 & 6:18:49 & -71:01 & 180 & ... & $1.405$ & A & 267,324,353 \\
120624B & 44.033 & 11:23:46 & +08:56 & 180 & ... & $2.1974\pm0.0002$ & E & 285,351,353 \\
120521C & 192 & 14:17:08.73 & 42:08:41.0 & 1.6 & XRT & $6$ & P & 322,351 \\
120422A & 26.7 & 09:07:38.4 & 14:01:07.6 & 1 & UVOT & $0.2826$ & E & 342,351 \\
120404A & 5.35 & 15:40:02.29 & 12:53:06.3 & 0.65 & UVOT & $2.876$ & A & 266,351,352 \\
120327A & 38.7 & 16:27:27.48 & -29:24:53.74 & 0.48 & UVOT & $2.813$ & A & 265,351,352 \\
120326A & 62.9 & 18:15:37.13 & 69:15:35.36 & 0.5 & UVOT & $1.798$ & A & 264,351,352 \\
120311A & 69.6 & 18:12:22.11 & 14:17:46.4 & 1.5 & XRT & $<3$ & P & 263,351 \\
120308A & 3.5 & 14:36:20.05 & +79:41:12.2 & 0.55 & U & $<4.5$ & P & 350,351,356 \\
120224A & 60.6 & 02:43:46.13 & -17:45:40.6 & 1.4 & XRT & $1.1\pm0.2$ & A & 342,351 \\
120211A & 8.13 & 05:51:00.91 & -24:46:31.2 & 1.6 & XRT & $2.4\pm0.1$ & A & 342,351 \\
120119A & 61.7 & 08:00:06.94 & -09:04:53.8 & 0.3 & O & $1.7291$ & E & 340,342,350,351 \\
120118B & 253.8 & 08:19:29.04 & -07:11:05.1 & 1.4 & XRT & $2.9428$ & E & 342,351 \\
111229A & 23.26 & 05:05:08.86 & -84:42:39.1 & 0.55 & UVOT & $1.3805$ & A & 256,351,352 \\
111228A & 25.4 & 10:00:16.01 & 18:17:51.8 & 0.75 & UVOT & $0.7164$ & E & 342,351 \\
111225A & 101.20 & 00:52:37.22 & 51:34:19.5 & 0.67 & UVOT & $2.012$ & E & 347,351 \\
111215A & 106.8 & 23:18:13.32 & 32:29:38.4 & 1.4 & XRT & $...$ & ... & 351 \\
111211A & 796 & 10:12:22 & +11:11 & 180 & ... & $0.478$ & A & 254,255,353 \\
111209A & 25 & 00:57:22.63 & -46:48:03.8 & 0.5 & UVOT & $0.677$ & E & 286,323,351 \\
111129A & 25000 & 20:29:44.15 & -52:42:46.5 & 0.54 & UVOT & $1.0796$ & E & 342,351 \\
111123A & 7.6 & 10:19:23.13 & -20:38:41.0 & 1.4 & XRT & $3.1513$ & E & 342,351 \\
111107A & 290.0 & 08:37:54.66 & -66:31:12.3 & 0.65 & UVOT & $2.893$ & A & 253,351,352 \\
111008A & 26.6 & 04:01:48.23 & -32:42:33.5 & 1.4 & XRT & $4.9898$ & A & 252,351,352 \\
111005A & 63.46 & 14:53:08 & -19:44 & 180 & ... & $...$ & ... & 351,353 \\
110918A & 26 & 2:10:18 & -27:17 & 180 & ... & $0.982$ & E & 284,353 \\
110818A & ... & 21:09:20.87 & -63:58:51.7 & 1.4 & XRT & $3.3609$ & E & 342,351 \\
110808A & 103 & 03:49:04.27 & -44:11:40.1 & 0.64 & UVOT & $1.349$ & E & 342,351 \\
110801A & 48 & 05:57:44.87 & 80:57:21.1 & 0.51 & UVOT & $1.858$ & A & 251,351,352 \\
110731A & 385 & 18:42:00.99 & -28:32:13.8 & 0.2 & UVOT & $2.83$ & A & 250,351,352 \\
110726A & 38.8 & 19:06:52.08 & 56:04:16.5 & 0.51 & UVOT & $1.036$ & A & 249,351,352 \\
110715A & 5.2 & 15:50:44.09 & -46:14:06.53 & 0.56 & UVOT & $0.82$ & A & 247,351,352 \\
110709B & 13.0 & 10:58:37.11 & -23:27:16.7 & 0.7 & R & $2.09$ & E & 248,350,351 \\
110503A & 55.6 & 08:51:06.21 & 52:12:27.6 & 0.5 & UVOT & $1.613$ & A & 246,351,352 \\
110422A & 10.0 & 07:28:11.33 & 75:06:24.4 & 1.4 & XRT & $1.77$ & A & 245,351,352 \\
110213B & 25.9 & 02:47:01.51 & 01:08:43.8 & 2.4 & XRT & $1.083$ & A & 243,244,351 \\
110213A & 50 & 02:51:51.39 & 49:16:23.54 & 0.5 & UVOT & $1.46$ & A & 242,351,352 \\
110205A & 48.0 & 10:58:31.10 & +67:31:30.5 & 0.3 & O & $2.22$ & A & 240,241,350,351 \\
110128A & 257 & 12:55:35.10 & 28:03:54.1 & 1.3 & UVOT & $2.339$ & A & 239,351,352 \\
110106B & 30.7 & 08:56:37.08 & 47:00:09.4 & 1.4 & XRT & $0.618$ & E & 238,351 \\
101225A & 24.8 & 00:00:47.51 & 44:36:01.1 & 1.4 & XRT & $0.847$ & E & 323,351 \\
101219B & 1088.0 & 00:48:55.35 & -34:33:59.5 & 0.62 & UVOT & $0.55185$ & A & 234,351 \\
100906A & 0.2 & 01:54:44.11 & 55:37:49.6 & 0.61 & UVOT & $1.727$ & A & 225,351,352 \\
100901A & 34 & 01:49:03.42 & 22:45:30.8 & 0.81 & UVOT & $1.408$ & A & 224,351,352 \\
100814A & 0.6 & 01:29:53.59 & -17:59:43.5 & 0.4 & O & $1.4392$ & E & 342,350,351 \\
100802A & 114.4 & 00:09:52.38 & +47:45:18.8 & 0.5 & O & $<3.5$ & E & 175,350,351 \\
100728B & 439 & 02:56:13.46 & +00:16:52.1 & 0.52 & U & $2.106$ & A & 226,350,351,356 \\
100728A & 2.9 & 05:55:01.99 & -15:15:19.6 & 1.4 & XRT & $1.567$ & E & 342,351 \\
100724A & 174.5 & 12:58:10.37 & -11:06:09.4 & 1.5 & XRT & $1.289$ & E & 342,351 \\
100621A & 487 & 21:01:13.08 & -51:06:22.2 & 0.3 & I & $0.5426$ & E & 231,342,351 \\
100615A & 12.1 & 11:48:49.34 & -19:28:52.0 & 0.7 & X & $1.3978$ & E & 223,342,350,351 \\
100606A & 198.5 & 23:22:30.38 & -66:14:28.8 & 1.4 & XRT & $1.5545$ & E & 342,351 \\
100518A & 1.4 & 20:19:13 & -24:32 & 180 & ... & $4^{+0.3}_{-0.5}$ & P & 222,353 \\
100513A & 0.33 & 11:18:26.85 & 03:37:40.5 & 1.4 & XRT & $4.772$ & A & 221,351,352 \\
100508A & 63.6 & 05:04:58.99 & -20:42:41.1 & 0.6 & UVOT & $0.5201$ & E & 342,351 \\
100425A & 39 & 19:56:47.16 & -26:25:50.9 & 1.5 & XRT & $1.755$ & A & 220,351,352 \\
100424A & 480 & 13:57:47.48 & 01:32:18.6 & 1.7 & XRT & $2.4656$ & E & 342,351 \\
100418A & ... & 17:05:26.96 & 11:27:41.9 & 0.67 & UVOT & $0.6235$ & E & 342,351 \\
100414A & 84 & 12:14:28 & +20:27 & 660 & ... & $1.368$ & A & 219,324,353 \\
100316D & 52 & 7:10:28 & -56:09 & 180 & ... & $0.0591\pm0.0001$ & E & 218,257,353 \\
100316B & 37.0 & 10:53:57.141 & -45:28:21.54 & 0.52 & UVOT & $1.18$ & A & 217,351,352 \\
100302A & 104 & 13:02:03.87 & 74:35:24.5 & 1.5 & XRT & $4.813$ & A & 216,351,352 \\
100219A & 7.0 & 10:16:48.54 & -12:33:57.9 & 1 & UVOT & $4.6667$ & A & 215,351,352 \\
091208B & 26.497 & 01:57:34.10 & +16:53:22.6 & 0.25 & O & $1.0633$ & A & 179,236,350 \\
091127A & 1300 & 02:26:19.89 & -18:57:08.5 & 0.55 & U & $0.4904$ & E & 236,342,350,356 \\
091109A & 3.8 & 20:37:01.82 & -44:09:29.6 & 0.4 & O & $3.076$ & A & 214,236,350 \\
091029A & 17.9 & 04:00:42.62 & -55:57:20.0 & 0.5 & O & $2.752$ & A & 178,236,350 \\
091024A & 18.8 & 22:36:50 & +56:52 & 180 & ... & $1.092$ & A & 177,236,353,357 \\
091020A & 0.12 & 11:42:55.20 & 50:58:42.0 & 0.5 & UVOT & $1.71$ & A & 176,236,351,357 \\
091018A & 0.3 & 02:08:44.63 & -57:32:53.8 & 0.5 & O & $0.971$ & E & 236,342,350 \\
091003A & 14.80 & 16:46:05 & +36:38 & 780 & ... & $0.8969$ & E & 174,324,353 \\
090927A & 7.42 & 22:55:53.41 & -70:58:49.3 & 0.63 & UVOT & $1.37$ & A & 206,236,351 \\
090926B & 0.27 & 03:05:13.91 & -39:00:22.6 & 0.3 & X & $1.2427$ & E & 231,236,342 \\
090926A & 48.03 & 33:36.0 & -66:19:26.6 & 0.2 & ... & $2.1062$ & E & 212,324 \\
090902B & 39.18 & 39:45.4 & +27:19:27.1 & 0.5 & ... & $1.822$ & A & 204,205,324 \\
090814A & 112.28 & 15:58:26.39 & +25:37:52.4 & 0.4 & O & $0.696$ & A & 203,236,350 \\
090812A & 38.92 & 23:32:48.56 & -10:36:17.2 & 0.4 & O & $2.452$ & A & 201,202,236,350 \\
090809A & 4.37 & 21:54:43.19 & -00:05:01.83 & 0.6 & UVOT & $2.737$ & A & 200,236,351,357 \\
090726A & 20.224 & 16:34:43.29 & 72:53:03.1 & 1.5 & XRT & $2.71$ & A & 199,236,351,357 \\
090715B & 2.16 & 16:45:21.63 & +44:50:21.0 & 0.4 & O & $3$ & A & 198,236,350 \\
090709A & 99.28 & 19:19:42.64 & +60:43:39.3 & 0.5 & I & $0.403^{+0.5}_{-0.7}$ & E & 197,213,236,350 \\
090618A & 13.760 & 19:35:58.73 & +78:21:24.3 & 0.5 & O & $0.54$ & A & 196,236,350 \\
090530A & 19.328 & 11:57:40.49 & +26:35:37.7 & 0.4 & O & $1.266$ & A & 236,317,350 \\
090529A & 78.22 & 14:09:52.56 & 24:27:32.2 & 0.7 & UVOT & $2.625$ & A & 195,236,351,357 \\
090519A & 75.09 & 09:29:07.00 & +00:10:48.9 & 0.6 & O & $3.85$ & A & 193,194,236,350 \\
090516A & 7.84 & 09:13:02.60 & -11:51:15.0 & 0.4 & O & $4.109$ & A & 192,236,350 \\
090429B & 56.68 & 14:02:40.11 & 32:10:13.9 & 1.5 & XRT & $9.2$ & P & 235,236,351 \\
090424A & 265.39 & 12:38:05.08 & +16:50:15.0 & 0.6 & O & $0.544$ & E & 189,236,350 \\
090423A & 88.73 & 09:55:33.26 & 18:08:57.9 & 1.4 & XRT & $8.23$ & A & 209,236,351,357 \\
090418A & 113.34 & 17:57:15.16 & +33:24:20.9 & 0.4 & O & $1.608$ & A & 186,188,236,350 \\
090417B & 40.46 & 13:58:46.58 & +47:01:04.8 & 1 & X & $0.345$ & E & 106,187,236,350 \\
090407A & 70 & 04:35:55.07 & -12:40:45.1 & 1.4 & XRT & $1.4485\pm0.0006$ & E & 236,261,351 \\
090328A & 58.26 & 02:39.7 & -41:52:53.8 & 0.25 & ... & $0.7357\pm0.0004$ & E & 185,233,324 \\
090323A & 208.00 & 42:50.3 & +17:03:11.90 & 0.05 & ... & $3.568\pm0.004$ & A & 184,233,324 \\
090313A & 0.04 & 13:13:36.20 & +08:05:49.6 & 0.7 & O & $3.375$ & A & 182,183,236,350 \\
090205A & 5.66 & 14:43:38.61 & -27:51:10.4 & 1.4 & XRT & $4.6497$ & A & 181,236,351,357 \\
090201A & 5.61 & 06:08:12.52 & -46:35:25.0 & 1.4 & XRT & $2.1$ & E & 236,342,351 \\
090113A & 1.24 & 02:08:13.80 & 33:25:42.3 & 1.5 & XRT & $1.7493\pm0.0002$ & E & 236,261,351 \\
090102A & 49.47 & 08:32:58.54 & 33:06:51.2 & 1.1 & UVOT & $1.547$ & A & 180,236,351,357 \\
081230A & 9.77 & 02:29:19.467 & -25:08:51.0 & 0.9 & UVOT & $2.03^{+0.16}_{-0.14}$ & P & 229,236,351 \\
081228A & 56.31 & 2:37:52 & +30:51 & 180 & ... & $3.44^{+0.15}_{-0.32}$ & P & 229,236,353 \\
081222A & 282.49 & 01:30:57.59 & -34:05:41.49 & 0.5 & UVOT & $2.77$ & A & 161,236,350,351 \\
081221A & 315.44 & 01:03:10.16 & -24:32:51.6 & 0.25 & I & $2.259$ & E & 236,342,350 \\
081210A & 61.697 & 04:41:56.20 & -11:15:26.8 & 0.64 & U & $2.0631$ & E & 236,342,350,356 \\
081203A & 135.170 & 15:32:07.58 & 63:31:14.9 & 0.5 & UVOT & $2.05\pm0.01$ & A & 208,236,351,357 \\
081128A & 70.66 & 01:23:13.10 & +38:07:38.7 & 0.2 & O & $<4$ & P & 236,350 \\
081121A & 0.35 & 05:57:06.15 & -60:36:10.0 & 0.6 & UVOT & $2.512$ & A & 160,236,350,351 \\
081118A & 8.80 & 05:30:22.18 & -43:18:05.1 & 0.6 & O & $2.58$ & A & 158,159,236,350 \\
081109A & 84.78 & 22:03:09.63 & -54:42:39.9 & 0.3 & O & $0.9785$ & E & 231,236,342 \\
081029A & 9.10 & 23:07:05.35 & -68:09:19.8 & 0.5 & UVOT & $3.8479$ & A & 157,236,350,351 \\
081028A & 29.30 & 08:07:34.76 & 02:18:29.8 & 1.5 & XRT & $3.038$ & A & 156,236,351,357 \\
081008A & 66.00 & 18:39:49.877 & -57:25:52.87 & 0.6 & UVOT & $1.967$ & A & 155,236,350,351 \\
081007A & 3.00 & 22:39:50.40 & -40:08:48.8 & 0.5 & UVOT & $0.5295\pm0.0001$ & E & 154,236,351,357 \\
080928A & 33.00 & 06:20:16.83 & -55:11:58.7 & 0.4 & O & $1.6919$ & A & 173,236,350 \\
080916C & 33.91 & 59:23.3 & -56:38:18.0 & 0.5 & ... & $4.35$ & P & 153,229,324 \\
080916A & 145.91 & 22:25:06.23 & -57:01:22.9 & 0.4 & O & $0.6887$ & A & 173,236,350 \\
080913A & 223.00 & 04:22:54.71 & -25:07:46.7 & 1.5 & XRT & $6.7$ & A & 173,236,351,357 \\
080906A & 96.77 & 15:12:10.65 & -80:31:03.2 & 0.64 & UVOT & $2$ & P & 152,236,351,352 \\
080905B & 17.67 & 20:06:57.89 & -62:33:47.0 & 0.7 & UVOT & $2.3739$ & A & 173,236,351,357 \\
080825B & 49.28 & 13:57:08 & -68:57 & 180 & ... & $4.31^{+0.14}_{-0.15}$ & P & 151,229,353 \\
080810A & 221.49 & 23:47:10.49 & +00:19:11.3 & 0.3 & O & $3.3604$ & A & 173,236,350 \\
080805A & 275.05 & 20:56:53.43 & -62:26:39.3 & 0.3 & O & $1.5052$ & E & 231,236,342 \\
080804A & 284.42 & 21:54:40.18 & -53:11:04.8 & 0.35 & O & $2.2059$ & E & 236,342,350 \\
080721A & 179.52 & 14:57:55.84 & -11:43:24.6 & 0.4 & O & $2.5914$ & A & 173,236,350 \\
080710A & 9.01 & 00:33:05.63 & +19:30:05.4 & 0.3 & O & $0.8454$ & A & 173,236,350 \\
080707A & 233.66 & 02:10:28.40 & 33:06:34.2 & 1.1 & UVOT & $1.2322$ & A & 173,236,351,357 \\
080703A & 62.977 & 06:47:12.639 & -63:13:08.96 & 0.5 & UVOT & $...$ & ... & 236,351 \\
080607A & 61.35 & 12:59:47.21 & +15:55:10.5 & 0.4 & O & $3.0368$ & A & 173,236,350 \\
080605A & 7.46 & 17:28:30.05 & +04:00:56.0 & 0.3 & O & $1.6408$ & E & 231,236,342 \\
080604A & 148.19 & 15:47:51.68 & 20:33:28.0 & 0.5 & UVOT & $1.4171$ & A & 173,236,351,357 \\
080603B & 101.62 & 11:46:07.66 & 68:03:39.99 & 0.3 & UVOT & $2.6892$ & A & 173,236,350,351 \\
080603A & 1.02 & 18:37:31 & +62:44 & 180 & ... & $1.688$ & A & 149,353 \\
080602A & 50 & 01:16:42.17 & -09:13:55.9 & 1.7 & XRT & $1.8204$ & E & 236,342,351 \\
080523A & 107.67 & 01:23:11.54 & -64:01:51.2 & 1.5 & XRT & $<3$ & P & 148,236,351 \\
080520A & 106.62 & 18:40:46.30 & -54:59:31.0 & 0.5 & UVOT & $1.5457$ & E & 173,236,351,357 \\
080517A & 37.19 & 06:48:58.07 & 50:44:06.8 & 1.6 & XRT & $0.089\pm0.003$ & E & 236,346,351 \\
080515A & 176.29 & 0:12:36 & +32:36 & 180 & ... & $2.47$ & E & 236,353,354 \\
080514B & 112.06 & 21:31:17 & +00:44 & 1020 & ... & $1.8^{+0.4}_{-0.3}$ & P & 140,147,353 \\
080430A & 30.17 & 11:01:14.76 & +51:41:08.0 & 0.4 & O & $0.767$ & A & 145,146,236,350 \\
080413B & 3.52 & 21:44:34.65 & -19:58:52.40 & 0.5 & UVOT & $1.1012$ & E & 236,342,351 \\
080413A & 78.86 & 19:09:11.75 & -27:40:40.4 & 0.4 & O & $2.433$ & A & 173,236,350 \\
080411A & 18.05 & 02:31:55.19 & -71:18:07.30 & 0.5 & UVOT & $1.0301$ & A & 173,236,350,351 \\
080330A & 69.16 & 11:17:04.51 & 30:37:22.1 & 1 & UVOT & $1.5119$ & A & 173,236,351,357 \\
080325A & 59.12 & 18:31:34.23 & +36:31:24.8 & 0.3 & I & $1.78$ & E & 2,211,236,350 \\
080320A & ... & 11:50:56.44 & 57:09:24.2 & 1.4 & XRT & $...$ & ... & 236,351 \\
080319C & 74.29 & 17:15:55.49 & 55:23:30.6 & 0.53 & UVOT & $1.9492$ & A & 173,236,351,357 \\
080319B & 48.00 & 14:31:40.99 & +36:18:08.7 & 0.3 & O & $0.9382$ & A & 173,236,350 \\
080319A & 3.32 & 13:45:20.01 & +44:04:48.4 & 0.7 & O & $2.43^{+0.23}_{-0.61}$ & E & 144,236,350 \\
080310A & 64.61 & 14:40:13.80 & -00:10:30.7 & 0.4 & O & $2.4274$ & A & 143,173,236,350 \\
080307A & 20.91 & 09:06:30.88 & 35:08:19.5 & 1.4 & XRT & $...$ & ... & 236,351 \\
080212A & 6.3 & 15:24:35.38 & -22:44:30.1 & 1.4 & XRT & $...$ & ... & 236,351 \\
080210A & 0.32 & 16:45:04.01 & 13:49:35.9 & 0.6 & UVOT & $2.6419$ & A & 173,236,350,351 \\
080207A & 14.15 & 13:50:02.97 & +07:30:07.3 & 0.5 & X & $2.0856$ & E & 236,282,342,350 \\
080205A & 8.00 & 06:33:00.62 & 62:47:31.98 & 0.5 & UVOT & $2.72^{+0.24}_{-0.74}$ & P & 236,350,351 \\
080129A & 46.36 & 07:01:08.17 & -07:50:46.6 & 1.4 & XRT & $4.349$ & A & 168,236,351,357 \\
071122A & 56.33 & 18:26:25.26 & 47:04:30.5 & 1.8 & XRT & $1.14$ & A & 133,236,351,357 \\
071117A & 67.05 & 22:20:10.54 & -63:26:35.9 & 1.5 & XRT & $1.3308$ & E & 173,236,351,357 \\
071112C & 162.82 & 02:36:50.95 & +28:22:16.8 & 0.41 & O & $0.8227$ & A & 173,350,351 \\
071031A & 13.82 & 00:25:37.27 & -58:03:34.2 & 0.5 & UVOT & $2.6918$ & A & 173,236,351 \\
071025A & 29.55 & 23:40:17.07 & +31:46:42.8 & 0.35 & I & $4.8^{+0.4}_{-0.4}$ & A & 131,227,236,350 \\
071021A & 124.86 & 22:42:34.30 & +23:43:06.2 & 0.6 & O & $2.4515$ & E & 130,236,342,350 \\
071020A & 43.62 & 07:58:39.78 & +32:51:40.4 & 0.35 & I & $2.1462$ & A & 129,173,236,350 \\
071010B & 352.37 & 10:02:07 & +45:44 & 180 & ... & $0.947$ & A & 128,236,353,357 \\
071010A & 122.22 & 19:12:24 & -32:23 & 180 & ... & $0.98$ & A & 127,236,352,353 \\
071003A & 117.38 & 20:07:25 & +10:58 & 180 & ... & $1.60435$ & A & 142,236,353,357 \\
070810A & 39.36 & 12:39:51.22 & 10:45:04.3 & 0.6 & UVOT & $2.17$ & A & 126,236,260,351 \\
070808A & 290 & 00:27:03.36 & +01:10:34.4 & 1.5 & X & $...$ & ... & 125,236,260 \\
070802A & 104.06 & 02:27:35.72 & -55:31:39.0 & 0.3 & B & $2.4538$ & E & 231,236,342 \\
070721B & 50.22 & 02:12:32.96 & -02:11:40.8 & 0.38 & O & $3.6298$ & A & 173,236,260,350 \\
070714A & 0.04 & 02:51:43.31 & 30:14:35.0 & 1.8 & XRT & $1.58$ & E & 236,351,354 \\
070621A & 1.8 & 21:35:10.08 & -24:49:03.1 & 1.4 & X & $<5.5$ & E & 124,236,260,350 \\
070612A & 80.00 & 8:05:32 & +37:16 & 180 & ... & $0.617$ & E & 123,236,352,353 \\
070611A & 6.07 & 00:07:58.01 & -29:45:20.0 & 0.5 & UVOT & $2.0394$ & A & 173,236,260,351 \\
070529A & 15 & 18:54:58.19 & 20:39:34.0 & 0.5 & UVOT & $2.4996$ & A & 122,236,351,357 \\
070521A & 150.49 & 16:10:38.62 & 30:15:22.4 & 1.4 & XRT & $2.0865$ & E & 236,342,351 \\
070518A & 241.30 & 16:56:47.7 & 55:17:42.3 & 1 & UVOT & $1.161$ & E & 236,351,354 \\
070508A & 228.72 & 20:51:11.70 & -78:23:05.1 & 0.4 & O & $0.82$ & E & 121,236,350 \\
070506A & 4.30 & 23:08:52.39 & 10:43:20.8 & 0.5 & UVOT & $2.309$ & A & 173,236,260,351 \\
070419B & 36.13 & 21:02:49.77 & -31:15:49.0 & 0.39 & O & $1.9586$ & E & 236,342,350 \\
070419A & 6.32 & 12:10:58.84 & 39:55:31.2 & 1.7 & XRT & $0.9705$ & A & 173,236,351,357 \\
070411A & 148.38 & 07:09:20.01 & 01:03:52.3 & 1.5 & XRT & $2.9538$ & A & 173,236,351,357 \\
070330A & 9.04 & 17:58:09.98 & -63:47:34.80 & 0.5 & UVOT & $...$ & ... & 236,351 \\
070328A & 1.28 & 04:20:27.68 & -34:04:00.7 & 1.4 & X & $2.0627$ & E & 120,236,260,342 \\
070318A & 58.43 & 03:13:56.81 & -42:56:46.1 & 0.35 & O & $0.8401$ & E & 236,342,350 \\
070306A & 15.80 & 09:52:23.31 & +10:28:55.4 & 0.3 & O & $1.4965$ & E & 231,236,342 \\
070224A & 0.43 & 11:56:06.57 & -13:19:48.8 & 1.6 & R & $1.9922$ & E & 118,236,260,342 \\
070223A & 336.86 & 10:13:48.39 & +43:08:00.7 & 0.4 & I & $1.6295$ & E & 119,236,350 \\
070208A & 3 & 13:11:32.61 & 61:57:54.3 & 1.5 & XRT & $1.165$ & E & 117,236,351,357 \\
070129A & 3.00 & 02:28:00.94 & +11:41:04.1 & 0.31 & O & $2.3384$ & E & 236,342,350 \\
070125A & 0.8 & 51:17.8 & +31:09:04.11 & 0.3 & ... & $1.547$ & A & 115,116,173 \\
070110A & 33.26 & 00:03:39.27 & -52:58:27.2 & 0.3 & O & $2.3523$ & E & 236,342,350 \\
070103A & 365.28 & 23:30:13.80 & +26:52:34.4 & 1.5 & X & $2.6208$ & E & 114,236,260,342 \\
061222B & 13.18 & 07:01:24.67 & -25:51:35.2 & 1.7 & XRT & $3.355$ & A & 98,236,351,357 \\
061222A & 108.90 & 23:53:03.41 & +46:31:58.6 & 0.3 & I & $2.088$ & E & 99,166,236,350 \\
061202A & 38.63 & 07:02:06.07 & -74:41:54.7 & 1.4 & XRT & $2.2543$ & E & 236,342,351 \\
061126A & 4.35 & 05:46:24.46 & 64:12:38.5 & 0.5 & UVOT & $1.1588$ & E & 141,236,351 \\
061121A & 20.90 & 09:48:54.55 & -13:11:42.9 & 0.36 & O & $1.3145$ & A & 173,236,260,350 \\
061110B & 4.35 & 21:35:40.39 & +06:52:34.0 & 0.24 & O & $3.4344$ & A & 173,236,260,350 \\
061110A & 0.49 & 22:25:09.84 & -02:15:31.4 & 0.37 & O & $0.7578$ & E & 236,342,350 \\
061021A & 238.14 & 09:40:36.12 & -21:57:04.8 & 0.3 & O & $0.3453$ & E & 236,342,350 \\
061007A & 160.00 & 03:05:19.58 & -50:30:02.3 & 0.33 & O & $1.2622$ & A & 95,236,260,350 \\
060927A & 102.04 & 21:58:12.01 & +05:21:48.6 & 0.19 & O & $5.4636$ & A & 111,236,260,350 \\
060926A & 6.64 & 17:35:43.66 & 13:02:18.6 & 0.5 & UVOT & $3.2086$ & A & 173,236,351,357 \\
060923C & 72.12 & 23:04:28.28 & +03:55:28.1 & 3.5 & J & $...$ & ... & 94,236,260 \\
060923B & 131.52 & 15:52:46.70 & -30:54:13.7 & 1.8 & X & $1.5094$ & E & 93,236,260,342 \\
060923A & 209.24 & 16:58:28.14 & +12:21:37.9 & 1.5 & K & $2.6$ & E & 162,236,260,291 \\
060912A & 48.00 & 00:21:08.14 & +20:58:17.4 & 0.35 & O & $0.9362$ & E & 236,342,350 \\
060908A & 100.00 & 02:07:18.41 & +00:20:31.3 & 0.42 & O & $1.8836$ & A & 236,260,283,350 \\
060906A & 64.00 & 02:43:00.88 & 30:21:42.7 & 1.4 & XRT & $3.6856$ & A & 173,236,351,357 \\
060904B & 459.05 & 03:52:50.54 & -00:43:31.1 & 0.5 & UVOT & $0.7029$ & E & 173,236,351,357 \\
060814A & 70 & 14:45:21.31 & +20:35:10.5 & 0.18 & O & $1.9223$ & E & 236,342,350 \\
060807A & 79.71 & 16:50:02.65 & 31:35:29.9 & 1.4 & XRT & $...$ & ... & 236,351 \\
060805A & 18.40 & 14:43:43.47 & +12:35:11.2 & 1.6 & X & $2.3633$ & E & 92,236,260,342 \\
060729A & 37.25 & 06:21:31.80 & -62:22:12.3 & 0.27 & O & $0.5429$ & E & 236,342,350 \\
060719A & 96.00 & 01:13:43.71 & -48:22:51.0 & 0.29 & O & $1.5318$ & E & 236,342,350 \\
060714A & 0.24 & 15:11:26.41 & -06:33:58.3 & 0.43 & O & $2.7108$ & A & 76,236,260,350 \\
060708A & 0.13 & 00:31:13.82 & -33:45:32.4 & 0.5 & UVOT & $1.92$ & P & 207,236,260,351 \\
060707A & 94.19 & 23:48:19.06 & -17:54:17.3 & 0.37 & O & $3.4246$ & E & 236,342,350 \\
060614A & 0.78 & 21:23:32.08 & -53:01:36.2 & 0.56 & UVOT & $0.125$ & E & 101,260,344,351 \\
060607A & 50.28 & 21:58:50.40 & -22:29:47.1 & 0.38 & I & $3.0749$ & A & 139,236,260,350 \\
060605A & 81.22 & 21:28:37.32 & -06:03:31.3 & 0.5 & UVOT & $3.773$ & A & 164,236,260,351 \\
060604A & 132.76 & 22:28:55.01 & -10:54:55.8 & 0.6 & UVOT & $2.1355$ & E & 236,342,351 \\
060602A & 44.51 & 09:58:16.28 & +00:18:14.4 & 5.2 & R & $0.787$ & E & 88,132,236,260 \\
060526A & 43.80 & 15:31:18.34 & +00:17:04.9 & 0.16 & O & $3.2213$ & A & 87,236,260,350 \\
060522A & 75.74 & 21:31:44.84 & +02:53:09.7 & 0.42 & O & $5.11$ & A & 112,236,260,350 \\
060512A & 0.5 & 13:03:05.81 & 41:11:27.2 & 0.5 & UVOT & $0.4428$ & E & 89,236,351 \\
060510B & 22.42 & 15:56:29.48 & +78:34:12.1 & 0.2 & O & $4.9$ & A & 86,236,350 \\
060505A & 7.79 & 22:07:03.32 & -27:48:53.0 & 2 & B & $0.0889$ & E & 109,169,260,351 \\
060502A & 67.41 & 16:03:42.62 & +66:36:03.0 & 0.4 & O & $1.5026$ & A & 173,236,350 \\
060418A & 8.95 & 15:45:42.60 & -03:38:20.0 & 0.5 & UVOT & $1.4901$ & A & 103,236,351,357 \\
060319A & 51.54 & 11:45:33.04 & 60:00:38.9 & 1.4 & XRT & $1.172$ & E & 236,291,351 \\
060306A & 5.03 & 02:44:22.92 & -02:08:54.1 & 1.3 & X & $1.5597$ & E & 106,236,342,350 \\
060223A & 18.78 & 03:40:49.56 & -17:07:48.4 & 1 & UVOT & $4.406$ & A & 112,236,260,351 \\
060218A & 44.58 & 03:21:39.68 & +16:52:01.9 & 0.28 & O & $0.03351$ & E & 79,236,260,350 \\
060210A & 171.90 & 03:50:57.38 & +27:01:34.2 & 0.6 & O & $3.9122$ & A & 85,173,236,350 \\
060206A & 144.95 & 13:31:43.45 & 35:03:03.2 & 1.5 & XRT & $4.0559$ & A & 173,236,351,357 \\
060204B & 53.74 & 14:07:14.89 & +27:40:36.2 & 1.1 & O & $2.3393$ & E & 84,236,342,350 \\
060202A & 4.93 & 02:23:22.94 & +38:23:03.9 & 0.5 & I & $0.785$ & E & 236,291,350 \\
060124A & 0.50 & 05:08:25.86 & 69:44:26.4 & 1.4 & XRT & $2.3$ & A & 173,236,351,357 \\
060123A & 113.04 & 11:59:00 & +45:31 & 180 & ... & $1.099$ & E & 83,351,352,353 \\
060115A & 66.86 & 03:36:08.32 & +17:20:42.8 & 0.31 & O & $3.5328$ & A & 173,236,260,350 \\
060111A & 116.04 & 18:24:49.10 & 37:36:14.7 & 1.4 & XRT & $2.32$ & E & 236,351,355 \\
060108A & 9.96 & 09:48:02.06 & 31:55:06.9 & 1.5 & XRT & $2.03$ & P & 82,236,351,352 \\
051117B & 66.65 & 05:40:43.38 & -19:16:27.2 & 1.7 & X & $0.4805$ & E & 68,236,260,342 \\
051111A & 5 & 23:12:33.08 & 18:22:28.6 & 1.5 & XRT & $1.55$ & A & 173,236,351,357 \\
051109B & 102.98 & 23:01:50.36 & 38:40:46.7 & 1.5 & XRT & $0.08$ & E & 91,236,351,352 \\
051109A & 539.12 & 22:01:15.32 & 40:49:23.7 & 0.5 & UVOT & $2.346$ & A & 67,236,351,357 \\
051022A & 96.00 & 23:56:00 & +19:36 & 120 & ... & $0.809$ & E & 104,138,353 \\
051016B & 74.68 & 08:48:27.85 & +13:39:20.4 & 1.4 & UVW2 & $0.9358$ & E & 66,236,260,342 \\
051008A & 275.20 & 13:31:29.62 & 42:05:53.4 & 1.4 & XRT & $2.77^{+0.15}_{-0.2}$ & P & 236,341,351 \\
051006A & 69.12 & 07:23:14.14 & +09:30:20.0 & 1.5 & X & $1.059$ & E & 65,236,259,260 \\
051001A & 11.36 & 23:23:48.72 & -31:31:23.6 & 1.5 & X & $2.4295$ & E & 106,236,342,350 \\
050922C & 262.95 & 21:09:33.08 & -08:45:30.3 & 0.3 & O & $2.1992$ & A & 64,76,236,260,350 \\
050922B & 4 & 00:23:13.37 & -05:36:16.7 & 1.7 & X & $4.9^{+0.3}_{-0.6}$ & P & 63,236,260,350 \\
050915A & 0.14 & 05:26:44.81 & -28:00:59.4 & 1.4 & H & $2.5275$ & E & 62,236,260,342 \\
050908A & 28.54 & 01:21:50.70 & -12:57:18.0 & 1.5 & V & $3.3467$ & A & 61,173,236,260 \\
050904A & 109.17 & 00:54:50.88 & +14:05:09.5 & 0.4 & O & $6.295$ & A & 100,236,260,350 \\
050826A & 8.91 & 05:51:01.56 & -02:38:35.9 & 1.5 & XRT & $0.296$ & E & 108,236,351,357 \\
050824A & 0.74 & 00:48:56.21 & +22:36:33.1 & 1.5 & UVW2 & $0.8277$ & E & 135,236,260,342 \\
050822A & 60.94 & 03:24:27.22 & -46:02:00.1 & 0.7 & X & $1.434$ & E & 106,236,259,260,350 \\
050820A & 11.32 & 22:29:38.10 & +19:33:36.8 & 0.31 & O & $2.61469$ & A & 113,260,350,351 \\
050819A & 1040 & 23:55:01.62 & +24:51:39.0 & 1.5 & X & $2.5042$ & E & 60,236,260,342 \\
050814A & 242.18 & 17:36:45.39 & +46:20:21.2 & 0.3 & O & $5.3\pm0.3$ & P & 59,73,236,350 \\
050803A & 7.55 & 23:22:37.85 & +05:47:08.5 & 1.4 & X & $4.3^{+0.6}_{-2.4}$ & P & 58,236,260,350 \\
050802A & 139.46 & 14:37:05.84 & +27:47:12.4 & 0.6 & O & $1.7102$ & A & 173,236,350 \\
050801A & 172.16 & 13:36:35 & -21:55:41 & 1 & UVOT & $1.38$ & P & 207,236,260,351 \\
050730A & 658.2 & 14:08:17.10 & -03:46:17.6 & 0.37 & O & $3.96855$ & A & 53,236,260,350 \\
050726A & 900 & 13:20:11.95 & -32:03:51.2 & 0.32 & U & $<3.5$ & P & 236,350 \\
050714B & 2.61 & 11:18:47.71 & -15:32:49.0 & 1.5 & X & $2.4383$ & E & 57,236,260,342 \\
050713A & 122.21 & 21:22:09.30 & 77:04:28.8 & 1.4 & XRT & $<3.6$ & P & 166,236,351 \\
050525A & 13.21 & 18:32:32.59 & +26:20:22.3 & 0.31 & O & $0.6063$ & E & 236,342,350 \\
050505A & 14.22 & 09:27:03.33 & 30:16:24.4 & 1.4 & XRT & $4.2748$ & A & 78,236,351,357 \\
050502B & 3.5 & 09:30:10.13 & +16:59:48.0 & 1.4 & R & $5.2$ & P & 230,236,260 \\
050502A & 1.40 & 13:29:46 & +42:40 & 180 & ... & $3.793$ & A & 55,56,353 \\
050416A & 1.27 & 12:33:54.64 & +21:03:26.8 & 1.4 & UVW2 & $0.6542$ & E & 105,236,260,342 \\
050408A & 9.01 & 12:01:55 & +10:52 & 120 & ... & $1.2356\pm0.0008$ & E & 52,138,353 \\
050401A & 64.00 & 16:31:28.80 & +02:11:14.0 & 0.43 & O & $2.8983$ & A & 81,236,260,350 \\
050319A & 13.38 & 10:16:47.94 & +43:32:53.5 & 0.4 & O & $3.2425$ & A & 173,236,350 \\
050318A & 37.20 & 03:18:51.01 & -46:23:44.0 & 0.6 & O & $1.4436$ & A & 52,54,236,260,350 \\
050315A & 178 & 20:25:54.17 & -42:36:02.2 & 0.28 & O & $1.95$ & A & 52,236,260,350 \\
050223A & 4.02 & 18:05:32 & -62:30 & 240 & ... & $0.584$ & E & 75,236,353,357 \\
050219A & 64.0 & 11:05:38.98 & -40:41:03.1 & 1.9 & XRT & $0.211$ & E & 236,321,351 \\
050215B & 26.04 & 11:37:47.57 & 40:47:49.4 & 2.2 & XRT & $2.62$ & E & 236,351,355 \\
050128A & 190.63 & 14:38:17.66 & -34:45:54.7 & 1.7 & XRT & $<5.5$ & P & 236,350,351 \\
050126A & 4.54 & 18:32:27 & +42:23 & 240 & ... & $1.29002\pm0.00002$ & E & 50,236,353 \\
041219A & 156.29 & 0:24:26 & +62:50 & 120 & ... & $0.31\pm0.26$ & P & 258,351,353 \\
041006A & 53.42 & 0:54:53 & +01:12 & 300 & ... & $0.716$ & E & 77,138,353 \\
040924A & 18.29 & 2:06:19 & +16:01 & 360 & ... & $0.858\pm0.001$ & E & 136,138,353 \\
040912A & 181.70 & 23:56:54 & -01:00 & 420 & ... & $1.563\pm0.001$ & E & 102,138,353 \\
031203A & 35.73 & 8:02:30 & -39:51 & 120 & ... & $0.1055\pm0.0001$ & E & 46,138,353 \\
030528A & 24.82 & 17:04:02 & -22:39 & 120 & ... & $0.782\pm0.001$ & A & 48,138,353 \\
030429A & 104.12 & 12:13:06 & -20:56 & 120 & ... & $2.658\pm0.004$ & A & 43,138,353 \\
030329A & 26 & 10:44:50 & +21:31 & 120 & ... & $0.1685$ & E & 40,138,353 \\
030328A & 37.72 & 12:10:46 & -09:22 & 120 & ... & $1.5216$ & A & 74,138,353 \\
030323A & 144.00 & 11:06:06 & -21:54 & 720 & ... & $3.3736\pm0.0006$ & E & 39,41,353 \\
030226A & 88.12 & 11:33:05 & +25:54 & 120 & ... & $1.986\pm0.001$ & A & 44,138,353 \\
030115A & 27.46 & ... & ... & ... & ... & $...$ & ... & 138 \\
021211A & 19.40 & 8:08:55 & +06:44 & 840 & ... & $1.006$ & E & 38,138,353 \\
021004A & 145.05 & 0:26:56 & +18:56 & 120 & ... & $2.3351$ & E & 19,138,353 \\
020903A & 49.70 & 22:49:01 & -20:56 & 960 & ... & $0.251$ & E & 29,45,353 \\
020819B & 2.76 & 23:27:24 & +06:16 & 120 & ... & $0.41$ & E & 28,49,353 \\
020813A & 46.87 & 19:46:38 & -19:35 & 60 & ... & $1.255$ & E & 33,138,353 \\
020427A & 94.91 & ... & ... & ... & ... & $...$ & ... & 27 \\
020410A & 0.22 & ... & ... & ... & ... & $...$ & ... & 42 \\
020405A & 8.84 & 13:58:10 & -31:23 & 900 & ... & $0.6908\pm0.0017$ & E & 31,172,353 \\
020331A & 0.02 & ... & ... & ... & ... & $...$ & ... & 138 \\
020322A & 58.88 & ... & ... & ... & ... & $...$ & ... & 172 \\
020305A & 16.62 & 12:43:03 & -14:33 & 1500 & ... & $2.8$ & P & 47,138,353 \\
020127A & 17.5 & 8:15:06 & +36:44 & 480 & ... & $1.9$ & P & 107,138,353 \\
020124A & 6.62 & 9:33:08 & -11:35 & 1140 & ... & $3.198\pm0.004$ & A & 36,138,353 \\
011211A & 28.39 & 11:15:16 & -21:56 & 60 & ... & $2.14\pm0.001$ & A & 20,172,353 \\
011121A & 33.30 & 11:34:25 & -76:02 & 120 & ... & $0.36$ & E & 37,172,353 \\
011030A & 151.74 & 20:43:35 & +77:17 & 120 & ... & $<3$ & P & 18,26,353 \\
010921A & 40.0 & 22:55:35 & +40:56 & 1200 & ... & $0.4509$ & E & 21,172,353 \\
010222A & 95.57 & 14:52:12 & +43:01 & 120 & ... & $1.47688$ & A & 24,172,353 \\
000926A & 21.68 & 17:04:15 & +51:46 & 180 & ... & $2.0379\pm0.0008$ & A & 34,172,353 \\
000911A & 23.84 & 2:18:42 & +07:48 & 180 & ... & $1.0585$ & E & 13,22,353 \\
000418A & 10.62 & 12:25:21 & +20:05 & 240 & ... & $1.1181\pm0.0001$ & E & 32,172,353 \\
000301C & 28.00 & 16:20:22 & +29:25 & 360 & ... & $2.0404\pm0.0008$ & A & 15,172,353 \\
000214A & 48.00 & 18:54:18 & -66:27 & 480 & ... & $...$ & ... & 172,353 \\
000210A & 520 & 1:59:15 & -40:40 & 180 & ... & $0.846$ & E & 23,172,353 \\
000131A & 22.08 & 6:13:33 & -51:56 & 180 & ... & $4.5\pm0.015$ & A & 11,12,353 \\
991216A & 3.37 & 5:19:31 & +11:11 & 180 & ... & $1.02$ & A & 9,172,353 \\
991208A & 9.21 & 16:33:55 & +46:26 & 840 & ... & $0.7063\pm0.0017$ & E & 8,14,353 \\
990712A & 10.38 & 22:31:50 & -73:24 & 120 & ... & $0.4331\pm0.0004$ & E & 16,172,353 \\
990705A & 62.8 & 5:09:32 & -72:09 & 360 & ... & $0.8424\pm0.0002$ & E & 25,172,353 \\
990510A & 12.95 & 13:38:06 & -80:30 & 180 & ... & $1.619$ & A & 16,172,353 \\
990506A & 25.91 & 11:54:41 & -26:45 & 420 & ... & $1.30658\pm0.00004$ & E & 32,172,353 \\
990308A & 138.27 & ... & ... & ... & ... & $...$ & ... & 172 \\
990123A & 26 & 15:25:29 & +44:45 & 120 & ... & $1.6004$ & A & 10,172,353 \\
981226A & 76.23 & ... & ... & ... & ... & $1.11\pm0.06$ & P & 51,172 \\
980703A & 20.33 & 23:59:07 & +08:35.6 & 240 & ... & $0.966$ & E & 4,172,353 \\
980613A & 4.23 & 10:17:46 & +71:29.9 & 240 & ... & $1.0969$ & E & 35,172,353 \\
980519A & 48.94 & ... & ... & ... & ... & $...$ & ... & 172 \\
980425A & 3.3 & 19:34:54 & -52:49.9 & 480 & ... & $0.0085\pm0.0002$ & E & 5,172,353 \\
980329A & 20 & 7:02:41 & +38:50.7 & 180 & ... & $3.5$ & P & 30,172,353 \\
980326A & 87.34 & 8:36:26 & -18:53.0 & 480 & ... & $...$ & ... & 172,353 \\
971214A & 66 & 11:56:30 & +65:12.0 & 240 & ... & $3.42$ & E & 6,172,353 \\
970828A & 1500 & 18:08:29 & +59:18.0 & 120 & ... & $0.9578$ & E & 17,353 \\
970508A & 40.0 & 6:53:28 & +79:17.4 & 180 & ... & $0.835$ & A & 3,172,353 \\
970228A & 179.4 & 5:01:57 & +11:46.4 & 180 & ... & $0.695\pm0.002$ & E & 7,172,353 \\
\hline
&SGRB&\\\hline
130603B & 0.18 & 21:51:00 & +33:41 & 10800 & ... & $0.384$ & E & 339,349,353 \\
101224A & 0.2 & 15:09:00.60 & 42:25:05.6 & 1.5 & XRT & $4.707$ & A & 337,351,352 \\
101219A & 0.6 & 12:24:15.45 & 15:06:17.0 & 1.5 & XRT & $6.32$ & A & 336,351,352 \\
100816A & 2.9 & 19:17:28.78 & -15:05:39.2 & 0.61 & UVOT & $0.725$ & A & 338,351,352 \\
100625A & 0.33 & 03:06:22.69 & -62:38:21.7 & 0.42 & UVOT & $2.4$ & P & 335,351 \\
100206A & 0.12 & 17:02:31 & +46:45 & 5400 & ... & $1.027$ & A & 333,334,353 \\
100117A & 0.3 & 18:27:06.04 & -55:38:08.7 & 0.43 & UVOT & $0.8893$ & E & 342,351 \\
091109B & 0.27 & 06:51:44.61 & 23:01:25.2 & 0.62 & UVOT & $1.6019$ & E & 342,351 \\
090515A & 0.04 & 12:57:28.45 & 28:23:05.7 & 1.7 & XRT & $4.7$ & A & 332,351,352 \\
090510A & 5.66 & 13:09:08.54 & 49:50:29.4 & 0.48 & UVOT & $3.26$ & A & 331,351,352 \\
090426A & 1.24 & 08:27:57.56 & 46:14:25.3 & 0.5 & UVOT & $3.956$ & A & 330,351,352 \\
090305A & 0.35 & 12:16:21.42 & 20:12:32.9 & 1.6 & XRT & $1.02$ & E & 345,351,352 \\
080905A & 1.02 & 13:57:13.25 & 00:38:30.8 & 1.5 & XRT & $4.954$ & A & 329,351,352 \\
080503A & 0.32 & 02:02:34.26 & 33:28:25.7 & 1.6 & XRT & $5.283$ & A & 328,351,352 \\
080123A & 0.04 & 04:38:13.81 & -34:15:24.3 & 1.6 & XRT & $1.4155$ & E & 342,351 \\
071227A & 1.8 & 14:45:58 & +15:00 & 0 & ... & $1.98$ & A & 343,353 \\
070809A & 1.28 & 07:00:37.13 & -73:08:13.5 & 0.51 & UVOT & $1.2079$ & E & 342,351 \\
070724A & 0.43 & 09:41:20.26 & 66:45:38.6 & 0.5 & UVOT & $2.739$ & A & 327,351 \\
070714B & 3 & 12:34:05.16 & 27:57:02.6 & 1.4 & XRT & $3\pm0.1$ & A & 342,351 \\
070707A & 0.8 & 5:40:57 & -04:26 & 540 & ... & $0.642$ & E & 325,326,353 \\
070429B & 0.49 & 04:29:30.78 & 28:52:58.9 & 1.4 & XRT & $5.3$ & A & 318,351,352 \\
061217A & 0.24 & 22:09:19.36 & -31:45:44.3 & 0.64 & UVOT & $4.042$ & A & 316,351,352 \\
061210A & 0.13 & 10:25:53 & +09:54 & 1800 & ... & $2.4$ & A & 314,315,353 \\
061201A & 0.78 & 04:43:52.18 & -62:59:42.7 & 1.4 & XRT & $1.6854$ & E & 342,351 \\
061006A & 0.5 & 23:15:40.55 & -44:38:25.4 & 0.6 & UVOT & $0.596$ & E & 342,351 \\
060801A & 0.50 & 23:00:16.14 & -05:22:05.2 & 0.5 & UVOT & $1.293$ & A & 313,351,352 \\
060502B & 0.14 & 1:27:41 & +09:33 & 18900 & ... & $1.874$ & A & 311,312,353 \\
060313A & 0.74 & 19:44:27.09 & -02:57:30.4 & 0.55 & UVOT & $0.717$ & E & 310,351,352 \\
060121A & 2.61 & 02:44:42.97 & -26:09:11.5 & 1.4 & XRT & $0.3483$ & E & 319,342,351 \\
051227A & 3.5 & 14:23:34.04 & 45:36:27.1 & 0.5 & UVOT & $1.238$ & A & 309,351,352 \\
051221A & 1.40 & 23:54:29.89 & 29:25:46.2 & 0.74 & UVOT & $0.4791$ & A & 308,351,352 \\
051210A & 1.27 & 1:09:54 & +00:00 & 24720 & ... & $0.145$ & E & 289,307,353 \\
050724A & 2.76 & 23:48:55.08 & 36:06:01.5 & 1.5 & XRT & $1.1548$ & E & 342,351 \\
050709A & 0.22 & 17:19:10.58 & 16:43:11.9 & 0.53 & UVOT & $2.006$ & A & 306,351,352 \\
050509B & 0.02 & 14:57:40.88 & 28:12:25.8 & 0.51 & UVOT & $2.092$ & A & 305,351,352 \\
\enddata
\tablecomments{References.
(1) \citet{};
(2) \citet{-1};
(3) \citet{1997IAUC.6655....1G};
(4) \citet{1998ApJ...508L..17D};
(5) \citet{1998IAUC.6896....3W};
(6) \citet{1998Natur.393...35K};
(7) \citet{1999GCN...289....1D};
(8) \citet{1999GCN...450....1H};
(9) \citet{1999GCN...496....1V};
(10) \citet{1999Natur.398..389K};
(11) \citet{2000A&A...364L..54A};
(12) \citet{2000GCN...529....1H};
(13) \citet{2000GCN...791....1H};
(14) \citet{2001A&A...370..398C};
(15) \citet{2001A&A...370..909J};
(16) \citet{2001ApJ...546..672V};
(17) \citet{2001ApJ...562..654D};
(18) \citet{2001GCN..1138....1H};
(19) \citet{2002A&A...396L..21M};
(20) \citet{2002AJ....124..639H};
(21) \citet{2002ApJ...571L.121P};
(22) \citet{2002ApJ...573...85P};
(23) \citet{2002ApJ...577..680P};
(24) \citet{2002ApJ...578..818M};
(25) \citet{2002ApJ...581L..81L};
(26) \citet{2002GCN..1268....1F};
(27) \citet{2002GCN..1383....1I};
(28) \citet{2002GCN..1507....1H};
(29) \citet{2002GCN..1530....1R};
(30) \citet{2003A&A...402..125J};
(31) \citet{2003A&A...404..465M};
(32) \citet{2003AJ....125..999B};
(33) \citet{2003ApJ...584L..47B};
(34) \citet{2003ApJ...586..128C};
(35) \citet{2003ApJ...591L..13D};
(36) \citet{2003ApJ...597..699H};
(37) \citet{2003ApJ...599.1223G};
(38) \citet{2003GCN..1785....1V};
(39) \citet{2003GCN..1956....1G};
(40) \citet{2003Natur.423..847H};
(41) \citet{2004A&A...419..927V};
(42) \citet{2004A&A...427..445N};
(43) \citet{2004A&A...427..785J};
(44) \citet{2004AJ....128.1942K};
(45) \citet{2004ApJ...606..994S};
(46) \citet{2004ApJ...611..200P};
(47) \citet{2005A&A...437..411G};
(48) \citet{2005A&A...444..425R};
(49) \citet{2005ApJ...629...45J};
(50) \citet{2005ApJ...629..328B};
(51) \citet{2005ApJ...631L..29C};
(52) \citet{2005ApJ...634..501B};
(53) \citet{2005ApJ...634L..25C};
(54) \citet{2005GCN..3114....1M};
(55) \citet{2005GCN..3332....1P};
(56) \citet{2005GCN..3339....1C};
(57) \citet{2005GCN..3613....1L};
(58) \citet{2005GCN..3748....1B};
(59) \citet{2005GCN..3807....1C};
(60) \citet{2005GCN..3827....1K};
(61) \citet{2005GCN..3960....1D};
(62) \citet{2005GCN..3984....1B};
(63) \citet{2005GCN..4008....1N};
(64) \citet{2005GCN..4015....1J};
(65) \citet{2005GCN..4062....1M};
(66) \citet{2005GCN..4107....1B};
(67) \citet{2005GCN..4221....1Q};
(68) \citet{2005GCN..4282....1B};
(69) \citet{2005Natur.437..845F};
(70) \citet{2005Natur.437..851G};
(71) \citet{2005Natur.437..855V};
(72) \citet{2005Natur.438..988B};
(73) \citet{2006A&A...447..897J};
(74) \citet{2006A&A...455..423M};
(75) \citet{2006A&A...459L...5P};
(76) \citet{2006A&A...460L..13J};
(77) \citet{2006ApJ...636..391S};
(78) \citet{2006ApJ...642..979B};
(79) \citet{2006ApJ...643L..99M};
(80) \citet{2006ApJ...650..261S};
(81) \citet{2006ApJ...652.1011W};
(82) \citet{2006GCN..4539....1M};
(83) \citet{2006GCN..4622....1B};
(84) \citet{2006GCN..4661....1G};
(85) \citet{2006GCN..4726....1M};
(86) \citet{2006GCN..5104....1P};
(87) \citet{2006GCN..5170....1B};
(88) \citet{2006GCN..5203....1J};
(89) \citet{2006GCN..5217....1B};
(90) \citet{2006GCN..5238....1B};
(91) \citet{2006GCN..5387....1P};
(92) \citet{2006GCN..5398....1Z};
(93) \citet{2006GCN..5590....1S};
(94) \citet{2006GCN..5604....1C};
(95) \citet{2006GCN..5715....1O};
(96) \citet{2006GCN..5946....1C};
(97) \citet{2006GCN..5952....1B};
(98) \citet{2006GCN..5962....1B};
(99) \citet{2006GCN..5978....1C};
(100) \citet{2006Natur.440..184K};
(101) \citet{2006Natur.444.1053G};
(102) \citet{2007A&A...461..485S};
(103) \citet{2007A&A...468...83V};
(104) \citet{2007A&A...475..101C};
(105) \citet{2007AJ....133..122H};
(106) \citet{2007AJ....133.1027B};
(107) \citet{2007ApJ...660..504B};
(108) \citet{2007ApJ...661L.127M};
(109) \citet{2007ApJ...662.1129O};
(110) \citet{2007ApJ...664.1000B};
(111) \citet{2007ApJ...669....1R};
(112) \citet{2007ApJ...671..272C};
(113) \citet{2007ApJS..168..231P};
(114) \citet{2007GCN..5988....1S};
(115) \citet{2007GCN..6034....1C};
(116) \citet{2007GCN..6049....1G};
(117) \citet{2007GCN..6083....1C};
(118) \citet{2007GCN..6142....1T};
(119) \citet{2007GCN..6221....1R};
(120) \citet{2007GCN..6224....1M};
(121) \citet{2007GCN..6398....1J};
(122) \citet{2007GCN..6470....1B};
(123) \citet{2007GCN..6556....1C};
(124) \citet{2007GCN..6560....1S};
(125) \citet{2007GCN..6718....1C};
(126) \citet{2007GCN..6741....1T};
(127) \citet{2007GCN..6864....1P};
(128) \citet{2007GCN..6888....1C};
(129) \citet{2007GCN..6953....1B};
(130) \citet{2007GCN..6971....1C};
(131) \citet{2007GCN..6989....1B};
(132) \citet{2007GCN..6997....1J};
(133) \citet{2007GCN..7124....1C};
(134) \citet{2007GCN..7154....1B};
(135) \citet{2007MNRAS.377..273S};
(136) \citet{2008A&A...481..319W};
(137) \citet{2008A&A...486..405M};
(138) \citet{2008A&A...491..157P};
(139) \citet{2008A&A...491..189F};
(140) \citet{2008A&A...491L..29R};
(141) \citet{2008ApJ...672..449P};
(142) \citet{2008ApJ...688..470P};
(143) \citet{2008GCN..7381....1C};
(144) \citet{2008GCN..7429....1C};
(145) \citet{2008GCN..7654....1C};
(146) \citet{2008GCN..7670....1R};
(147) \citet{2008GCN..7752....1H};
(148) \citet{2008GCN..7770....1F};
(149) \citet{2008GCN..7791....1P};
(150) \citet{2008GCN..7889....1P};
(151) \citet{2008GCN..8133....1E};
(152) \citet{2008GCN..8212....1H};
(153) \citet{2008GCN..8257....1C};
(154) \citet{2008GCN..8335....1B};
(155) \citet{2008GCN..8346....1C};
(156) \citet{2008GCN..8434....1B};
(157) \citet{2008GCN..8438....1D};
(158) \citet{2008GCN..8528....1D};
(159) \citet{2008GCN..8531....1D};
(160) \citet{2008GCN..8542....1B};
(161) \citet{2008GCN..8713....1C};
(162) \citet{2008MNRAS.388.1743T};
(163) \citet{2008arXiv0802.0874C};
(164) \citet{2009A&A...497..729F};
(165) \citet{2009A&A...498..711D};
(166) \citet{2009AJ....138.1690P};
(167) \citet{2009ApJ...690..231B};
(168) \citet{2009ApJ...693.1912G};
(169) \citet{2009ApJ...696..971X};
(170) \citet{2009ApJ...696.1871P};
(171) \citet{2009ApJ...704..877B};
(172) \citet{2009ApJS..180..192F};
(173) \citet{2009ApJS..185..526F};
(174) \citet{2009GCN..10031...1C};
(175) \citet{2009GCN..10042...1d};
(176) \citet{2009GCN..10053...1X};
(177) \citet{2009GCN..10065...1C};
(178) \citet{2009GCN..10100...1C};
(179) \citet{2009GCN..10272...1P};
(180) \citet{2009GCN..8766....1D};
(181) \citet{2009GCN..8892....1F};
(182) \citet{2009GCN..8979....1C};
(183) \citet{2009GCN..8994....1C};
(184) \citet{2009GCN..9043....1H};
(185) \citet{2009GCN..9060....1F};
(186) \citet{2009GCN..9151....1C};
(187) \citet{2009GCN..9156....1B};
(188) \citet{2009GCN..9179....1P};
(189) \citet{2009GCN..9243....1C};
(190) \citet{2009GCN..9264....1L};
(191) \citet{2009GCN..9353....1R};
(192) \citet{2009GCN..9383....1d};
(193) \citet{2009GCN..9403....1T};
(194) \citet{2009GCN..9409....1T};
(195) \citet{2009GCN..9457....1M};
(196) \citet{2009GCN..9518....1C};
(197) \citet{2009GCN..9635....1M};
(198) \citet{2009GCN..9673....1W};
(199) \citet{2009GCN..9712....1F};
(200) \citet{2009GCN..9761....1M};
(201) \citet{2009GCN..9769....1C};
(202) \citet{2009GCN..9771....1d};
(203) \citet{2009GCN..9797....1J};
(204) \citet{2009GCN..9873....1C};
(205) \citet{2009GCN..9874....1O};
(206) \citet{2009GCN..9958....1L};
(207) \citet{2009MNRAS.395..490O};
(208) \citet{2009MNRAS.395L..21K};
(209) \citet{2009Natur.461.1254T};
(210) \citet{2010ApJ...708....9F};
(211) \citet{2010ApJ...719..378H};
(212) \citet{2010ApJ...720..862R};
(213) \citet{2010ApJ...725.1202L};
(214) \citet{2010GCN..10350...1R};
(215) \citet{2010GCN..10441...1G};
(216) \citet{2010GCN..10466...1C};
(217) \citet{2010GCN..10495...1V};
(218) \citet{2010GCN..10524...1S};
(219) \citet{2010GCN..10606...1C};
(220) \citet{2010GCN..10684...1G};
(221) \citet{2010GCN..10752...1C};
(222) \citet{2010GCN..10782...1A};
(223) \citet{2010GCN..10915...1B};
(224) \citet{2010GCN..11164...1C};
(225) \citet{2010GCN..11230...1T};
(226) \citet{2010GCN..11317...1F};
(227) \citet{2010MNRAS.406.2473P};
(228) \citet{2010MNRAS.408..383R};
(229) \citet{2011A&A...526A.153K};
(230) \citet{2011A&A...526A.154A};
(231) \citet{2011A&A...534A.108K};
(232) \citet{2011ApJ...730...26F};
(233) \citet{2011ApJ...732...29C};
(234) \citet{2011ApJ...735L..24S};
(235) \citet{2011ApJ...736....7C};
(236) \citet{2011ApJS..195....2S};
(237) \citet{2011GCN..11518...1C};
(238) \citet{2011GCN..11538...1C};
(239) \citet{2011GCN..11607...1S};
(240) \citet{2011GCN..11633...1M};
(241) \citet{2011GCN..11638...1C};
(242) \citet{2011GCN..11708...1M};
(243) \citet{2011GCN..11722...1G};
(244) \citet{2011GCN..11736...1C};
(245) \citet{2011GCN..11978...1D};
(246) \citet{2011GCN..11993...1D};
(247) \citet{2011GCN..12164...1P};
(248) \citet{2011GCN..12190...1Z};
(249) \citet{2011GCN..12202...1C};
(250) \citet{2011GCN..12225...1T};
(251) \citet{2011GCN..12234...1C};
(252) \citet{2011GCN..12431...1W};
(253) \citet{2011GCN..12537...1C};
(254) \citet{2011GCN..12676...1G};
(255) \citet{2011GCN..12677...1V};
(256) \citet{2011GCN..12777...1C};
(257) \citet{2011MNRAS.411.2792S};
(258) \citet{2011MNRAS.413.2173G};
(259) \citet{2012ApJ...752...62J};
(260) \citet{2012ApJ...756..187H};
(261) \citet{2012ApJ...758...46K};
(262) \citet{2012ApJ...758..122P};
(263) \citet{2012GCN..13051...1D};
(264) \citet{2012GCN..13118...1T};
(265) \citet{2012GCN..13134...1K};
(266) \citet{2012GCN..13213...1C};
(267) \citet{2012GCN..13441...1T};
(268) \citet{2012GCN..13460...1X};
(269) \citet{2012GCN..13493...1G};
(270) \citet{2012GCN..13498...1D};
(271) \citet{2012GCN..13512...1C};
(272) \citet{2012GCN..13532...1T};
(273) \citet{2012GCN..13562...1T};
(274) \citet{2012GCN..13628...1T};
(275) \citet{2012GCN..13723...1S};
(276) \citet{2012GCN..13730...1H};
(277) \citet{2012GCN..13810...1K};
(278) \citet{2012GCN..14009...1T};
(279) \citet{2012GCN..14059...1P};
(280) \citet{2012GCN..14120...1F};
(281) \citet{2012GCN..14123...1K};
(282) \citet{2012MNRAS.421...25S};
(283) \citet{2012arXiv1205.3779M};
(284) \citet{2013A&A...556A..23E};
(285) \citet{2013A&A...557L..18D};
(286) \citet{2013ApJ...766...30G};
(287) \citet{2013ApJ...769...56F};
(288) \citet{2013ApJ...774...26C};
(289) \citet{2013ApJ...775L...5K};
(290) \citet{2013ApJ...776...98X};
(291) \citet{2013ApJ...778..128P};
(292) \citet{2013GCN..14207...1C};
(293) \citet{2013GCN..14286...1F};
(294) \citet{2013GCN..14366...1T};
(295) \citet{2013GCN..14390...1K};
(296) \citet{2013GCN..14437...1D};
(297) \citet{2013GCN..14493...1F};
(298) \citet{2013GCN..14567...1T};
(299) \citet{2013GCN..14621...1C};
(300) \citet{2013GCN..14634...1S};
(301) \citet{2013GCN..14674...1S};
(302) \citet{2013GCN..14685...1S};
(303) \citet{2013GCN..14748...1C};
(304) \citet{2013GCN..14762...1C};
(305) \citet{2013GCN..14848...1S};
(306) \citet{2013GCN..14882...1T};
(307) \citet{2013GCN..14972...1A};
(308) \citet{2013GCN..15144...1C};
(309) \citet{2013GCN..15187...1D};
(310) \citet{2013GCN..15307...1C};
(311) \citet{2013GCN..15330...1R};
(312) \citet{2013GCN..15331...1J};
(313) \citet{2013GCN..15407...1X};
(314) \citet{2013GCN..15470...1D};
(315) \citet{2013GCN..15477...1Y};
(316) \citet{2013GCN..15494...1H};
(317) \citet{2013GCN..15571...1G};
(318) \citet{2013GCN..15624...1C};
(319) \citet{2014A&A...568A..75G};
(320) \citet{2014A&A...569A..93J};
(321) \citet{2014A&A...572A..47R};
(322) \citet{2014ApJ...781....1L};
(323) \citet{2014ApJ...781...13L};
(324) \citet{2014ApJS..211...13V};
(325) \citet{2014GCN..15644...1J};
(326) \citet{2014GCN..15652...1C};
(327) \citet{2014GCN..15800...1M};
(328) \citet{2014GCN..15936...1J};
(329) \citet{2014GCN..15966...1C};
(330) \citet{2014GCN..16125...1T};
(331) \citet{2014GCN..16150...1T};
(332) \citet{2014GCN..16181...1P};
(333) \citet{2014GCN..16224...1H};
(334) \citet{2014GCN..16229...1M};
(335) \citet{2014GCN..16241...1M};
(336) \citet{2014GCN..16269...1C};
(337) \citet{2014GCN..16301...1C};
(338) \citet{2014GCN..16310...1D};
(339) \citet{2014GCN..16363...1B};
(340) \citet{2014MNRAS.440.1810M};
(341) \citet{2014MNRAS.442.2586V};
(342) \citet{2015A&A...581A.125K};
(343) \citet{2015ApJ...803L..24C};
(344) \citet{2015ApJ...805...89L};
(345) \citet{2015GCN..17988...1J-1};
(346) \citet{2015MNRAS.446.3911S};
(347) \citet{2015MNRAS.446.4116V};
(348) \citet{2015MNRAS.452..824K};
(349) \citet{2015MNRAS.452.1535C};
(350) \citet{2015arXiv150402482P};
(351) \citet{GRBtable};
(352) \citet{GRBtablez};
(353) \citet{Greiner};
(354) \citet{Keck GRB Host project};
(355) \citet{Keck GRB Host project:};
(356) \citet{Swift GRB Table};
(357) \citet{sakamoto2011};
}
\end{deluxetable}


==> tbprompt2.tex <==
\begin{deluxetable}{llclcllllllll}
\tabletypesize{\scriptsize}
\setlength{\voffset}{10mm}
%%\tabcolsep0.1in\footnotesize
\tablecolumns{10}
\tablewidth{0pc}
\tablecaption{prompt \label{tbprompt2}}
\tablehead {
\colhead{GRB}        &
\colhead{z} &
\colhead{Method}      &
\colhead{ref}      &
\colhead{Instrument} &
\colhead{$T_{90}$} &
\colhead{ref}      &
\colhead{$E_{\gamma, \rm iso}$}      &
\colhead{$L_{\rm p,iso}$}      &
\colhead{$f$} &
\colhead{$f_{\rm eff}$} &\\

\colhead{}        &
\colhead{} &
\colhead{}      &
\colhead{}      &
\colhead{$T_{90}$} &
\colhead{s} &
\colhead{}      &
\colhead{${\rm erg\ cm^{-2}}$ }      &
\colhead{${\rm erg\ s^{-1}\ cm^{-2}}$}      &
\colhead{} &
\colhead{} &\\

}

\startdata

140606B& $0.384$ & E & $292$ & Fermi & $23.6$ & $34$ & $4.60\times 10^{51}$ & $1.88\times 10^{51}$ & $...$ & $...$ \\
140518A& $4.707$ & A & $284$ & Swift & $60.5$ & $37$ & $3.04\times 10^{53}$ & $1.60\times 10^{53}$ & $...$ & $...$ \\
140515A& $6.320$ & A & $283$ & Swift & $23.4$ & $37$ & $2.27\times 10^{53}$ & $2.33\times 10^{53}$ & $...$ & $...$ \\
140512A& $0.725$ & A & $285$ & Swift & $154.8$ & $37$ & $5.63\times 10^{52}$ & $6.71\times 10^{51}$ & $...$ & $...$ \\
140509A& $2.400$ & P & $282$ & Swift & $23.20$ & $37$ & $4.37\times 10^{52}$ & $1.63\times 10^{52}$ & $...$ & $...$ \\
140508A& $1.027$ & A & $281$ & Fermi & $44.3$ & $33$ & $2.26\times 10^{53}$ & $6.74\times 10^{52}$ & $...$ & $...$ \\
140506A& $0.889$ & E & $287$ & Swift & $111.1$ & $37$ & $1.83\times 10^{52}$ & $1.01\times 10^{52}$ & $...$ & $...$ \\
140430A& $1.602$ & E & $287$ & Swift & $173.6$ & $37$ & $1.51\times 10^{52}$ & $5.73\times 10^{51}$ & $...$ & $...$ \\
140428A& $4.700$ & A & $280$ & Swift & $17.42$ & $37$ & $3.69\times 10^{52}$ & $3.10\times 10^{52}$ & $...$ & $...$ \\
140423A& $3.260$ & A & $279$ & Swift & $134$ & $37$ & $5.45\times 10^{53}$ & $6.19\times 10^{52}$ & $...$ & $...$ \\
140419A& $3.956$ & A & $278$ & Swift & $94.7$ & $37$ & $1.43\times 10^{54}$ & $5.73\times 10^{53}$ & $...$ & $...$ \\
140318A& $1.020$ & E & $289$ & Swift & $8.43$ & $37$ & $3.49\times 10^{51}$ & $1.07\times 10^{51}$ & $...$ & $...$ \\
140311A& $4.954$ & A & $277$ & Swift & $71.4$ & $37$ & $2.28\times 10^{53}$ & $6.10\times 10^{52}$ & $...$ & $...$ \\
140304A& $5.283$ & A & $276$ & Swift & $15.6$ & $37$ & $1.28\times 10^{53}$ & $1.04\times 10^{53}$ & $...$ & $...$ \\
140301A& $1.415$ & E & $287$ & Swift & $31.0$ & $37$ & $4.82\times 10^{51}$ & $1.22\times 10^{51}$ & $...$ & $...$ \\
140226A& $1.980$ & A & $288$ & ... & $...$ & $...$ & $4.81\times 10^{52}$ & $2.20\times 10^{52}$ & $...$ & $...$ \\
140213A& $1.208$ & E & $287$ & Swift & $60.0$ & $37$ & $1.05\times 10^{53}$ & $3.70\times 10^{52}$ & $...$ & $...$ \\
140206A& $2.739$ & A & $275$ & Swift & $93.6$ & $37$ & $3.00\times 10^{53}$ & $1.86\times 10^{53}$ & $...$ & $...$ \\
140114A& $3.000$ & A & $287$ & Swift & $139.7$ & $37$ & $1.28\times 10^{53}$ & $8.96\times 10^{51}$ & $...$ & $...$ \\
131231A& $0.642$ & E & $274$ & Fermi & $31$ & $32$ & $2.21\times 10^{53}$ & $2.17\times 10^{52}$ & $...$ & $...$ \\
131227A& $5.300$ & A & $268$ & Swift & $18.0$ & $37$ & $1.42\times 10^{53}$ & $1.03\times 10^{53}$ & $...$ & $...$ \\
131117A& $4.042$ & A & $266$ & Swift & $11.00$ & $37$ & $1.13\times 10^{53}$ & $1.50\times 10^{53}$ & $...$ & $...$ \\
131108A& $2.400$ & A & $265$ & Fermi & $19$ & $29$ & $5.95\times 10^{53}$ & $2.14\times 10^{53}$ & $...$ & $...$ \\
131105A& $1.685$ & E & $287$ & Swift & $112.3$ & $37$ & $2.21\times 10^{53}$ & $2.72\times 10^{52}$ & $...$ & $...$ \\
131103A& $0.596$ & E & $287$ & Swift & $17.3$ & $37$ & $1.65\times 10^{51}$ & $3.17\times 10^{50}$ & $...$ & $...$ \\
131030A& $1.293$ & A & $264$ & Swift & $41.1$ & $37$ & $2.97\times 10^{53}$ & $1.03\times 10^{53}$ & $...$ & $...$ \\
131011A& $1.874$ & A & $263$ & Fermi & $77$ & $28$ & $1.05\times 10^{53}$ & $1.59\times 10^{52}$ & $...$ & $...$ \\
131004A& $0.717$ & E & $262$ & Swift & $1.54$ & $37$ & $8.01\times 10^{50}$ & $1.48\times 10^{51}$ & $...$ & $...$ \\
130925A& $0.348$ & E & $287$ & Swift & $7000$ & $30$ & $3.21\times 10^{50}$ & $8.56\times 10^{49}$ & $...$ & $...$ \\
130907A& $1.238$ & A & $261$ & Swift & $360$ & $37$ & $2.98\times 10^{54}$ & $1.86\times 10^{53}$ & $...$ & $...$ \\
130831A& $0.479$ & A & $260$ & Swift & $32.5$ & $37$ & $6.63\times 10^{51}$ & $3.23\times 10^{51}$ & $...$ & $...$ \\
130702A& $0.145$ & E & $243$ & Fermi & $59$ & $27$ & $5.05\times 10^{50}$ & $3.15\times 10^{49}$ & $...$ & $...$ \\
130701A& $1.155$ & E & $287$ & Swift & $4.38$ & $37$ & $2.22\times 10^{52}$ & $3.55\times 10^{52}$ & $...$ & $...$ \\
130612A& $2.006$ & A & $259$ & Swift & $4.0$ & $37$ & $9.11\times 10^{51}$ & $9.28\times 10^{51}$ & $...$ & $...$ \\
130610A& $2.092$ & A & $258$ & Swift & $46.4$ & $37$ & $5.20\times 10^{52}$ & $1.33\times 10^{52}$ & $...$ & $...$ \\
130606A& $5.913$ & A & $242$ & Swift & $276.58$ & $37$ & $2.02\times 10^{53}$ & $2.52\times 10^{53}$ & $...$ & $...$ \\
130604A& $1.060$ & E & $257$ & Swift & $37.7$ & $37$ & $1.35\times 10^{52}$ & $1.34\times 10^{51}$ & $...$ & $...$ \\
130528A& $1.250$ & E & $270$ & Swift & $59.4$ & $37$ & $5.31\times 10^{52}$ & $6.09\times 10^{51}$ & $...$ & $...$ \\
130518A& $2.490$ & A & $255$ & Fermi & $48$ & $26$ & $1.78\times 10^{54}$ & $6.01\times 10^{53}$ & $...$ & $...$ \\
130514A& $3.600$ & P & $254$ & Swift & $204$ & $37$ & $5.71\times 10^{53}$ & $5.61\times 10^{52}$ & $...$ & $...$ \\
130511A& $1.303$ & A & $253$ & Swift & $5.43$ & $37$ & $4.18\times 10^{51}$ & $5.01\times 10^{51}$ & $...$ & $...$ \\
130505A& $2.270$ & A & $252$ & Swift & $88$ & $37$ & $5.49\times 10^{54}$ & $1.99\times 10^{54}$ & $...$ & $...$ \\
130427B& $2.780$ & A & $251$ & Swift & $27.0$ & $37$ & $6.49\times 10^{52}$ & $3.95\times 10^{52}$ & $...$ & $...$ \\
130427A& $0.340$ & E & $244$ & Swift & $162.83$ & $37$ & $1.17\times 10^{54}$ & $1.84\times 10^{53}$ & $...$ & $...$ \\
130420A& $1.297$ & A & $250$ & Swift & $123.5$ & $37$ & $6.54\times 10^{52}$ & $5.43\times 10^{51}$ & $...$ & $...$ \\
130418A& $1.217$ & A & $249$ & Swift & $300$ & $37$ & $9.34\times 10^{52}$ & $3.30\times 10^{51}$ & $...$ & $...$ \\
130408A& $3.757$ & A & $248$ & Swift & $28$ & $37$ & $2.80\times 10^{53}$ & $5.77\times 10^{53}$ & $...$ & $...$ \\
130215A& $0.597$ & A & $246$ & Swift & $65.7$ & $37$ & $4.17\times 10^{52}$ & $2.13\times 10^{51}$ & $...$ & $...$ \\
130131B& $2.539$ & E & $247$ & Swift & $4.30$ & $37$ & $2.98\times 10^{52}$ & $2.81\times 10^{52}$ & $...$ & $...$ \\
121229A& $2.707$ & A & $237$ & Swift & $100$ & $24$ & $1.97\times 10^{52}$ & $8.70\times 10^{50}$ & $...$ & $...$ \\
121212A& $...$ & ... & $...$ & Swift & $6.8$ & $37$ & $3.79\times 10^{51}$ & $3.63\times 10^{51}$ & $...$ & $...$ \\
121211A& $1.023$ & A & $236$ & Swift & $182$ & $37$ & $2.18\times 10^{51}$ & $2.06\times 10^{51}$ & $...$ & $...$ \\
121209A& $2.100$ & A & $287$ & Swift & $42.7$ & $37$ & $1.09\times 10^{53}$ & $3.44\times 10^{52}$ & $...$ & $...$ \\
121201A& $3.383$ & E & $287$ & Swift & $85$ & $37$ & $3.81\times 10^{52}$ & $1.18\times 10^{52}$ & $...$ & $...$ \\
121128A& $2.200$ & A & $235$ & Swift & $23.3$ & $37$ & $1.21\times 10^{53}$ & $5.33\times 10^{52}$ & $...$ & $...$ \\
121027A& $1.773$ & E & $287$ & Swift & $62.6$ & $37$ & $3.46\times 10^{52}$ & $4.54\times 10^{51}$ & $...$ & $...$ \\
121024A& $2.301$ & E & $287$ & Swift & $69$ & $37$ & $5.00\times 10^{52}$ & $1.70\times 10^{52}$ & $...$ & $...$ \\
120922A& $3.100$ & P & $234$ & Swift & $173$ & $37$ & $2.06\times 10^{53}$ & $2.56\times 10^{52}$ & $...$ & $...$ \\
120909A& $3.930$ & A & $233$ & Fermi & $112$ & $1$ & $3.78\times 10^{53}$ & $9.46\times 10^{52}$ & $...$ & $...$ \\
120907A& $0.970$ & A & $232$ & Swift & $16.9$ & $37$ & $2.55\times 10^{51}$ & $3.14\times 10^{51}$ & $...$ & $...$ \\
120815A& $2.359$ & E & $287$ & Swift & $9.7$ & $37$ & $1.47\times 10^{52}$ & $1.24\times 10^{52}$ & $...$ & $...$ \\
120811C& $2.671$ & A & $231$ & Swift & $26.8$ & $37$ & $6.24\times 10^{52}$ & $3.45\times 10^{52}$ & $...$ & $...$ \\
120805A& $3.100$ & A & $287$ & Swift & $48.00$ & $37$ & $8.82\times 10^{52}$ & $1.47\times 10^{52}$ & $...$ & $...$ \\
120802A& $3.796$ & A & $230$ & Swift & $50$ & $37$ & $2.68\times 10^{53}$ & $1.83\times 10^{53}$ & $...$ & $...$ \\
120729A& $0.800$ & A & $229$ & Swift & $71.5$ & $37$ & $1.89\times 10^{52}$ & $5.87\times 10^{51}$ & $...$ & $...$ \\
120724A& $1.480$ & A & $228$ & Swift & $72.8$ & $37$ & $7.51\times 10^{52}$ & $1.53\times 10^{52}$ & $...$ & $...$ \\
120722A& $0.959$ & E & $287$ & Swift & $42.4$ & $37$ & $6.37\times 10^{51}$ & $7.16\times 10^{50}$ & $...$ & $...$ \\
120716A& $2.486$ & A & $227$ & Fermi & $234$ & $23$ & $2.91\times 10^{53}$ & $7.96\times 10^{52}$ & $...$ & $...$ \\
120714B& $0.399$ & E & $287$ & Swift & $159$ & $37$ & $1.61\times 10^{51}$ & $6.33\times 10^{49}$ & $...$ & $...$ \\
120712A& $4.175$ & A & $226$ & Swift & $14.7$ & $37$ & $1.76\times 10^{53}$ & $1.27\times 10^{53}$ & $...$ & $...$ \\
120711A& $1.405$ & A & $225$ & Fermi & $44.033$ & $31$ & $1.82\times 10^{54}$ & $1.71\times 10^{53}$ & $...$ & $...$ \\
120624B& $2.197$ & E & $240$ & Swift & $192$ & $37$ & $3.21\times 10^{54}$ & $2.32\times 10^{53}$ & $...$ & $...$ \\
120521C& $6.000$ & P & $272$ & Swift & $26.7$ & $37$ & $1.35\times 10^{53}$ & $1.25\times 10^{53}$ & $...$ & $...$ \\
120422A& $0.283$ & E & $287$ & Swift & $5.35$ & $37$ & $2.97\times 10^{50}$ & $8.97\times 10^{49}$ & $...$ & $...$ \\
120404A& $2.876$ & A & $224$ & Swift & $38.7$ & $37$ & $6.16\times 10^{52}$ & $1.28\times 10^{52}$ & $...$ & $...$ \\
120327A& $2.813$ & A & $223$ & Swift & $62.9$ & $37$ & $1.88\times 10^{53}$ & $6.53\times 10^{52}$ & $...$ & $...$ \\
120326A& $1.798$ & A & $222$ & Swift & $69.6$ & $37$ & $3.19\times 10^{52}$ & $1.55\times 10^{52}$ & $...$ & $...$ \\
120311A& $3.000$ & P & $221$ & Swift & $3.5$ & $37$ & $1.35\times 10^{52}$ & $3.22\times 10^{52}$ & $...$ & $...$ \\
120308A& $4.500$ & P & $293$ & Swift & $60.6$ & $37$ & $1.00\times 10^{53}$ & $2.14\times 10^{53}$ & $...$ & $...$ \\
120224A& $1.100$ & A & $287$ & Swift & $8.13$ & $37$ & $1.75\times 10^{51}$ & $7.79\times 10^{50}$ & $...$ & $...$ \\
120211A& $2.400$ & A & $287$ & Swift & $61.7$ & $37$ & $3.38\times 10^{52}$ & $6.02\times 10^{51}$ & $...$ & $...$ \\
120119A& $1.729$ & E & $287$ & Swift & $253.8$ & $37$ & $3.56\times 10^{53}$ & $5.64\times 10^{52}$ & $...$ & $...$ \\
120118B& $2.943$ & E & $287$ & Swift & $23.26$ & $37$ & $5.65\times 10^{52}$ & $1.61\times 10^{52}$ & $...$ & $...$ \\
111229A& $1.381$ & A & $215$ & Swift & $25.4$ & $37$ & $3.68\times 10^{51}$ & $1.84\times 10^{51}$ & $    1.17$ & $1.13\pm0.43$ \\
111228A& $0.716$ & E & $287$ & Swift & $101.20$ & $37$ & $3.91\times 10^{52}$ & $4.27\times 10^{51}$ & $    1.62$ & $1.30\pm0.19$ \\
111225A& $2.012$ & E & $291$ & Swift & $106.8$ & $37$ & $3.08\times 10^{52}$ & $3.91\times 10^{51}$ & $    1.16$ & $1.13\pm0.16$ \\
111215A& $2.060$ & P & $291$ & Swift & $796$ & $37$ & $1.11\times 10^{53}$ & $2.95\times 10^{51}$ & $...$ & $...$ \\
111211A& $0.478$ & A & $214$ & Konus-Wind & $25$ & $22$ & $...$ & $...$ & $...$ & $...$ \\
111209A& $0.677$ & E & $273$ & Swift & $25000$ & $25$ & $8.03\times 10^{53}$ & $2.82\times 10^{50}$ & $...$ & $...$ \\
111129A& $1.080$ & E & $287$ & Swift & $7.6$ & $37$ & $1.65\times 10^{51}$ & $9.40\times 10^{50}$ & $    1.10$ & $1.10\pm0.12$ \\
111123A& $3.151$ & E & $287$ & Swift & $290.0$ & $37$ & $3.68\times 10^{53}$ & $1.49\times 10^{52}$ & $    1.17$ & $1.13\pm0.16$ \\
111107A& $2.893$ & A & $213$ & Swift & $26.6$ & $37$ & $2.05\times 10^{52}$ & $2.95\times 10^{52}$ & $    1.21$ & $1.15\pm0.23$ \\
111008A& $4.990$ & A & $212$ & Swift & $63.46$ & $37$ & $3.93\times 10^{53}$ & $3.66\times 10^{53}$ & $    1.52$ & $1.27\pm0.03$ \\
111005A& $0.013$ & ... & $211$ & Swift & $26$ & $37$ & $5.39\times 10^{47}$ & $6.12\times 10^{46}$ & $    1.24$ & $1.16\pm0.07$ \\
110918A& $0.982$ & E & $239$ & ... & $...$ & $...$ & $1.83\times 10^{54}$ & $4.20\times 10^{54}$ & $...$ & $...$ \\
110818A& $3.361$ & E & $287$ & Swift & $103$ & $37$ & $1.71\times 10^{53}$ & $6.05\times 10^{52}$ & $    1.26$ & $1.17\pm0.14$ \\
110808A& $1.349$ & E & $287$ & Swift & $48$ & $37$ & $5.74\times 10^{52}$ & $9.27\times 10^{53}$ & $    1.05$ & $1.08\pm0.11$ \\
110801A& $1.858$ & A & $210$ & Swift & $385$ & $37$ & $9.65\times 10^{52}$ & $5.09\times 10^{51}$ & $    1.09$ & $1.10\pm0.24$ \\
110731A& $2.830$ & A & $209$ & Swift & $38.8$ & $37$ & $4.91\times 10^{53}$ & $3.16\times 10^{53}$ & $    3.50$ & $1.25\pm0.29$ \\
110726A& $1.036$ & A & $208$ & Swift & $5.2$ & $37$ & $1.16\times 10^{52}$ & $1.00\times 10^{52}$ & $    1.25$ & $1.17\pm0.07$ \\
110715A& $0.820$ & A & $207$ & Swift & $13.0$ & $37$ & $4.81\times 10^{52}$ & $4.18\times 10^{52}$ & $    9.70$ & $1.15\pm0.01$ \\
110709B& $2.090$ & E & $293$ & Swift & $55.6$ & $37$ & $2.69\times 10^{53}$ & $3.52\times 10^{53}$ & $    1.52$ & $1.27\pm0.21$ \\
110503A& $1.613$ & A & $206$ & Swift & $10.0$ & $37$ & $1.80\times 10^{53}$ & $1.99\times 10^{53}$ & $    3.12$ & $1.28\pm0.12$ \\
110422A& $1.770$ & A & $205$ & Swift & $25.9$ & $37$ & $7.20\times 10^{53}$ & $2.80\times 10^{53}$ & $    4.00$ & $1.29\pm0.16$ \\
110213B& $1.083$ & A & $204$ & Konus-Wind & $50$ & $21$ & $8.08\times 10^{52}$ & $...$ & $...$ & $...$ \\
110213A& $1.460$ & A & $203$ & Swift & $48.0$ & $37$ & $7.34\times 10^{52}$ & $2.90\times 10^{52}$ & $    1.35$ & $1.21\pm0.27$ \\
110205A& $2.220$ & A & $202$ & Swift & $257$ & $37$ & $6.10\times 10^{53}$ & $2.74\times 10^{52}$ & $    1.54$ & $1.27\pm0.11$ \\
110128A& $2.339$ & A & $201$ & Swift & $30.7$ & $37$ & $2.31\times 10^{52}$ & $9.70\times 10^{51}$ & $    1.12$ & $1.11\pm0.29$ \\
110106B& $0.618$ & E & $200$ & Swift & $24.8$ & $37$ & $5.34\times 10^{51}$ & $6.68\times 10^{50}$ & $    1.15$ & $1.12\pm0.01$ \\
101225A& $0.847$ & E & $273$ & Swift & $1088.0$ & $37$ & $8.21\times 10^{51}$ & $...$ & $...$ & $...$ \\
101219B& $0.552$ & A & $197$ & Swift & $34$ & $37$ & $4.47\times 10^{51}$ & $2.59\times 10^{50}$ & $...$ & $...$ \\
100906A& $1.727$ & A & $189$ & Swift & $114.4$ & $37$ & $2.61\times 10^{53}$ & $5.18\times 10^{52}$ & $    2.35$ & $1.47\pm0.05$ \\
100901A& $1.408$ & A & $188$ & Swift & $439$ & $37$ & $3.38\times 10^{52}$ & $2.61\times 10^{51}$ & $    1.10$ & $1.10\pm0.2$ \\
100814A& $1.439$ & E & $287$ & Swift & $174.5$ & $37$ & $9.39\times 10^{52}$ & $1.00\times 10^{52}$ & $    1.75$ & $1.34\pm0.07$ \\
100802A& $3.500$ & E & $293$ & Swift & $487$ & $37$ & $5.03\times 10^{52}$ & $2.21\times 10^{52}$ & $    1.24$ & $1.16\pm0.27$ \\
100728B& $2.106$ & A & $190$ & Swift & $12.1$ & $37$ & $4.86\times 10^{52}$ & $3.65\times 10^{52}$ & $    1.25$ & $1.17\pm0.09$ \\
100728A& $1.567$ & E & $287$ & Swift & $198.5$ & $37$ & $9.47\times 10^{53}$ & $3.92\times 10^{52}$ & $    2.37$ & $1.48\pm0.38$ \\
100724A& $1.289$ & E & $287$ & Swift & $1.4$ & $37$ & $1.49\times 10^{51}$ & $2.74\times 10^{51}$ & $    1.38$ & $1.38\pm0.21$ \\
100621A& $0.543$ & E & $287$ & Swift & $63.6$ & $37$ & $4.39\times 10^{52}$ & $3.20\times 10^{51}$ & $    4.11$ & $1.21\pm0.11$ \\
100615A& $1.398$ & E & $287$ & Swift & $39$ & $37$ & $7.15\times 10^{52}$ & $1.88\times 10^{52}$ & $    1.87$ & $1.37\pm0.21$ \\
100606A& $1.554$ & E & $287$ & Swift & $480$ & $37$ & $2.94\times 10^{53}$ & $4.82\times 10^{52}$ & $    1.75$ & $1.34\pm0.14$ \\
100518A& $4.000$ & P & $187$ & ... & $...$ & $...$ & $5.52\times 10^{52}$ & $4.24\times 10^{52}$ & $...$ & $...$ \\
100513A& $4.772$ & A & $186$ & Swift & $84$ & $37$ & $1.40\times 10^{53}$ & $2.80\times 10^{52}$ & $    1.15$ & $1.12\pm0.16$ \\
100508A& $0.520$ & E & $287$ & Swift & $52$ & $37$ & $2.87\times 10^{51}$ & $2.24\times 10^{50}$ & $...$ & $...$ \\
100425A& $1.755$ & A & $185$ & Swift & $37.0$ & $37$ & $9.42\times 10^{51}$ & $4.23\times 10^{51}$ & $    1.18$ & $1.13\pm0.34$ \\
100424A& $2.466$ & E & $287$ & Swift & $104$ & $37$ & $4.54\times 10^{52}$ & $3.03\times 10^{51}$ & $...$ & $...$ \\
100418A& $0.624$ & E & $287$ & Swift & $7.0$ & $37$ & $7.66\times 10^{50}$ & $2.15\times 10^{50}$ & $    1.12$ & $1.11\pm0.12$ \\
100414A& $1.368$ & A & $184$ & Fermi & $26.497$ & $31$ & $5.63\times 10^{53}$ & $3.30\times 10^{52}$ & $...$ & $...$ \\
100316D& $0.059$ & E & $216$ & Swift & $1300$ & $19$ & $5.72\times 10^{48}$ & $1.13\times 10^{47}$ & $...$ & $...$ \\
100316B& $1.180$ & A & $183$ & Swift & $3.8$ & $37$ & $1.65\times 10^{51}$ & $1.33\times 10^{51}$ & $    1.31$ & $1.19\pm0.12$ \\
100302A& $4.813$ & A & $182$ & Swift & $17.9$ & $37$ & $2.82\times 10^{52}$ & $2.04\times 10^{52}$ & $    1.25$ & $1.17\pm0.34$ \\
100219A& $4.667$ & A & $181$ & Swift & $18.8$ & $37$ & $5.48\times 10^{52}$ & $2.96\times 10^{52}$ & $    1.17$ & $1.13\pm0.1$ \\
091208B& $1.063$ & A & $154$ & Swift & $14.80$ & $20$ & $2.81\times 10^{52}$ & $2.03\times 10^{52}$ & $    1.81$ & $1.52\pm0.16$ \\
091127A& $0.490$ & E & $287$ & Swift & $7.42$ & $20$ & $1.86\times 10^{52}$ & $6.24\times 10^{51}$ & $    2.25$ & $1.70\pm0.03$ \\
091109A& $3.076$ & A & $180$ & Swift & $48.03$ & $20$ & $1.42\times 10^{54}$ & $3.52\times 10^{53}$ & $...$ & $...$ \\
091029A& $2.752$ & A & $153$ & Swift & $39.18$ & $20$ & $1.33\times 10^{53}$ & $3.22\times 10^{52}$ & $...$ & $...$ \\
091024A& $1.092$ & A & $152$ & Swift & $112.28$ & $20$ & $5.15\times 10^{52}$ & $1.01\times 10^{52}$ & $...$ & $...$ \\
091020A& $1.710$ & A & $151$ & Swift & $38.92$ & $20$ & $6.85\times 10^{52}$ & $1.81\times 10^{52}$ & $    1.60$ & $1.09\pm0.06$ \\
091018A& $0.971$ & E & $287$ & Swift & $4.37$ & $20$ & $7.07\times 10^{51}$ & $4.18\times 10^{51}$ & $    2.31$ & $1.39\pm0.12$ \\
091003A& $0.897$ & E & $150$ & Fermi & $20.224$ & $31$ & $7.17\times 10^{52}$ & $2.93\times 10^{52}$ & $...$ & $...$ \\
090927A& $1.370$ & A & $173$ & Swift & $2.16$ & $20$ & $1.83\times 10^{51}$ & $4.59\times 10^{51}$ & $    1.48$ & $...$ \\
090926B& $1.243$ & E & $287$ & Swift & $99.28$ & $20$ & $4.48\times 10^{52}$ & $3.89\times 10^{51}$ & $    1.50$ & $1.10\pm0.05$ \\
090926A& $2.106$ & E & $178$ & Fermi & $13.760$ & $31$ & $1.98\times 10^{54}$ & $6.55\times 10^{53}$ & $...$ & $...$ \\
090902B& $1.822$ & A & $172$ & Fermi & $19.328$ & $31$ & $3.05\times 10^{54}$ & $7.80\times 10^{53}$ & $...$ & $...$ \\
090814A& $0.696$ & A & $171$ & Swift & $78.22$ & $20$ & $3.68\times 10^{52}$ & $2.10\times 10^{51}$ & $...$ & $...$ \\
090812A& $2.452$ & A & $170$ & Swift & $75.09$ & $20$ & $4.45\times 10^{53}$ & $8.14\times 10^{52}$ & $    1.50$ & $1.11\pm0.1$ \\
090809A& $2.737$ & A & $169$ & Swift & $7.84$ & $20$ & $2.45\times 10^{53}$ & $2.16\times 10^{53}$ & $    1.30$ & $...$ \\
090726A& $2.710$ & A & $168$ & Swift & $56.68$ & $20$ & $3.17\times 10^{52}$ & $5.41\times 10^{51}$ & $...$ & $...$ \\
090715B& $3.000$ & A & $167$ & Swift & $265.39$ & $20$ & $2.10\times 10^{53}$ & $8.12\times 10^{52}$ & $    1.56$ & $1.09\pm0.07$ \\
090709A& $0.403$ & E & $179$ & Swift & $88.73$ & $20$ & $4.09\times 10^{52}$ & $2.46\times 10^{51}$ & $    2.50$ & $1.27\pm0.03$ \\
090618A& $0.540$ & A & $166$ & Swift & $113.34$ & $20$ & $2.80\times 10^{53}$ & $1.26\times 10^{52}$ & $    7.50$ & $1.23\pm0.03$ \\
090530A& $1.266$ & A & $267$ & Swift & $40.46$ & $20$ & $1.27\times 10^{52}$ & $5.33\times 10^{51}$ & $    1.50$ & $1.31\pm0.09$ \\
090529A& $2.625$ & A & $165$ & Swift & $70$ & $20$ & $2.19\times 10^{52}$ & $3.00\times 10^{51}$ & $...$ & $...$ \\
090519A& $3.850$ & A & $164$ & Swift & $58.26$ & $20$ & $2.66\times 10^{53}$ & $1.03\times 10^{53}$ & $...$ & $...$ \\
090516A& $4.109$ & A & $163$ & Swift & $208.00$ & $20$ & $7.31\times 10^{53}$ & $8.66\times 10^{52}$ & $...$ & $...$ \\
090429B& $9.200$ & P & $198$ & Swift & $5.61$ & $20$ & $6.08\times 10^{53}$ & $1.94\times 10^{54}$ & $    1.33$ & $1.25\pm0.12$ \\
090424A& $0.544$ & E & $160$ & Swift & $49.47$ & $20$ & $4.14\times 10^{52}$ & $1.65\times 10^{52}$ & $   11.25$ & $1.18\pm0.11$ \\
090423A& $8.230$ & A & $176$ & Swift & $9.77$ & $20$ & $7.89\times 10^{52}$ & $1.14\times 10^{53}$ & $    1.31$ & $1.22\pm0.11$ \\
090418A& $1.608$ & A & $158$ & Swift & $56.31$ & $20$ & $1.62\times 10^{53}$ & $1.24\times 10^{53}$ & $...$ & $...$ \\
090417B& $0.345$ & E & $159$ & Swift & $282.49$ & $20$ & $1.57\times 10^{52}$ & $1.70\times 10^{50}$ & $...$ & $...$ \\
090407A& $1.448$ & E & $219$ & Swift & $315.44$ & $20$ & $1.42\times 10^{52}$ & $1.45\times 10^{51}$ & $    1.14$ & $1.07\pm0.07$ \\
090328A& $0.736$ & E & $196$ & Fermi & $61.697$ & $31$ & $9.23\times 10^{52}$ & $1.36\times 10^{52}$ & $...$ & $...$ \\
090323A& $3.568$ & A & $196$ & Fermi & $135.170$ & $31$ & $3.94\times 10^{54}$ & $3.21\times 10^{53}$ & $...$ & $...$ \\
090313A& $3.375$ & A & $157$ & Swift & $70.66$ & $20$ & $6.80\times 10^{52}$ & $1.16\times 10^{52}$ & $...$ & $...$ \\
090205A& $4.650$ & A & $156$ & Swift & $8.80$ & $20$ & $1.54\times 10^{52}$ & $1.35\times 10^{52}$ & $    1.19$ & $...$ \\
090201A& $2.100$ & E & $287$ & Swift & $84.78$ & $20$ & $8.00\times 10^{53}$ & $2.70\times 10^{53}$ & $    2.00$ & $1.20\pm0.14$ \\
090113A& $1.749$ & E & $219$ & Swift & $9.10$ & $20$ & $1.66\times 10^{52}$ & $1.25\times 10^{52}$ & $    1.50$ & $1.19\pm0.16$ \\
090102A& $1.547$ & A & $155$ & Swift & $29.30$ & $20$ & $2.35\times 10^{53}$ & $4.80\times 10^{52}$ & $...$ & $...$ \\
081230A& $2.030$ & P & $193$ & Swift & $66.00$ & $20$ & $1.71\times 10^{52}$ & $2.91\times 10^{51}$ & $...$ & $...$ \\
081228A& $3.440$ & P & $193$ & Swift & $3.00$ & $20$ & $4.48\times 10^{51}$ & $8.12\times 10^{51}$ & $    1.35$ & $1.18\pm0.34$ \\
081222A& $2.770$ & A & $141$ & Swift & $33.00$ & $20$ & $2.40\times 10^{53}$ & $1.22\times 10^{53}$ & $    2.31$ & $1.20\pm0.12$ \\
081221A& $2.259$ & E & $287$ & Swift & $33.91$ & $20$ & $3.95\times 10^{53}$ & $8.30\times 10^{52}$ & $    3.75$ & $1.20\pm0.16$ \\
081210A& $2.063$ & E & $287$ & Swift & $145.91$ & $20$ & $6.71\times 10^{52}$ & $2.47\times 10^{52}$ & $    1.45$ & $1.22\pm0.06$ \\
081203A& $2.050$ & A & $175$ & Swift & $223.00$ & $20$ & $3.38\times 10^{53}$ & $3.27\times 10^{53}$ & $    1.50$ & $1.16\pm0.12$ \\
081128A& $4.000$ & P & $293$ & Swift & $96.77$ & $20$ & $4.42\times 10^{53}$ & $1.14\times 10^{53}$ & $    1.19$ & $1.10\pm0.23$ \\
081121A& $2.512$ & A & $140$ & Swift & $17.67$ & $20$ & $2.84\times 10^{53}$ & $8.65\times 10^{52}$ & $    1.14$ & $1.11\pm0.34$ \\
081118A& $2.580$ & A & $139$ & Swift & $49.28$ & $20$ & $3.80\times 10^{52}$ & $4.12\times 10^{51}$ & $...$ & $...$ \\
081109A& $0.979$ & E & $287$ & Swift & $221.49$ & $20$ & $3.31\times 10^{52}$ & $3.46\times 10^{51}$ & $    1.31$ & $1.07\pm0.1$ \\
081029A& $3.848$ & A & $138$ & Swift & $275.05$ & $20$ & $2.03\times 10^{53}$ & $2.03\times 10^{52}$ & $...$ & $...$ \\
081028A& $3.038$ & A & $137$ & Swift & $284.42$ & $20$ & $3.51\times 10^{53}$ & $1.71\times 10^{52}$ & $...$ & $...$ \\
081008A& $1.967$ & A & $136$ & Swift & $179.52$ & $20$ & $1.30\times 10^{53}$ & $1.33\times 10^{52}$ & $    1.31$ & $1.16\pm0.25$ \\
081007A& $0.529$ & E & $135$ & Swift & $9.01$ & $20$ & $1.48\times 10^{51}$ & $4.53\times 10^{50}$ & $    1.35$ & $1.26\pm0.03$ \\
080928A& $1.692$ & A & $149$ & Swift & $233.66$ & $20$ & $1.37\times 10^{52}$ & $1.02\times 10^{52}$ & $    1.38$ & $1.22\pm0.07$ \\
080916C& $4.350$ & P & $193$ & Fermi & $62.977$ & $31$ & $2.72\times 10^{54}$ & $7.01\times 10^{53}$ & $...$ & $...$ \\
080916A& $0.689$ & A & $149$ & Swift & $61.35$ & $20$ & $1.81\times 10^{52}$ & $2.55\times 10^{51}$ & $    1.50$ & $1.15\pm0.03$ \\
080913A& $6.700$ & A & $149$ & Swift & $7.46$ & $20$ & $6.37\times 10^{52}$ & $1.25\times 10^{53}$ & $    1.26$ & $1.19\pm0.09$ \\
080906A& $2.000$ & P & $134$ & Swift & $148.19$ & $20$ & $9.40\times 10^{52}$ & $6.62\times 10^{51}$ & $    1.24$ & $1.10\pm0.27$ \\
080905B& $2.374$ & A & $149$ & Swift & $101.62$ & $20$ & $4.69\times 10^{52}$ & $1.78\times 10^{52}$ & $    1.26$ & $1.12\pm0.09$ \\
080825B& $4.310$ & P & $193$ & AGILE & $50$ & $16$ & $3.59\times 10^{53}$ & $2.96\times 10^{53}$ & $...$ & $...$ \\
080810A& $3.360$ & A & $149$ & Swift & $107.67$ & $20$ & $3.54\times 10^{53}$ & $1.05\times 10^{53}$ & $...$ & $...$ \\
080805A& $1.505$ & E & $287$ & Swift & $106.62$ & $20$ & $4.46\times 10^{52}$ & $4.13\times 10^{51}$ & $    1.23$ & $1.12\pm0.14$ \\
080804A& $2.206$ & E & $287$ & Swift & $37.19$ & $20$ & $1.55\times 10^{53}$ & $4.29\times 10^{52}$ & $    1.50$ & $1.10\pm0.11$ \\
080721A& $2.591$ & A & $149$ & Swift & $176.29$ & $20$ & $1.20\times 10^{54}$ & $1.00\times 10^{54}$ & $    4.81$ & $1.34\pm0.07$ \\
080710A& $0.845$ & A & $149$ & Swift & $112.06$ & $20$ & $9.34\times 10^{51}$ & $1.05\times 10^{51}$ & $    1.11$ & $1.10\pm0.01$ \\
080707A& $1.232$ & A & $149$ & Swift & $30.17$ & $20$ & $4.79\times 10^{51}$ & $1.54\times 10^{51}$ & $    1.25$ & $1.11\pm0.21$ \\
080703A& $...$ & ... & $...$ & Swift & $3.52$ & $20$ & $5.87\times 10^{51}$ & $7.40\times 10^{51}$ & $...$ & $...$ \\
080607A& $3.037$ & A & $149$ & Swift & $78.86$ & $20$ & $1.76\times 10^{54}$ & $2.13\times 10^{54}$ & $    5.60$ & $1.20\pm0.07$ \\
080605A& $1.641$ & E & $287$ & Swift & $18.05$ & $20$ & $2.31\times 10^{53}$ & $3.24\times 10^{53}$ & $    1.42$ & $1.11\pm0.43$ \\
080604A& $1.417$ & A & $149$ & Swift & $69.16$ & $20$ & $9.49\times 10^{51}$ & $8.55\times 10^{50}$ & $...$ & $...$ \\
080603B& $2.689$ & A & $149$ & Swift & $59.12$ & $20$ & $9.56\times 10^{52}$ & $1.18\times 10^{53}$ & $    1.65$ & $1.11\pm0.19$ \\
080602A& $1.820$ & E & $287$ & Swift & $74.29$ & $20$ & $8.73\times 10^{52}$ & $5.97\times 10^{52}$ & $    1.25$ & $1.07\pm0.16$ \\
080523A& $3.000$ & P & $132$ & Swift & $48.00$ & $20$ & $4.25\times 10^{52}$ & $7.73\times 10^{51}$ & $    1.10$ & $1.07\pm0.29$ \\
080520A& $1.546$ & E & $149$ & Swift & $3.32$ & $20$ & $1.35\times 10^{51}$ & $1.71\times 10^{51}$ & $    1.32$ & $...$ \\
080517A& $0.089$ & E & $290$ & Swift & $64.61$ & $20$ & $3.37\times 10^{49}$ & $3.29\times 10^{48}$ & $...$ & $...$ \\
080515A& $2.470$ & E & $294$ & Swift & $20.91$ & $20$ & $2.52\times 10^{53}$ & $1.57\times 10^{53}$ & $    1.12$ & $1.07\pm0.34$ \\
080514B& $1.800$ & P & $128$ & Suzaku & $6.3$ & $15$ & $2.58\times 10^{53}$ & $4.62\times 10^{53}$ & $...$ & $...$ \\
080430A& $0.767$ & A & $131$ & Swift & $14.15$ & $20$ & $4.57\times 10^{51}$ & $1.34\times 10^{51}$ & $    1.46$ & $1.12\pm0.12$ \\
080413B& $1.101$ & E & $287$ & Swift & $8.00$ & $20$ & $2.37\times 10^{53}$ & $2.15\times 10^{53}$ & $    2.38$ & $1.53\pm0.16$ \\
080413A& $2.433$ & A & $149$ & Swift & $46.36$ & $20$ & $1.74\times 10^{53}$ & $6.00\times 10^{53}$ & $    1.75$ & $1.13\pm0.06$ \\
080411A& $1.030$ & A & $149$ & Swift & $56.33$ & $20$ & $2.35\times 10^{53}$ & $9.71\times 10^{52}$ & $    6.85$ & $1.13\pm0.03$ \\
080330A& $1.512$ & A & $149$ & Swift & $67.05$ & $20$ & $5.77\times 10^{51}$ & $2.10\times 10^{51}$ & $    1.19$ & $1.11\pm0.23$ \\
080325A& $1.780$ & E & $38$ & Swift & $162.82$ & $20$ & $9.60\times 10^{52}$ & $6.02\times 10^{51}$ & $...$ & $...$ \\
080320A& $...$ & ... & $...$ & Swift & $13.82$ & $20$ & $6.34\times 10^{51}$ & $3.30\times 10^{51}$ & $    1.12$ & $1.09\pm0.05$ \\
080319C& $1.949$ & A & $149$ & Swift & $29.55$ & $20$ & $1.36\times 10^{53}$ & $8.98\times 10^{52}$ & $    1.52$ & $1.09\pm0.34$ \\
080319B& $0.938$ & A & $149$ & Swift & $124.86$ & $20$ & $1.33\times 10^{54}$ & $9.80\times 10^{52}$ & $    8.00$ & $1.11\pm0.27$ \\
080319A& $2.430$ & E & $293$ & Swift & $43.62$ & $20$ & $1.77\times 10^{54}$ & $2.24\times 10^{53}$ & $    1.18$ & $1.07\pm0.1$ \\
080310A& $2.427$ & A & $149$ & Swift & $352.37$ & $20$ & $7.43\times 10^{52}$ & $7.97\times 10^{51}$ & $    1.19$ & $1.07\pm0.07$ \\
080307A& $...$ & ... & $...$ & Swift & $122.22$ & $20$ & $1.91\times 10^{52}$ & $1.96\times 10^{51}$ & $...$ & $...$ \\
080212A& $...$ & ... & $...$ & Swift & $117.38$ & $20$ & $5.76\times 10^{53}$ & $6.70\times 10^{52}$ & $...$ & $...$ \\
080210A& $2.642$ & A & $149$ & Swift & $39.36$ & $20$ & $6.33\times 10^{52}$ & $1.54\times 10^{52}$ & $    1.23$ & $1.09\pm0.03$ \\
080207A& $2.086$ & E & $287$ & Swift & $290$ & $20$ & $3.76\times 10^{53}$ & $1.72\times 10^{52}$ & $...$ & $...$ \\
080205A& $2.720$ & P & $293$ & Swift & $104.06$ & $20$ & $7.22\times 10^{52}$ & $1.10\times 10^{52}$ & $    1.19$ & $1.09\pm0.07$ \\
080129A& $4.349$ & A & $147$ & Swift & $50.22$ & $20$ & $1.20\times 10^{53}$ & $1.27\times 10^{52}$ & $...$ & $...$ \\
071122A& $1.140$ & A & $124$ & Swift & $80.00$ & $20$ & $4.62\times 10^{51}$ & $5.11\times 10^{50}$ & $...$ & $...$ \\
071117A& $1.331$ & E & $149$ & Swift & $6.07$ & $20$ & $4.09\times 10^{52}$ & $1.09\times 10^{53}$ & $    2.40$ & $1.44\pm0.16$ \\
071112C& $0.823$ & A & $149$ & Swift & $15$ & $37$ & $4.14\times 10^{52}$ & $1.83\times 10^{52}$ & $...$ & $...$ \\
071031A& $2.692$ & A & $149$ & Swift & $150.49$ & $20$ & $3.79\times 10^{52}$ & $4.25\times 10^{51}$ & $    1.12$ & $1.07\pm0.09$ \\
071025A& $4.800$ & A & $191$ & Swift & $241.30$ & $20$ & $5.61\times 10^{53}$ & $5.93\times 10^{52}$ & $    1.25$ & $1.09\pm0.38$ \\
071021A& $2.451$ & E & $287$ & Swift & $228.72$ & $20$ & $4.30\times 10^{52}$ & $6.24\times 10^{51}$ & $    1.12$ & $1.09\pm0.14$ \\
071020A& $2.146$ & A & $149$ & Swift & $4.30$ & $20$ & $9.38\times 10^{52}$ & $2.31\times 10^{53}$ & $    2.25$ & $...$ \\
071010B& $0.947$ & A & $122$ & Swift & $36.13$ & $20$ & $1.72\times 10^{52}$ & $6.24\times 10^{51}$ & $    2.25$ & $1.35\pm0.24$ \\
071010A& $0.980$ & A & $121$ & Swift & $6.32$ & $20$ & $1.17\times 10^{52}$ & $5.16\times 10^{51}$ & $    1.11$ & $1.08\pm0.29$ \\
071003A& $1.604$ & A & $130$ & Swift & $148.38$ & $20$ & $3.47\times 10^{53}$ & $2.07\times 10^{53}$ & $    1.57$ & $1.18\pm0.11$ \\
070810A& $2.170$ & A & $120$ & Swift & $9.04$ & $20$ & $1.58\times 10^{53}$ & $9.36\times 10^{52}$ & $    1.40$ & $1.18\pm0.14$ \\
070808A& $...$ & ... & $...$ & Swift & $58.43$ & $20$ & $3.89\times 10^{52}$ & $1.66\times 10^{52}$ & $    1.41$ & $1.19\pm0.43$ \\
070802A& $2.454$ & E & $287$ & Swift & $15.80$ & $20$ & $8.61\times 10^{51}$ & $3.15\times 10^{51}$ & $...$ & $...$ \\
070721B& $3.630$ & A & $149$ & Swift & $336.86$ & $20$ & $4.48\times 10^{54}$ & $9.14\times 10^{53}$ & $    1.38$ & $1.10\pm0.16$ \\
070714A& $1.580$ & E & $294$ & Swift & $3.00$ & $20$ & $2.95\times 10^{52}$ & $4.63\times 10^{52}$ & $    1.50$ & $1.50\pm0.21$ \\
070621A& $5.500$ & E & $293$ & Swift & $33.26$ & $20$ & $5.55\times 10^{53}$ & $1.74\times 10^{53}$ & $...$ & $...$ \\
070612A& $0.617$ & E & $119$ & Swift & $365.28$ & $20$ & $2.95\times 10^{53}$ & $6.57\times 10^{51}$ & $    1.12$ & $1.10\pm0.06$ \\
070611A& $2.039$ & A & $149$ & Swift & $13.18$ & $20$ & $9.92\times 10^{51}$ & $5.04\times 10^{51}$ & $    1.14$ & $1.09\pm0.12$ \\
070529A& $2.500$ & A & $118$ & Swift & $108.90$ & $20$ & $1.52\times 10^{53}$ & $2.61\times 10^{52}$ & $...$ & $...$ \\
070521A& $2.087$ & E & $287$ & Swift & $38.63$ & $20$ & $2.47\times 10^{53}$ & $1.74\times 10^{53}$ & $    2.29$ & $1.22\pm0.05$ \\
070518A& $1.161$ & E & $294$ & Swift & $4.35$ & $20$ & $1.23\times 10^{51}$ & $6.73\times 10^{50}$ & $    1.20$ & $1.12\pm0.1$ \\
070508A& $0.820$ & E & $117$ & Swift & $20.90$ & $20$ & $9.60\times 10^{52}$ & $3.65\times 10^{52}$ & $    4.38$ & $1.17\pm0.25$ \\
070506A& $2.309$ & A & $149$ & Swift & $4.35$ & $20$ & $6.11\times 10^{51}$ & $7.10\times 10^{51}$ & $    1.33$ & $...$ \\
070419B& $1.959$ & E & $287$ & Swift & $238.14$ & $20$ & $1.78\times 10^{54}$ & $8.21\times 10^{52}$ & $    1.24$ & $1.09\pm0.16$ \\
070419A& $0.971$ & A & $149$ & Swift & $160.00$ & $20$ & $4.17\times 10^{52}$ & $8.39\times 10^{50}$ & $...$ & $...$ \\
070411A& $2.954$ & A & $149$ & Swift & $102.04$ & $20$ & $1.18\times 10^{53}$ & $1.22\times 10^{52}$ & $    1.11$ & $1.07\pm0.09$ \\
070330A& $...$ & ... & $...$ & Swift & $6.64$ & $20$ & $3.73\times 10^{51}$ & $3.33\times 10^{51}$ & $    1.21$ & $1.08\pm0.38$ \\
070328A& $2.063$ & E & $287$ & Swift & $72.12$ & $20$ & $5.29\times 10^{53}$ & $1.24\times 10^{53}$ & $    1.73$ & $1.23\pm0.14$ \\
070318A& $0.840$ & E & $287$ & Swift & $131.52$ & $20$ & $1.79\times 10^{52}$ & $2.03\times 10^{51}$ & $    1.32$ & $1.09\pm0.11$ \\
070306A& $1.496$ & E & $287$ & Swift & $209.24$ & $20$ & $7.91\times 10^{52}$ & $1.19\times 10^{52}$ & $    1.38$ & $1.09\pm0.24$ \\
070224A& $1.992$ & E & $287$ & Swift & $48.00$ & $20$ & $7.66\times 10^{51}$ & $1.40\times 10^{51}$ & $    1.11$ & $1.09\pm0.29$ \\
070223A& $1.629$ & E & $293$ & Swift & $100.00$ & $20$ & $2.49\times 10^{52}$ & $1.89\times 10^{51}$ & $...$ & $...$ \\
070208A& $1.165$ & E & $116$ & Swift & $64.00$ & $20$ & $3.40\times 10^{51}$ & $9.97\times 10^{50}$ & $    1.16$ & $1.09\pm0.01$ \\
070129A& $2.338$ & E & $287$ & Swift & $459.05$ & $20$ & $7.90\times 10^{52}$ & $3.12\times 10^{51}$ & $...$ & $...$ \\
070125A& $1.547$ & A & $149$ & Konus-Wind & $70$ & $12$ & $9.21\times 10^{53}$ & $3.03\times 10^{53}$ & $...$ & $...$ \\
070110A& $2.352$ & E & $287$ & Swift & $79.71$ & $20$ & $5.79\times 10^{52}$ & $5.93\times 10^{51}$ & $...$ & $...$ \\
070103A& $2.621$ & E & $287$ & Swift & $18.40$ & $20$ & $1.09\times 10^{52}$ & $8.07\times 10^{51}$ & $...$ & $...$ \\
061222B& $3.355$ & A & $103$ & Swift & $37.25$ & $20$ & $1.08\times 10^{54}$ & $1.81\times 10^{53}$ & $...$ & $...$ \\
061222A& $2.088$ & E & $145$ & Swift & $96.00$ & $20$ & $3.11\times 10^{53}$ & $2.04\times 10^{53}$ & $    2.62$ & $1.55\pm0.32$ \\
061202A& $2.254$ & E & $287$ & Swift & $94.19$ & $20$ & $1.14\times 10^{53}$ & $2.25\times 10^{52}$ & $    1.43$ & $1.09\pm0.43$ \\
061126A& $1.159$ & E & $129$ & Swift & $50.28$ & $20$ & $9.05\times 10^{52}$ & $6.17\times 10^{52}$ & $    2.12$ & $1.27\pm0.19$ \\
061121A& $1.315$ & A & $149$ & Swift & $81.22$ & $20$ & $2.64\times 10^{53}$ & $1.38\times 10^{53}$ & $    4.81$ & $1.35\pm0.16$ \\
061110B& $3.434$ & A & $149$ & Swift & $132.76$ & $20$ & $2.48\times 10^{54}$ & $3.52\times 10^{53}$ & $...$ & $...$ \\
061110A& $0.758$ & E & $287$ & Swift & $44.51$ & $20$ & $4.64\times 10^{52}$ & $2.07\times 10^{51}$ & $    1.32$ & $1.07\pm0.29$ \\
061021A& $0.345$ & E & $287$ & Swift & $43.80$ & $20$ & $5.45\times 10^{51}$ & $2.03\times 10^{51}$ & $    2.06$ & $1.28\pm0.34$ \\
061007A& $1.262$ & A & $100$ & Swift & $75.74$ & $20$ & $9.84\times 10^{53}$ & $1.74\times 10^{53}$ & $    3.62$ & $1.20\pm0.16$ \\
060927A& $5.464$ & A & $113$ & Swift & $22.42$ & $20$ & $4.14\times 10^{53}$ & $5.91\times 10^{53}$ & $    1.46$ & $1.11\pm0.12$ \\
060926A& $3.209$ & A & $149$ & Swift & $7.79$ & $20$ & $1.39\times 10^{52}$ & $1.59\times 10^{52}$ & $    1.21$ & $...$ \\
060923C& $...$ & ... & $...$ & Swift & $67.41$ & $20$ & $3.45\times 10^{53}$ & $3.48\times 10^{52}$ & $...$ & $...$ \\
060923B& $1.509$ & E & $287$ & Swift & $8.95$ & $20$ & $7.85\times 10^{52}$ & $2.99\times 10^{52}$ & $...$ & $...$ \\
060923A& $2.600$ & E & $245$ & Swift & $51.54$ & $20$ & $3.22\times 10^{53}$ & $1.41\times 10^{53}$ & $    1.25$ & $1.09\pm0.23$ \\
060912A& $0.936$ & E & $287$ & Swift & $5.03$ & $20$ & $7.62\times 10^{51}$ & $7.21\times 10^{51}$ & $    1.94$ & $1.40\pm0.34$ \\
060908A& $1.884$ & A & $238$ & Swift & $18.78$ & $20$ & $2.06\times 10^{53}$ & $5.91\times 10^{52}$ & $    1.60$ & $1.12\pm0.1$ \\
060906A& $3.686$ & A & $149$ & Swift & $44.58$ & $20$ & $1.22\times 10^{53}$ & $3.22\times 10^{52}$ & $...$ & $...$ \\
060904B& $0.703$ & E & $149$ & Swift & $171.90$ & $20$ & $6.15\times 10^{52}$ & $1.33\times 10^{52}$ & $    1.50$ & $1.19\pm0.07$ \\
060814A& $1.922$ & E & $287$ & Swift & $144.95$ & $20$ & $3.51\times 10^{53}$ & $8.12\times 10^{52}$ & $    2.15$ & $1.11\pm0.09$ \\
060807A& $...$ & ... & $...$ & Swift & $53.74$ & $20$ & $2.31\times 10^{52}$ & $5.59\times 10^{51}$ & $    1.12$ & $1.08\pm0.07$ \\
060805A& $2.363$ & E & $287$ & Swift & $4.93$ & $20$ & $2.00\times 10^{52}$ & $2.02\times 10^{52}$ & $...$ & $...$ \\
060729A& $0.543$ & E & $287$ & Swift & $113.04$ & $20$ & $4.86\times 10^{51}$ & $2.55\times 10^{50}$ & $    1.27$ & $1.10\pm0.16$ \\
060719A& $1.532$ & E & $287$ & Swift & $66.86$ & $20$ & $1.92\times 10^{52}$ & $4.79\times 10^{51}$ & $    1.38$ & $1.11\pm0.27$ \\
060714A& $2.711$ & A & $88$ & Swift & $116.04$ & $20$ & $9.66\times 10^{52}$ & $1.09\times 10^{52}$ & $...$ & $...$ \\
060708A& $1.920$ & P & $174$ & Swift & $9.96$ & $20$ & $1.10\times 10^{52}$ & $9.99\times 10^{51}$ & $    1.44$ & $1.21\pm0.38$ \\
060707A& $3.425$ & E & $287$ & Swift & $66.65$ & $20$ & $4.86\times 10^{53}$ & $1.27\times 10^{53}$ & $    1.16$ & $1.07\pm0.14$ \\
060614A& $0.125$ & E & $105$ & Swift & $5$ & $35$ & $2.13\times 10^{51}$ & $2.63\times 10^{50}$ & $    2.56$ & $2.26\pm0.23$ \\
060607A& $3.075$ & A & $127$ & Swift & $102.98$ & $20$ & $1.72\times 10^{54}$ & $3.47\times 10^{53}$ & $    1.25$ & $1.07\pm0.11$ \\
060605A& $3.773$ & A & $143$ & Swift & $539.12$ & $20$ & $5.43\times 10^{52}$ & $1.43\times 10^{52}$ & $    1.21$ & $1.11\pm0.24$ \\
060604A& $2.135$ & E & $287$ & Swift & $96.00$ & $20$ & $9.14\times 10^{51}$ & $1.55\times 10^{51}$ & $...$ & $...$ \\
060602A& $0.787$ & E & $123$ & Swift & $74.68$ & $20$ & $1.54\times 10^{53}$ & $6.38\times 10^{51}$ & $...$ & $...$ \\
060526A& $3.221$ & A & $96$ & Swift & $275.20$ & $20$ & $5.63\times 10^{52}$ & $2.02\times 10^{52}$ & $    1.35$ & $1.09\pm0.29$ \\
060522A& $5.110$ & A & $114$ & Swift & $69.12$ & $20$ & $1.35\times 10^{53}$ & $3.31\times 10^{52}$ & $...$ & $...$ \\
060512A& $0.443$ & E & $97$ & Swift & $11.36$ & $20$ & $3.25\times 10^{50}$ & $9.73\times 10^{49}$ & $    1.15$ & $1.07\pm0.11$ \\
060510B& $4.900$ & A & $95$ & Swift & $262.95$ & $20$ & $3.59\times 10^{54}$ & $2.41\times 10^{53}$ & $...$ & $...$ \\
060505A& $0.089$ & E & $111$ & Swift & $4$ & $37$ & $9.24\times 10^{49}$ & $2.51\times 10^{49}$ & $    1.58$ & $1.27\pm0.25$ \\
060502A& $1.503$ & A & $149$ & Swift & $28.54$ & $20$ & $4.93\times 10^{53}$ & $8.96\times 10^{52}$ & $    1.31$ & $1.10\pm0.32$ \\
060418A& $1.490$ & A & $107$ & Swift & $109.17$ & $20$ & $1.16\times 10^{53}$ & $1.77\times 10^{52}$ & $    1.94$ & $1.31\pm0.29$ \\
060319A& $1.172$ & E & $245$ & Swift & $8.91$ & $20$ & $2.30\times 10^{51}$ & $1.14\times 10^{51}$ & $    1.24$ & $1.16\pm0.16$ \\
060306A& $1.560$ & E & $287$ & Swift & $60.94$ & $20$ & $2.97\times 10^{52}$ & $1.57\times 10^{52}$ & $    2.25$ & $1.51\pm0.12$ \\
060223A& $4.406$ & A & $114$ & Swift & $11.32$ & $20$ & $5.56\times 10^{53}$ & $4.44\times 10^{53}$ & $    1.45$ & $1.20\pm0.05$ \\
060218A& $0.034$ & E & $91$ & Swift & $1040$ & $20$ & $9.33\times 10^{48}$ & $8.65\times 10^{46}$ & $...$ & $...$ \\
060210A& $3.912$ & A & $149$ & Swift & $242.18$ & $20$ & $6.49\times 10^{53}$ & $9.50\times 10^{52}$ & $    1.58$ & $1.16\pm0.1$ \\
060206A& $4.056$ & A & $149$ & Swift & $7.55$ & $20$ & $1.31\times 10^{53}$ & $2.00\times 10^{53}$ & $    1.56$ & $...$ \\
060204B& $2.339$ & E & $287$ & Swift & $139.46$ & $20$ & $8.31\times 10^{53}$ & $9.76\times 10^{52}$ & $    1.26$ & $1.07\pm0.07$ \\
060202A& $0.785$ & E & $245$ & Swift & $172.16$ & $20$ & $8.66\times 10^{51}$ & $2.88\times 10^{50}$ & $...$ & $...$ \\
060124A& $2.300$ & A & $149$ & Swift & $658.2$ & $20$ & $2.11\times 10^{53}$ & $1.29\times 10^{53}$ & $    3.38$ & $1.34\pm0.2$ \\
060115A& $3.533$ & A & $149$ & Swift & $122.21$ & $20$ & $1.47\times 10^{53}$ & $2.67\times 10^{52}$ & $    1.15$ & $1.07\pm0.07$ \\
060111A& $2.320$ & E & $295$ & Swift & $13.21$ & $20$ & $3.18\times 10^{53}$ & $1.17\times 10^{53}$ & $    1.53$ & $1.14\pm0.16$ \\
060108A& $2.030$ & P & $94$ & Swift & $14.22$ & $20$ & $7.69\times 10^{51}$ & $3.07\times 10^{51}$ & $    1.21$ & $1.10\pm0.38$ \\
051117B& $0.480$ & E & $287$ & Swift & $9.01$ & $20$ & $3.34\times 10^{51}$ & $1.07\times 10^{51}$ & $    1.15$ & $1.08\pm0.29$ \\
051111A& $1.550$ & A & $149$ & Swift & $64.00$ & $20$ & $1.12\times 10^{53}$ & $1.65\times 10^{52}$ & $    1.34$ & $1.07\pm0.01$ \\
051109B& $0.080$ & E & $99$ & Swift & $13.38$ & $20$ & $6.78\times 10^{49}$ & $1.14\times 10^{49}$ & $    1.16$ & $1.08\pm0.21$ \\
051109A& $2.346$ & A & $81$ & Swift & $37.20$ & $20$ & $8.28\times 10^{52}$ & $4.02\times 10^{52}$ & $    1.44$ & $1.12\pm0.32$ \\
051022A& $0.809$ & E & $108$ & HETE-2 & $178$ & $14$ & $6.10\times 10^{53}$ & $4.23\times 10^{52}$ & $...$ & $...$ \\
051016B& $0.936$ & E & $287$ & Swift & $4.02$ & $20$ & $9.49\times 10^{51}$ & $8.81\times 10^{51}$ & $    1.30$ & $1.15\pm0.43$ \\
051008A& $2.770$ & P & $286$ & Swift & $64.0$ & $20$ & $6.22\times 10^{53}$ & $2.31\times 10^{53}$ & $    1.81$ & $1.17\pm0.16$ \\
051006A& $1.059$ & E & $218$ & Swift & $26.04$ & $20$ & $1.29\times 10^{52}$ & $2.71\times 10^{51}$ & $    1.27$ & $1.08\pm0.29$ \\
051001A& $2.429$ & E & $287$ & Swift & $190.63$ & $20$ & $4.94\times 10^{52}$ & $2.97\times 10^{51}$ & $    1.10$ & $1.06\pm0.34$ \\
050922C& $2.199$ & A & $88$ & Swift & $4.54$ & $20$ & $9.53\times 10^{52}$ & $1.88\times 10^{53}$ & $    3.29$ & $...$ \\
050922B& $4.900$ & P & $293$ & Swift & $156.29$ & $20$ & $2.04\times 10^{54}$ & $4.62\times 10^{53}$ & $    1.27$ & $1.07\pm0.12$ \\
050915A& $2.527$ & E & $287$ & Swift & $53.42$ & $20$ & $4.87\times 10^{53}$ & $1.49\times 10^{53}$ & $    1.26$ & $1.07\pm0.06$ \\
050908A& $3.347$ & A & $149$ & Swift & $18.29$ & $20$ & $2.34\times 10^{52}$ & $1.03\times 10^{52}$ & $    1.12$ & $1.07\pm0.23$ \\
050904A& $6.295$ & A & $104$ & Swift & $181.70$ & $20$ & $1.23\times 10^{54}$ & $1.03\times 10^{53}$ & $...$ & $...$ \\
050826A& $0.296$ & E & $110$ & Swift & $35.73$ & $20$ & $6.27\times 10^{50}$ & $6.77\times 10^{49}$ & $    1.14$ & $1.07\pm0.34$ \\
050824A& $0.828$ & E & $287$ & Swift & $24.82$ & $20$ & $1.72\times 10^{51}$ & $3.23\times 10^{50}$ & $...$ & $...$ \\
050822A& $1.434$ & E & $218$ & Swift & $104.12$ & $20$ & $3.25\times 10^{52}$ & $3.96\times 10^{51}$ & $    1.29$ & $1.10\pm0.1$ \\
050820A& $2.615$ & A & $115$ & Swift & $26$ & $37$ & $2.59\times 10^{53}$ & $5.98\times 10^{52}$ & $    1.32$ & $1.14\pm0.2$ \\
050819A& $2.504$ & E & $287$ & Swift & $37.72$ & $20$ & $1.73\times 10^{52}$ & $3.60\times 10^{51}$ & $...$ & $...$ \\
050814A& $5.300$ & P & $85$ & Swift & $144.00$ & $20$ & $1.98\times 10^{53}$ & $3.25\times 10^{52}$ & $...$ & $...$ \\
050803A& $4.300$ & P & $293$ & Swift & $88.12$ & $20$ & $2.66\times 10^{53}$ & $5.49\times 10^{52}$ & $    1.34$ & $1.44\pm0.38$ \\
050802A& $1.710$ & A & $149$ & Swift & $27.46$ & $20$ & $4.41\times 10^{52}$ & $1.38\times 10^{52}$ & $    1.18$ & $1.08\pm0.03$ \\
050801A& $1.380$ & P & $174$ & Swift & $19.40$ & $20$ & $3.23\times 10^{51}$ & $2.35\times 10^{51}$ & $    1.39$ & $1.12\pm0.07$ \\
050730A& $3.969$ & A & $79$ & Swift & $145.05$ & $20$ & $2.06\times 10^{53}$ & $1.98\times 10^{52}$ & $    1.16$ & $1.08\pm0.03$ \\
050726A& $3.500$ & P & $293$ & Swift & $49.70$ & $20$ & $4.25\times 10^{53}$ & $1.26\times 10^{53}$ & $    1.13$ & $1.07\pm0.16$ \\
050714B& $2.438$ & E & $287$ & Swift & $46.87$ & $20$ & $1.43\times 10^{53}$ & $3.16\times 10^{52}$ & $...$ & $...$ \\
050713A& $3.600$ & P & $145$ & Swift & $94.91$ & $20$ & $3.09\times 10^{53}$ & $1.98\times 10^{53}$ & $    1.88$ & $1.14\pm0.14$ \\
050525A& $0.606$ & E & $287$ & Swift & $8.84$ & $20$ & $2.84\times 10^{52}$ & $1.93\times 10^{52}$ & $    9.38$ & $1.83\pm0.11$ \\
050505A& $4.275$ & A & $90$ & Swift & $58.88$ & $20$ & $2.90\times 10^{53}$ & $9.86\times 10^{52}$ & $...$ & $...$ \\
050502B& $5.200$ & P & $194$ & Swift & $16.62$ & $20$ & $5.51\times 10^{53}$ & $7.76\times 10^{53}$ & $    1.44$ & $1.15\pm0.21$ \\
050502A& $3.793$ & A & $80$ & Swift & $17.5$ & $10$ & $9.17\times 10^{52}$ & $6.32\times 10^{52}$ & $...$ & $...$ \\
050416A& $0.654$ & E & $287$ & Swift & $6.62$ & $20$ & $1.21\times 10^{52}$ & $9.77\times 10^{51}$ & $    1.54$ & $...$ \\
050408A& $1.236$ & E & $78$ & HETE-2 & $28.39$ & $14$ & $2.33\times 10^{52}$ & $...$ & $...$ & $...$ \\
050401A& $2.898$ & A & $93$ & Swift & $33.30$ & $20$ & $4.20\times 10^{53}$ & $2.08\times 10^{53}$ & $    1.51$ & $1.10\pm0.14$ \\
050319A& $3.243$ & A & $149$ & Swift & $151.74$ & $20$ & $5.92\times 10^{52}$ & $1.85\times 10^{52}$ & $    1.19$ & $1.12\pm0.19$ \\
050318A& $1.444$ & A & $78$ & Swift & $40.0$ & $20$ & $1.25\times 10^{52}$ & $6.13\times 10^{51}$ & $    1.56$ & $1.17\pm0.16$ \\
050315A& $1.950$ & A & $78$ & Swift & $95.57$ & $20$ & $6.34\times 10^{52}$ & $6.76\times 10^{51}$ & $    1.32$ & $1.08\pm0.29$ \\
050223A& $0.584$ & E & $87$ & Swift & $21.68$ & $20$ & $4.36\times 10^{51}$ & $3.18\times 10^{50}$ & $...$ & $...$ \\
050219A& $0.211$ & E & $271$ & Swift & $23.84$ & $20$ & $1.05\times 10^{52}$ & $9.81\times 10^{50}$ & $    1.75$ & $1.18\pm0.34$ \\
050215B& $2.620$ & E & $295$ & Swift & $10.62$ & $20$ & $6.95\times 10^{51}$ & $6.34\times 10^{52}$ & $...$ & $...$ \\
050128A& $5.500$ & P & $293$ & Swift & $28.00$ & $20$ & $2.23\times 10^{54}$ & $2.00\times 10^{54}$ & $    2.52$ & $1.23\pm0.16$ \\
050126A& $1.290$ & E & $76$ & Swift & $48.00$ & $20$ & $1.59\times 10^{52}$ & $2.73\times 10^{51}$ & $...$ & $...$ \\
041219A& $0.310$ & P & $217$ & Swift & $520$ & $37$ & $6.88\times 10^{52}$ & $3.74\times 10^{51}$ & $...$ & $...$ \\
041006A& $0.716$ & E & $89$ & HETE-2 & $22.08$ & $14$ & $2.11\times 10^{52}$ & $...$ & $...$ & $...$ \\
040924A& $0.858$ & E & $126$ & HETE-2 & $3.37$ & $14$ & $9.21\times 10^{51}$ & $2.09\times 10^{52}$ & $...$ & $...$ \\
040912A& $1.563$ & E & $106$ & HETE-2 & $9.21$ & $14$ & $8.47\times 10^{51}$ & $...$ & $...$ & $...$ \\
031203A& $0.105$ & E & $72$ & HETE-2 & $10.38$ & $14$ & $6.84\times 10^{49}$ & $1.78\times 10^{49}$ & $...$ & $...$ \\
030528A& $0.782$ & A & $74$ & HETE-2 & $62.8$ & $14$ & $2.22\times 10^{52}$ & $1.25\times 10^{51}$ & $...$ & $...$ \\
030429A& $2.658$ & A & $69$ & HETE-2 & $12.95$ & $14$ & $1.70\times 10^{52}$ & $7.47\times 10^{51}$ & $...$ & $...$ \\
030329A& $0.169$ & E & $67$ & HETE-2 & $25.91$ & $14$ & $1.55\times 10^{52}$ & $1.65\times 10^{51}$ & $...$ & $...$ \\
030328A& $1.522$ & A & $86$ & HETE-2 & $138.27$ & $14$ & $3.59\times 10^{53}$ & $1.40\times 10^{52}$ & $...$ & $...$ \\
030323A& $3.374$ & E & $68$ & HETE-2 & $26$ & $9$ & $...$ & $...$ & $...$ & $...$ \\
030226A& $1.986$ & A & $70$ & HETE-2 & $76.23$ & $14$ & $7.46\times 10^{52}$ & $5.76\times 10^{51}$ & $...$ & $...$ \\
030115A& $2.000$ & P & $269$ & HETE-2 & $20.33$ & $14$ & $3.01\times 10^{52}$ & $1.11\times 10^{52}$ & $...$ & $...$ \\
021211A& $1.006$ & E & $66$ & HETE-2 & $4.23$ & $14$ & $1.34\times 10^{52}$ & $8.62\times 10^{51}$ & $...$ & $...$ \\
021004A& $2.335$ & E & $50$ & HETE-2 & $48.94$ & $14$ & $4.33\times 10^{52}$ & $6.68\times 10^{51}$ & $...$ & $...$ \\
020903A& $0.251$ & E & $71$ & HETE-2 & $3.3$ & $8$ & $2.03\times 10^{49}$ & $6.36\times 10^{48}$ & $...$ & $...$ \\
020819B& $0.410$ & E & $75$ & Ulysses & $20$ & $7$ & $...$ & $...$ & $...$ & $...$ \\
020813A& $1.255$ & E & $61$ & HETE-2 & $87.34$ & $14$ & $1.34\times 10^{54}$ & $7.36\times 10^{52}$ & $...$ & $...$ \\
020427A& $...$ & ... & $...$ & BeppoSAX & $66$ & $6$ & $1.52\times 10^{52}$ & $2.35\times 10^{51}$ & $...$ & $...$ \\
020405A& $0.691$ & E & $59$ & BeppoSAX & $40.0$ & $18$ & $1.07\times 10^{53}$ & $1.38\times 10^{52}$ & $...$ & $...$ \\
020331A& $...$ & ... & $...$ & HETE-2 & $179.4$ & $14$ & $9.31\times 10^{52}$ & $8.32\times 10^{51}$ & $...$ & $...$ \\
020322A& $...$ & ... & $...$ & BeppoSAX & $11.0$ & $18$ & $2.30\times 10^{52}$ & $1.82\times 10^{52}$ & $...$ & $...$ \\
020305A& $2.800$ & P & $73$ & HETE-2 & $39.06$ & $14$ & $3.09\times 10^{53}$ & $...$ & $...$ & $...$ \\
020127A& $1.900$ & P & $109$ & HETE-2 & $6.99$ & $14$ & $3.36\times 10^{52}$ & $1.43\times 10^{52}$ & $...$ & $...$ \\
020124A& $3.198$ & A & $64$ & HETE-2 & $51.17$ & $14$ & $2.09\times 10^{53}$ & $5.33\times 10^{52}$ & $...$ & $...$ \\
011211A& $2.140$ & A & $51$ & BeppoSAX & $51.0$ & $18$ & $3.23\times 10^{52}$ & $2.63\times 10^{51}$ & $...$ & $...$ \\
011121A& $0.360$ & E & $65$ & BeppoSAX & $47.0$ & $18$ & $6.42\times 10^{52}$ & $5.86\times 10^{51}$ & $...$ & $...$ \\
011030A& $3.000$ & P & $57$ & BeppoSAX & $1400$ & $5$ & $1.35\times 10^{53}$ & $3.37\times 10^{51}$ & $...$ & $...$ \\
010921A& $0.451$ & E & $52$ & BeppoSAX & $22.0$ & $18$ & $1.51\times 10^{52}$ & $1.70\times 10^{51}$ & $...$ & $...$ \\
010222A& $1.477$ & A & $55$ & BeppoSAX & $74.0$ & $18$ & $1.38\times 10^{54}$ & $3.19\times 10^{53}$ & $...$ & $...$ \\
000926A& $2.038$ & A & $62$ & BeppoSAX & $1.30$ & $18$ & $7.66\times 10^{51}$ & $1.93\times 10^{52}$ & $...$ & $...$ \\
000911A& $1.058$ & E & $53$ & Uly/Ko/NE & $500$ & $4$ & $6.53\times 10^{53}$ & $1.17\times 10^{53}$ & $...$ & $...$ \\
000418A& $1.118$ & E & $60$ & BeppoSAX & $2.0$ & $18$ & $...$ & $...$ & $...$ & $...$ \\
000301C& $2.040$ & A & $47$ & BeppoSAX & $87.0$ & $18$ & $1.41\times 10^{53}$ & $5.82\times 10^{51}$ & $...$ & $...$ \\
000214A& $...$ & ... & $...$ & BeppoSAX & $8.0$ & $18$ & $2.92\times 10^{53}$ & $2.47\times 10^{53}$ & $...$ & $...$ \\
000210A& $0.846$ & E & $54$ & BeppoSAX & $9.0$ & $18$ & $1.54\times 10^{53}$ & $9.74\times 10^{52}$ & $...$ & $...$ \\
000131A& $4.500$ & A & $45$ & Uly/Ko/NE & $50$ & $3$ & $1.61\times 10^{54}$ & $4.14\times 10^{53}$ & $...$ & $...$ \\
991216A& $1.020$ & A & $43$ & BeppoSAX & $45.0$ & $18$ & $6.00\times 10^{53}$ & $3.33\times 10^{53}$ & $...$ & $...$ \\
991208A& $0.706$ & E & $46$ & Uly/Ko/NE & $60$ & $2$ & $2.66\times 10^{53}$ & $4.73\times 10^{52}$ & $...$ & $...$ \\
990712A& $0.433$ & E & $48$ & BeppoSAX & $38.0$ & $18$ & $7.94\times 10^{51}$ & $2.28\times 10^{51}$ & $...$ & $...$ \\
990705A& $0.842$ & E & $56$ & BeppoSAX & $32.0$ & $18$ & $2.59\times 10^{53}$ & $2.35\times 10^{52}$ & $...$ & $...$ \\
990510A& $1.619$ & A & $48$ & BeppoSAX & $57.0$ & $18$ & $2.03\times 10^{53}$ & $6.92\times 10^{52}$ & $...$ & $...$ \\
990506A& $1.307$ & E & $60$ & BeppoSAX & $129.0$ & $18$ & $8.66\times 10^{53}$ & $1.00\times 10^{53}$ & $...$ & $...$ \\
990308A& $...$ & ... & $...$ & BeppoSAX & $0.36$ & $18$ & $6.32\times 10^{52}$ & $5.14\times 10^{52}$ & $...$ & $...$ \\
990123A& $1.600$ & A & $44$ & BeppoSAX & $61.0$ & $18$ & $6.46\times 10^{54}$ & $9.51\times 10^{53}$ & $...$ & $...$ \\
981226A& $1.110$ & P & $77$ & BeppoSAX & $17.0$ & $18$ & $5.50\times 10^{51}$ & $7.40\times 10^{50}$ & $...$ & $...$ \\
980703A& $0.966$ & E & $40$ & BeppoSAX & $76.0$ & $18$ & $1.33\times 10^{53}$ & $1.17\times 10^{52}$ & $...$ & $...$ \\
980613A& $1.097$ & E & $63$ & BeppoSAX & $42.0$ & $18$ & $5.34\times 10^{51}$ & $1.79\times 10^{51}$ & $...$ & $...$ \\
980519A& $...$ & ... & $...$ & BeppoSAX & $33.0$ & $18$ & $1.64\times 10^{53}$ & $2.55\times 10^{53}$ & $...$ & $...$ \\
980425A& $0.009$ & E & $41$ & BeppoSAX & $22.0$ & $18$ & $9.40\times 10^{47}$ & $4.71\times 10^{46}$ & $...$ & $...$ \\
980329A& $3.500$ & P & $58$ & BeppoSAX & $19.0$ & $18$ & $3.31\times 10^{54}$ & $7.10\times 10^{53}$ & $...$ & $...$ \\
980326A& $...$ & ... & $...$ & BeppoSAX & $312.0$ & $18$ & $1.37\times 10^{52}$ & $1.34\times 10^{52}$ & $...$ & $...$ \\
971214A& $3.420$ & E & $42$ & BeppoSAX & $6.0$ & $18$ & $3.56\times 10^{53}$ & $1.22\times 10^{53}$ & $...$ & $...$ \\
970828A& $0.958$ & E & $49$ & ... & $...$ & $...$ & $3.00\times 10^{53}$ & $2.45\times 10^{52}$ & $...$ & $...$ \\
970508A& $0.835$ & A & $39$ & BeppoSAX & $14.0$ & $18$ & $7.65\times 10^{51}$ & $2.65\times 10^{51}$ & $...$ & $...$ \\
970228A& $...$ & ... & $...$ & BeppoSAX & $56.0$ & $18$ & $1.96\times 10^{53}$ & $1.98\times 10^{53}$ & $...$ & $...$ \\
\hline
&SGRB&\\\hline
130603B& $0.356$ & E & $256$ & Swift & $0.18$ & $37$ & $2.02\times 10^{51}$ & $4.15\times 10^{52}$ & $...$ & $...$ \\
101224A& $...$ & ... & $...$ & Swift & $0.2$ & $37$ & $2.34\times 10^{50}$ & $4.62\times 10^{50}$ & $    1.63$ & $1.63\pm0.43$ \\
101219A& $0.718$ & E & $199$ & Swift & $0.6$ & $37$ & $4.49\times 10^{51}$ & $6.00\times 10^{52}$ & $    2.75$ & $2.75\pm0.45$ \\
100816A& $0.805$ & E & $287$ & Swift & $2.9$ & $37$ & $7.93\times 10^{51}$ & $9.04\times 10^{51}$ & $    2.62$ & $1.52\pm0.03$ \\
100625A& $0.452$ & A & $241$ & Swift & $0.33$ & $37$ & $9.17\times 10^{50}$ & $1.65\times 10^{51}$ & $    2.63$ & $2.63\pm0.26$ \\
100206A& $0.407$ & E & $220$ & Swift & $0.12$ & $37$ & $5.81\times 10^{50}$ & $7.86\times 10^{50}$ & $    2.70$ & $2.70\pm0.26$ \\
100117A& $0.920$ & E & $195$ & Swift & $0.3$ & $37$ & $1.32\times 10^{51}$ & $2.22\times 10^{51}$ & $    2.28$ & $2.28\pm0.21$ \\
091109B& $...$ & ... & $...$ & Swift & $0.27$ & $20$ & $6.87\times 10^{52}$ & $1.04\times 10^{53}$ & $    4.93$ & $4.93\pm0.65$ \\
090515A& $...$ & ... & $...$ & Swift & $0.04$ & $20$ & $2.90\times 10^{51}$ & $1.40\times 10^{53}$ & $    2.58$ & $2.58\pm0.32$ \\
090510A& $0.903$ & E & $162$ & Swift & $5.66$ & $20$ & $2.83\times 10^{52}$ & $5.57\times 10^{52}$ & $    5.00$ & $5.00\pm0.55$ \\
090426A& $2.609$ & A & $161$ & Swift & $1.24$ & $20$ & $5.50\times 10^{51}$ & $1.88\times 10^{52}$ & $    2.61$ & $1.48\pm0.15$ \\
090305A& $...$ & ... & $...$ & Swift & $0.35$ & $20$ & $2.18\times 10^{52}$ & $3.69\times 10^{52}$ & $    1.48$ & $1.48\pm0.16$ \\
080905A& $0.122$ & E & $192$ & Swift & $1.02$ & $20$ & $4.30\times 10^{49}$ & $3.05\times 10^{49}$ & $    1.85$ & $1.85\pm0.15$ \\
080503A& $...$ & ... & $...$ & Swift & $0.32$ & $17$ & $...$ & $...$ & $    1.97$ & $1.53\pm0.18$ \\
080123A& $0.495$ & ... & $179$ & Swift & $0.04$ & $20$ & $7.43\times 10^{50}$ & $2.09\times 10^{50}$ & $...$ & $...$ \\
071227A& $0.383$ & E & $125$ & Swift & $1.8$ & $35$ & $1.04\times 10^{51}$ & $3.16\times 10^{51}$ & $    3.00$ & $2.80\pm0.23$ \\
070809A& $0.219$ & E & $133$ & Swift & $1.28$ & $20$ & $3.18\times 10^{49}$ & $4.08\times 10^{49}$ & $    1.42$ & $1.42\pm0.25$ \\
070724A& $0.457$ & E & $148$ & Swift & $0.43$ & $20$ & $3.67\times 10^{50}$ & $5.95\times 10^{50}$ & $    1.53$ & $1.53\pm0.12$ \\
070714B& $0.923$ & E & $142$ & Swift & $3$ & $35$ & $...$ & $...$ & $    2.94$ & $2.54\pm0.34$ \\
070707A& $...$ & ... & $...$ & INTEGRAL & $0.8$ & $13$ & $6.88\times 10^{50}$ & $1.03\times 10^{51}$ & $...$ & $...$ \\
070429B& $0.904$ & E & $142$ & Swift & $0.49$ & $20$ & $4.00\times 10^{51}$ & $8.51\times 10^{51}$ & $    1.51$ & $1.51\pm0.19$ \\
061217A& $0.827$ & E & $112$ & Swift & $0.24$ & $20$ & $2.34\times 10^{51}$ & $1.69\times 10^{52}$ & $    1.74$ & $1.74\pm0.12$ \\
061210A& $0.410$ & E & $101$ & Swift & $0.13$ & $36$ & $...$ & $...$ & $    8.13$ & $7.83\pm0.38$ \\
061201A& $0.111$ & E & $102$ & Swift & $0.78$ & $20$ & $1.96\times 10^{50}$ & $1.31\times 10^{51}$ & $    4.67$ & $4.67\pm0.67$ \\
061006A& $0.438$ & E & $112$ & Swift & $0.5$ & $35$ & $2.32\times 10^{51}$ & $1.99\times 10^{52}$ & $    6.01$ & $5.41\pm0.32$ \\
060801A& $1.131$ & E & $146$ & Swift & $0.50$ & $20$ & $2.35\times 10^{52}$ & $8.96\times 10^{52}$ & $    2.19$ & $2.19\pm0.35$ \\
060502B& $0.287$ & A & $98$ & Swift & $0.14$ & $20$ & $2.19\times 10^{51}$ & $3.57\times 10^{51}$ & $    2.33$ & $2.33\pm0.24$ \\
060313A& $...$ & ... & $...$ & Swift & $0.74$ & $20$ & $1.28\times 10^{52}$ & $9.44\times 10^{52}$ & $    4.94$ & $4.94\pm0.43$ \\
060121A& $...$ & ... & $...$ & HETE-2 & $2.61$ & $14$ & $3.91\times 10^{51}$ & $2.04\times 10^{52}$ & $...$ & $...$ \\
051227A& $0.800$ & P & $144$ & Swift & $3.5$ & $35$ & $...$ & $...$ & $    1.38$ & $1.32\pm0.32$ \\
051221A& $0.546$ & E & $92$ & Swift & $1.40$ & $20$ & $3.12\times 10^{51}$ & $6.94\times 10^{52}$ & $    7.00$ & $7.00\pm0.65$ \\
051210A& $1.400$ & P & $177$ & Swift & $1.27$ & $35$ & $6.27\times 10^{51}$ & $1.45\times 10^{52}$ & $    1.44$ & $1.44\pm0.18$ \\
050724A& $0.258$ & A & $84$ & Swift & $2.76$ & $36$ & $...$ & $...$ & $    2.50$ & $2.02\pm0.19$ \\
050709A& $0.160$ & E & $82$ & HETE-2 & $0.22$ & $11$ & $3.27\times 10^{49}$ & $...$ & $...$ & $...$ \\
050509B& $0.226$ & A & $83$ & Swift & $0.02$ & $20$ & $7.09\times 10^{49}$ & $2.23\times 10^{50}$ & $    1.84$ & $1.84\pm0.29$ \\
\enddata
\tablecomments{References.
(1) \citet{};
(2) \citet{1999GCN...450....1H};
(3) \citet{2000GCN...529....1H};
(4) \citet{2000GCN...791....1H};
(5) \citet{2001GCN..1138....1H};
(6) \citet{2002GCN..1383....1I};
(7) \citet{2002GCN..1507....1H};
(8) \citet{2002GCN..1530....1R};
(9) \citet{2003GCN..1956....1G};
(10) \citet{2005GCN..3339....1C};
(11) \citet{2005Natur.437..855V};
(12) \citet{2007GCN..6049....1G};
(13) \citet{2008A&A...486..405M};
(14) \citet{2008A&A...491..157P};
(15) \citet{2008GCN..7752....1H};
(16) \citet{2008GCN..8133....1E};
(17) \citet{2009ApJ...696.1871P};
(18) \citet{2009ApJS..180..192F};
(19) \citet{2010GCN..10524...1S};
(20) \citet{2011ApJS..195....2S};
(21) \citet{2011GCN..11722...1G};
(22) \citet{2011GCN..12676...1G};
(23) \citet{2012GCN..13498...1D};
(24) \citet{2012GCN..14123...1K};
(25) \citet{2013ApJ...766...30G};
(26) \citet{2013GCN..14674...1S};
(27) \citet{2013GCN..14972...1A};
(28) \citet{2013GCN..15331...1J};
(29) \citet{2013GCN..15477...1Y};
(30) \citet{2014A&A...568A..75G};
(31) \citet{2014ApJS..211...13V};
(32) \citet{2014GCN..15644...1J};
(33) \citet{2014GCN..16224...1H};
(34) \citet{2014GCN..16363...1B};
(35) \citet{2015ApJ...805...89L};
(36) \citet{2015MNRAS.452..824K};
(37) \citet{GRBtable};
(38) \citet{-1};
(39) \citet{1997IAUC.6655....1G};
(40) \citet{1998ApJ...508L..17D};
(41) \citet{1998IAUC.6896....3W};
(42) \citet{1998Natur.393...35K};
(43) \citet{1999GCN...496....1V};
(44) \citet{1999Natur.398..389K};
(45) \citet{2000A&A...364L..54A};
(46) \citet{2001A&A...370..398C};
(47) \citet{2001A&A...370..909J};
(48) \citet{2001ApJ...546..672V};
(49) \citet{2001ApJ...562..654D};
(50) \citet{2002A&A...396L..21M};
(51) \citet{2002AJ....124..639H};
(52) \citet{2002ApJ...571L.121P};
(53) \citet{2002ApJ...573...85P};
(54) \citet{2002ApJ...577..680P};
(55) \citet{2002ApJ...578..818M};
(56) \citet{2002ApJ...581L..81L};
(57) \citet{2002GCN..1268....1F};
(58) \citet{2003A&A...402..125J};
(59) \citet{2003A&A...404..465M};
(60) \citet{2003AJ....125..999B};
(61) \citet{2003ApJ...584L..47B};
(62) \citet{2003ApJ...586..128C};
(63) \citet{2003ApJ...591L..13D};
(64) \citet{2003ApJ...597..699H};
(65) \citet{2003ApJ...599.1223G};
(66) \citet{2003GCN..1785....1V};
(67) \citet{2003Natur.423..847H};
(68) \citet{2004A&A...419..927V};
(69) \citet{2004A&A...427..785J};
(70) \citet{2004AJ....128.1942K};
(71) \citet{2004ApJ...606..994S};
(72) \citet{2004ApJ...611..200P};
(73) \citet{2005A&A...437..411G};
(74) \citet{2005A&A...444..425R};
(75) \citet{2005ApJ...629...45J};
(76) \citet{2005ApJ...629..328B};
(77) \citet{2005ApJ...631L..29C};
(78) \citet{2005ApJ...634..501B};
(79) \citet{2005ApJ...634L..25C};
(80) \citet{2005GCN..3332....1P};
(81) \citet{2005GCN..4221....1Q};
(82) \citet{2005Natur.437..845F};
(83) \citet{2005Natur.437..851G};
(84) \citet{2005Natur.438..988B};
(85) \citet{2006A&A...447..897J};
(86) \citet{2006A&A...455..423M};
(87) \citet{2006A&A...459L...5P};
(88) \citet{2006A&A...460L..13J};
(89) \citet{2006ApJ...636..391S};
(90) \citet{2006ApJ...642..979B};
(91) \citet{2006ApJ...643L..99M};
(92) \citet{2006ApJ...650..261S};
(93) \citet{2006ApJ...652.1011W};
(94) \citet{2006GCN..4539....1M};
(95) \citet{2006GCN..5104....1P};
(96) \citet{2006GCN..5170....1B};
(97) \citet{2006GCN..5217....1B};
(98) \citet{2006GCN..5238....1B};
(99) \citet{2006GCN..5387....1P};
(100) \citet{2006GCN..5715....1O};
(101) \citet{2006GCN..5946....1C};
(102) \citet{2006GCN..5952....1B};
(103) \citet{2006GCN..5962....1B};
(104) \citet{2006Natur.440..184K};
(105) \citet{2006Natur.444.1053G};
(106) \citet{2007A&A...461..485S};
(107) \citet{2007A&A...468...83V};
(108) \citet{2007A&A...475..101C};
(109) \citet{2007ApJ...660..504B};
(110) \citet{2007ApJ...661L.127M};
(111) \citet{2007ApJ...662.1129O};
(112) \citet{2007ApJ...664.1000B};
(113) \citet{2007ApJ...669....1R};
(114) \citet{2007ApJ...671..272C};
(115) \citet{2007ApJS..168..231P};
(116) \citet{2007GCN..6083....1C};
(117) \citet{2007GCN..6398....1J};
(118) \citet{2007GCN..6470....1B};
(119) \citet{2007GCN..6556....1C};
(120) \citet{2007GCN..6741....1T};
(121) \citet{2007GCN..6864....1P};
(122) \citet{2007GCN..6888....1C};
(123) \citet{2007GCN..6997....1J};
(124) \citet{2007GCN..7124....1C};
(125) \citet{2007GCN..7154....1B};
(126) \citet{2008A&A...481..319W};
(127) \citet{2008A&A...491..189F};
(128) \citet{2008A&A...491L..29R};
(129) \citet{2008ApJ...672..449P};
(130) \citet{2008ApJ...688..470P};
(131) \citet{2008GCN..7654....1C};
(132) \citet{2008GCN..7770....1F};
(133) \citet{2008GCN..7889....1P};
(134) \citet{2008GCN..8212....1H};
(135) \citet{2008GCN..8335....1B};
(136) \citet{2008GCN..8346....1C};
(137) \citet{2008GCN..8434....1B};
(138) \citet{2008GCN..8438....1D};
(139) \citet{2008GCN..8531....1D};
(140) \citet{2008GCN..8542....1B};
(141) \citet{2008GCN..8713....1C};
(142) \citet{2008arXiv0802.0874C};
(143) \citet{2009A&A...497..729F};
(144) \citet{2009A&A...498..711D};
(145) \citet{2009AJ....138.1690P};
(146) \citet{2009ApJ...690..231B};
(147) \citet{2009ApJ...693.1912G};
(148) \citet{2009ApJ...704..877B};
(149) \citet{2009ApJS..185..526F};
(150) \citet{2009GCN..10031...1C};
(151) \citet{2009GCN..10053...1X};
(152) \citet{2009GCN..10065...1C};
(153) \citet{2009GCN..10100...1C};
(154) \citet{2009GCN..10272...1P};
(155) \citet{2009GCN..8766....1D};
(156) \citet{2009GCN..8892....1F};
(157) \citet{2009GCN..8994....1C};
(158) \citet{2009GCN..9151....1C};
(159) \citet{2009GCN..9156....1B};
(160) \citet{2009GCN..9243....1C};
(161) \citet{2009GCN..9264....1L};
(162) \citet{2009GCN..9353....1R};
(163) \citet{2009GCN..9383....1d};
(164) \citet{2009GCN..9409....1T};
(165) \citet{2009GCN..9457....1M};
(166) \citet{2009GCN..9518....1C};
(167) \citet{2009GCN..9673....1W};
(168) \citet{2009GCN..9712....1F};
(169) \citet{2009GCN..9761....1M};
(170) \citet{2009GCN..9771....1d};
(171) \citet{2009GCN..9797....1J};
(172) \citet{2009GCN..9873....1C};
(173) \citet{2009GCN..9958....1L};
(174) \citet{2009MNRAS.395..490O};
(175) \citet{2009MNRAS.395L..21K};
(176) \citet{2009Natur.461.1254T};
(177) \citet{2010ApJ...708....9F};
(178) \citet{2010ApJ...720..862R};
(179) \citet{2010ApJ...725.1202L};
(180) \citet{2010GCN..10350...1R};
(181) \citet{2010GCN..10441...1G};
(182) \citet{2010GCN..10466...1C};
(183) \citet{2010GCN..10495...1V};
(184) \citet{2010GCN..10606...1C};
(185) \citet{2010GCN..10684...1G};
(186) \citet{2010GCN..10752...1C};
(187) \citet{2010GCN..10782...1A};
(188) \citet{2010GCN..11164...1C};
(189) \citet{2010GCN..11230...1T};
(190) \citet{2010GCN..11317...1F};
(191) \citet{2010MNRAS.406.2473P};
(192) \citet{2010MNRAS.408..383R};
(193) \citet{2011A&A...526A.153K};
(194) \citet{2011A&A...526A.154A};
(195) \citet{2011ApJ...730...26F};
(196) \citet{2011ApJ...732...29C};
(197) \citet{2011ApJ...735L..24S};
(198) \citet{2011ApJ...736....7C};
(199) \citet{2011GCN..11518...1C};
(200) \citet{2011GCN..11538...1C};
(201) \citet{2011GCN..11607...1S};
(202) \citet{2011GCN..11638...1C};
(203) \citet{2011GCN..11708...1M};
(204) \citet{2011GCN..11736...1C};
(205) \citet{2011GCN..11978...1D};
(206) \citet{2011GCN..11993...1D};
(207) \citet{2011GCN..12164...1P};
(208) \citet{2011GCN..12202...1C};
(209) \citet{2011GCN..12225...1T};
(210) \citet{2011GCN..12234...1C};
(211) \citet{2011GCN..12414...1L};
(212) \citet{2011GCN..12431...1W};
(213) \citet{2011GCN..12537...1C};
(214) \citet{2011GCN..12677...1V};
(215) \citet{2011GCN..12777...1C};
(216) \citet{2011MNRAS.411.2792S};
(217) \citet{2011MNRAS.413.2173G};
(218) \citet{2012ApJ...752...62J};
(219) \citet{2012ApJ...758...46K};
(220) \citet{2012ApJ...758..122P};
(221) \citet{2012GCN..13051...1D};
(222) \citet{2012GCN..13118...1T};
(223) \citet{2012GCN..13134...1K};
(224) \citet{2012GCN..13213...1C};
(225) \citet{2012GCN..13441...1T};
(226) \citet{2012GCN..13460...1X};
(227) \citet{2012GCN..13493...1G};
(228) \citet{2012GCN..13512...1C};
(229) \citet{2012GCN..13532...1T};
(230) \citet{2012GCN..13562...1T};
(231) \citet{2012GCN..13628...1T};
(232) \citet{2012GCN..13723...1S};
(233) \citet{2012GCN..13730...1H};
(234) \citet{2012GCN..13810...1K};
(235) \citet{2012GCN..14009...1T};
(236) \citet{2012GCN..14059...1P};
(237) \citet{2012GCN..14120...1F};
(238) \citet{2012arXiv1205.3779M};
(239) \citet{2013A&A...556A..23E};
(240) \citet{2013A&A...557L..18D};
(241) \citet{2013ApJ...769...56F};
(242) \citet{2013ApJ...774...26C};
(243) \citet{2013ApJ...775L...5K};
(244) \citet{2013ApJ...776...98X};
(245) \citet{2013ApJ...778..128P};
(246) \citet{2013GCN..14207...1C};
(247) \citet{2013GCN..14286...1F};
(248) \citet{2013GCN..14366...1T};
(249) \citet{2013GCN..14390...1K};
(250) \citet{2013GCN..14437...1D};
(251) \citet{2013GCN..14493...1F};
(252) \citet{2013GCN..14567...1T};
(253) \citet{2013GCN..14621...1C};
(254) \citet{2013GCN..14634...1S};
(255) \citet{2013GCN..14685...1S};
(256) \citet{2013GCN..14748...1C};
(257) \citet{2013GCN..14762...1C};
(258) \citet{2013GCN..14848...1S};
(259) \citet{2013GCN..14882...1T};
(260) \citet{2013GCN..15144...1C};
(261) \citet{2013GCN..15187...1D};
(262) \citet{2013GCN..15307...1C};
(263) \citet{2013GCN..15330...1R};
(264) \citet{2013GCN..15407...1X};
(265) \citet{2013GCN..15470...1D};
(266) \citet{2013GCN..15494...1H};
(267) \citet{2013GCN..15571...1G};
(268) \citet{2013GCN..15624...1C};
(269) \citet{2014A&A...565A.112H};
(270) \citet{2014A&A...569A..93J};
(271) \citet{2014A&A...572A..47R};
(272) \citet{2014ApJ...781....1L};
(273) \citet{2014ApJ...781...13L};
(274) \citet{2014GCN..15652...1C};
(275) \citet{2014GCN..15800...1M};
(276) \citet{2014GCN..15936...1J};
(277) \citet{2014GCN..15966...1C};
(278) \citet{2014GCN..16125...1T};
(279) \citet{2014GCN..16150...1T};
(280) \citet{2014GCN..16181...1P};
(281) \citet{2014GCN..16229...1M};
(282) \citet{2014GCN..16241...1M};
(283) \citet{2014GCN..16269...1C};
(284) \citet{2014GCN..16301...1C};
(285) \citet{2014GCN..16310...1D};
(286) \citet{2014MNRAS.442.2586V};
(287) \citet{2015A&A...581A.125K};
(288) \citet{2015ApJ...803L..24C};
(289) \citet{2015GCN..17988...1J-1};
(290) \citet{2015MNRAS.446.3911S};
(291) \citet{2015MNRAS.446.4116V};
(292) \citet{2015MNRAS.452.1535C};
(293) \citet{2015arXiv150402482P};
(294) \citet{Keck GRB Host project};
(295) \citet{Keck GRB Host project:};
}
\end{deluxetable}


==> tbprompt3.tex <==
\begin{deluxetable}{lllllllllllll}
\tabletypesize{\scriptsize}
%%\tabcolsep0.1in\footnotesize
\tablecolumns{10}
\tablewidth{0pc}
\tablecaption{prompt \label{tbprompt3}}
\tablehead {
\colhead{GRB}        &
\colhead{z} &
\colhead{$E_{iso} {\rm erg\ cm^{-2}}$ }      &
\colhead{$L_{p,iso} {\rm erg\ s^{-1}\ cm^{-2}}$}      &
\colhead{$f$} &
\colhead{$f_{\rm eff}$} &
\colhead{reference}      &\\
}

\startdata

140606B& $0.384$ & $4.6028962e+51$ & $1.8821922e+51$ & $...$ & $...$ & $0$ \\
140518A& $4.707$ & $7.9187400e+52$ & $2.8854648e+52$ & $1.18$ & $1.02\pm0.01$ & $0$ \\
140515A& $6.32$ & $7.0778147e+52$ & $5.2291156e+52$ & $1.21$ & $1.04\pm0.02$ & $0$ \\
140512A& $0.725$ & $5.6315257e+52$ & $6.7147110e+51$ & $1.78$ & $1.25\pm0.13$ & $0$ \\
140509A& $2.4$ & $4.3721742e+52$ & $1.6286230e+52$ & $...$ & $...$ & $0$ \\
140508A& $1.027$ & $2.2581757e+53$ & $6.7389433e+52$ & $...$ & $...$ & $0$ \\
140506A& $0.8893$ & $1.8334250e+52$ & $1.0099367e+52$ & $1.5$ & $1.13\pm0.06$ & $0$ \\
140430A& $1.6019$ & $1.5060891e+52$ & $5.7339402e+51$ & $1.44$ & $1.06\pm0.03$ & $0$ \\
140428A& $4.7$ & $3.6860092e+52$ & $3.1030486e+52$ & $...$ & $...$ & $0$ \\
140423A& $3.26$ & $5.4471181e+53$ & $6.1851154e+52$ & $1.19$ & $1.03\pm0.01$ & $0$ \\
140419A& $3.956$ & $1.4260154e+54$ & $5.7269762e+53$ & $1.63$ & $1.06\pm0.03$ & $0$ \\
140318A& $1.02$ & $3.4883404e+51$ & $1.0689195e+51$ & $1.14$ & $1.04\pm0.02$ & $0$ \\
140311A& $4.954$ & $2.2845721e+53$ & $6.0984523e+52$ & $...$ & $...$ & $0$ \\
140304A& $5.283$ & $1.2798250e+53$ & $1.0407695e+53$ & $1.3$ & $1.05\pm0.03$ & $0$ \\
140301A& $1.4155$ & $4.8225465e+51$ & $1.2249926e+51$ & $1.1$ & $1.02\pm0.01$ & $0$ \\
140226A& $1.98$ & $4.8121133e+52$ & $2.2022293e+52$ & $...$ & $...$ & $0$ \\
140213A& $1.2079$ & $1.0521632e+53$ & $3.6954526e+52$ & $3$ & $1.38\pm0.19$ & $0$ \\
140206A& $2.739$ & $2.9985832e+53$ & $1.8590868e+53$ & $4.38$ & $1.75\pm0.38$ & $0$ \\
140114A& $3$ & $1.2843573e+53$ & $8.9590540e+51$ & $...$ & $...$ & $0$ \\
131231A& $0.6427$ & $2.2108707e+53$ & $2.1767213e+52$ & $...$ & $...$ & $0$ \\
131227A& $5.3$ & $1.4243541e+53$ & $1.0318287e+53$ & $1.18$ & $1.03\pm0.01$ & $0$ \\
131117A& $4.042$ & $1.4424829e+52$ & $1.3371620e+52$ & $1.16$ & $1.04\pm0.02$ & $0$ \\
131108A& $2.4$ & $5.9539417e+53$ & $2.1441507e+53$ & $...$ & $...$ & $0$ \\
131105A& $1.6854$ & $2.2094881e+53$ & $2.7220906e+52$ & $1.1$ & $1.03\pm0.01$ & $0$ \\
131103A& $0.5960$ & $1.6533068e+51$ & $3.1694063e+50$ & $1.25$ & $1.09\pm0.04$ & $0$ \\
131030A& $1.293$ & $2.9685824e+53$ & $1.0313575e+53$ & $4.63$ & $1.25\pm0.13$ & $0$ \\
131011A& $1.874$ & $1.0545980e+53$ & $1.5939608e+52$ & $...$ & $...$ & $0$ \\
131004A& $0.717$ & $8.0131016e+50$ & $1.4783500e+51$ & $1.94$ & $1.94\pm0.16$ & $0$ \\
130925A& $0.3483$ & $3.2130940e+50$ & $8.5553649e+49$ & $1.81$ & $1.09\pm0.04$ & $0$ \\
130907A& $1.238$ & $2.9774617e+54$ & $1.8556747e+53$ & $4.75$ & $1.38\pm0.19$ & $0$ \\
130831A& $0.4791$ & $6.6299463e+51$ & $3.2257742e+51$ & $3.13$ & $1.25\pm0.13$ & $0$ \\
130702A& $0.145$ & $5.0540978e+50$ & $3.1486791e+49$ & $...$ & $...$ & $0$ \\
130701A& $1.1548$ & $2.2200916e+52$ & $3.5466500e+52$ & $2.13$ & $1.19\pm0.09$ & $0$ \\
130612A& $2.006$ & $9.1103010e+51$ & $9.2786264e+51$ & $1.23$ & $1.03\pm0.01$ & $0$ \\
130610A& $2.092$ & $5.1953169e+52$ & $1.3286078e+52$ & $1.23$ & $1.04\pm0.02$ & $0$ \\
130606A& $5.913$ & $2.0195018e+53$ & $2.5224360e+53$ & $1.44$ & $1.06\pm0.03$ & $0$ \\
130604A& $1.06$ & $1.3487475e+52$ & $1.3418874e+51$ & $1.13$ & $1.03\pm0.01$ & $0$ \\
130528A& $1.25$ & $5.3079541e+52$ & $6.0862047e+51$ & $1.38$ & $1.06\pm0.03$ & $0$ \\
130518A& $2.49$ & $1.7781063e+54$ & $6.0131017e+53$ & $...$ & $...$ & $0$ \\
130514A& $3.6$ & $5.7083774e+53$ & $5.6095781e+52$ & $...$ & $...$ & $0$ \\
130511A& $1.3033$ & $4.1816681e+51$ & $5.0075294e+51$ & $1.35$ & $1.05\pm0.03$ & $0$ \\
130505A& $2.27$ & $2.7646336e+54$ & $1.9929211e+54$ & $3$ & $1.5\pm0.25$ & $0$ \\
130427B& $2.78$ & $6.4945739e+52$ & $3.9500472e+52$ & $1.31$ & $1.11\pm0.06$ & $0$ \\
130427A& $0.3401$ & $1.1716380e+54$ & $1.8455484e+53$ & $42.5$ & $4.75\pm1.88$ & $0$ \\
130420A& $1.297$ & $6.5430828e+52$ & $5.4286569e+51$ & $1.38$ & $1.15\pm0.08$ & $0$ \\
130418A& $1.217$ & $9.3381809e+52$ & $3.2966158e+51$ & $1.05$ & $1.01\pm0.01$ & $0$ \\
130408A& $3.757$ & $2.7984820e+53$ & $5.7686975e+53$ & $1.21$ & $1.06\pm0.03$ & $0$ \\
130215A& $0.597$ & $4.1672048e+52$ & $2.1315527e+51$ & $1.08$ & $1.03\pm0.01$ & $0$ \\
130131B& $2.5393$ & $2.9825890e+52$ & $2.8139125e+52$ & $1.21$ & $1.08\pm0.04$ & $0$ \\
121229A& $2.707$ & $1.9722438e+52$ & $8.6973342e+50$ & $...$ & $...$ & $0$ \\
121212A& $...$ & $3.7941231e+51$ & $3.6311287e+51$ & $...$ & $...$ & $0$ \\
121211A& $1.023$ & $2.1815671e+51$ & $2.0583601e+51$ & $1.19$ & $1.05\pm0.03$ & $0$ \\
121209A& $2.1$ & $1.0941890e+53$ & $3.4373952e+52$ & $1.36$ & $1.05\pm0.03$ & $0$ \\
121201A& $3.3830$ & $3.8134202e+52$ & $1.1799988e+52$ & $1.18$ & $1.08\pm0.04$ & $0$ \\
121128A& $2.20$ & $1.2094588e+53$ & $5.3266430e+52$ & $2.75$ & $1.63\pm0.31$ & $0$ \\
121027A& $1.7732$ & $3.4634973e+52$ & $4.5351773e+51$ & $1.19$ & $1.02\pm0.01$ & $0$ \\
121024A& $2.3012$ & $5.0033675e+52$ & $1.6954290e+52$ & $1.24$ & $1.09\pm0.04$ & $0$ \\
120922A& $3.1$ & $2.0593619e+53$ & $2.5563837e+52$ & $1.2$ & $1.03\pm0.01$ & $0$ \\
120909A& $3.93$ & $3.7834884e+53$ & $9.4584451e+52$ & $1.16$ & $1.04\pm0.02$ & $0$ \\
120907A& $0.970$ & $2.5470037e+51$ & $3.1385244e+51$ & $1.29$ & $1.06\pm0.03$ & $0$ \\
120815A& $2.3587$ & $1.4718162e+52$ & $1.2392782e+52$ & $1.28$ & $1.1\pm0.05$ & $0$ \\
120811C& $2.671$ & $6.2417167e+52$ & $3.4472967e+52$ & $1.54$ & $1.06\pm0.03$ & $0$ \\
120805A& $3.1$ & $8.8164226e+52$ & $1.4696229e+52$ & $...$ & $...$ & $0$ \\
120802A& $3.796$ & $1.1528684e+53$ & $5.6739431e+52$ & $1.35$ & $1.1\pm0.05$ & $0$ \\
120729A& $0.80$ & $1.8880261e+52$ & $5.8719790e+51$ & $1.51$ & $1.11\pm0.05$ & $0$ \\
120724A& $1.48$ & $8.0953753e+51$ & $1.0193926e+51$ & $...$ & $...$ & $0$ \\
120722A& $0.9590$ & $6.3681925e+51$ & $7.1559851e+50$ & $1.09$ & $1.02\pm0.01$ & $0$ \\
120716A& $2.486$ & $2.9117856e+53$ & $7.9581911e+52$ & $...$ & $...$ & $0$ \\
120714B& $0.3985$ & $1.6128298e+51$ & $6.3343606e+49$ & $...$ & $...$ & $0$ \\
120712A& $4.1745$ & $1.7566205e+53$ & $1.2709407e+53$ & $1.41$ & $1.06\pm0.03$ & $0$ \\
120711A& $1.405$ & $1.8178837e+54$ & $1.7123057e+53$ & $...$ & $...$ & $0$ \\
120624B& $2.1974$ & $3.2081394e+54$ & $2.3165156e+53$ & $1.62$ & $1.09\pm0.05$ & $0$ \\
120521C& $6$ & $1.3473757e+53$ & $1.2516612e+53$ & $...$ & $...$ & $0$ \\
120422A& $0.2826$ & $2.9720989e+50$ & $8.9713537e+49$ & $1.13$ & $1.05\pm0.03$ & $0$ \\
120404A& $2.876$ & $6.1632192e+52$ & $1.2757254e+52$ & $1.09$ & $1.01\pm0.01$ & $0$ \\
120327A& $2.813$ & $1.8772258e+53$ & $6.5330870e+52$ & $1.69$ & $1.13\pm0.06$ & $0$ \\
120326A& $1.798$ & $3.1896105e+52$ & $1.5468316e+52$ & $1.58$ & $1.06\pm0.03$ & $0$ \\
120311A& $3$ & $1.3532943e+52$ & $3.2156202e+52$ & $...$ & $...$ & $0$ \\
120308A& $4.5$ & $1.0005495e+53$ & $2.1378191e+53$ & $...$ & $...$ & $0$ \\
120224A& $1.1$ & $1.7495042e+51$ & $7.7878320e+50$ & $...$ & $...$ & $0$ \\
120211A& $2.4$ & $3.3810502e+52$ & $6.0161106e+51$ & $1.15$ & $1.05\pm0.03$ & $0$ \\
120119A& $1.7291$ & $3.5627820e+53$ & $5.6373092e+52$ & $2.33$ & $1.14\pm0.07$ & $0$ \\
120118B& $2.9428$ & $5.6473146e+52$ & $1.6109908e+52$ & $1.22$ & $1.04\pm0.02$ & $0$ \\
111229A& $1.3805$ & $3.6848206e+51$ & $1.8370042e+51$ & $1.17$ & $1.13226\pm0.43$ & $1$ \\
111228A& $0.7164$ & $3.9109946e+52$ & $4.2713643e+51$ & $1.62$ & $1.29847\pm0.19$ & $1$ \\
111225A& $2.012$ & $3.0831420e+52$ & $3.9060721e+51$ & $1.16$ & $1.12778\pm0.16$ & $1$ \\
111215A& $2.06$ & $1.1111384e+53$ & $2.9511015e+51$ & $...$ & $...$ & $0$ \\
111211A& $0.4786$ & $1.4889114e+52$ & $9.0408789e+51$ & $...$ & $...$ & $0$ \\
111209A& $0.6770$ & $8.0260402e+53$ & $2.8181410e+50$ & $...$ & $...$ & $0$ \\
111129A& $1.0796$ & $1.6537800e+51$ & $9.4041538e+50$ & $1.1$ & $1.1\pm0.12$ & $1$ \\
111123A& $3.1513$ & $3.6791445e+53$ & $1.4862159e+52$ & $1.17$ & $1.13226\pm0.16$ & $1$ \\
111107A& $2.893$ & $2.0464860e+52$ & $2.9529536e+52$ & $1.21$ & $1.14977\pm0.23$ & $1$ \\
111008A& $4.9898$ & $3.9332986e+53$ & $3.6648379e+53$ & $1.52$ & $1.26667\pm0.03$ & $1$ \\
111005A& $0.0133$ & $5.3901341e+47$ & $6.1204802e+46$ & $1.24$ & $1.1625\pm0.07$ & $1$ \\
110918A& $0.9843$ & $1.8369018e+54$ & $4.2281584e+54$ & $...$ & $...$ & $0$ \\
110818A& $3.3609$ & $1.7074394e+53$ & $6.0451441e+52$ & $1.26$ & $1.1708\pm0.14$ & $1$ \\
110808A& $1.3490$ & $5.7405851e+52$ & $9.2706862e+53$ & $1.05$ & $1.07561\pm0.11$ & $1$ \\
110801A& $1.858$ & $9.6454444e+52$ & $5.0900993e+51$ & $1.09$ & $1.09522\pm0.24$ & $1$ \\
110731A& $2.83$ & $4.9059014e+53$ & $3.1638766e+53$ & $3.5$ & $1.24576\pm0.29$ & $1$ \\
110726A& $1.036$ & $1.2666437e+51$ & $7.5910227e+50$ & $1.25$ & $1.16667\pm0.07$ & $1$ \\
110715A& $0.82$ & $4.8074887e+52$ & $4.1846054e+52$ & $9.7$ & $1.15085\pm0.01$ & $1$ \\
110709B& $2.09$ & $2.6937648e+53$ & $3.5215795e+53$ & $1.52$ & $1.26667\pm0.21$ & $1$ \\
110503A& $1.613$ & $1.7982911e+53$ & $1.9880108e+53$ & $3.12$ & $1.27969\pm0.12$ & $1$ \\
110422A& $1.770$ & $7.2018251e+53$ & $2.7965966e+53$ & $4$ & $1.29231\pm0.16$ & $1$ \\
110213B& $1.083$ & $8.0783004e+52$ & $2.9468454e+51$ & $...$ & $...$ & $0$ \\
110213A& $1.46$ & $7.3435439e+52$ & $2.8961538e+52$ & $1.35$ & $1.20638\pm0.27$ & $1$ \\
110205A& $2.22$ & $6.0987798e+53$ & $2.7364525e+52$ & $1.54$ & $1.27323\pm0.11$ & $1$ \\
110128A& $2.339$ & $2.3062508e+52$ & $9.7036374e+51$ & $1.12$ & $1.10943\pm0.29$ & $1$ \\
110106B& $0.618$ & $5.3352361e+51$ & $6.6823161e+50$ & $1.15$ & $1.12326\pm0.01$ & $1$ \\
101225A& $0.847$ & $8.2103286e+51$ & $1.6233672e+49$ & $...$ & $...$ & $0$ \\
101219B& $0.55185$ & $4.4737920e+51$ & $2.5866201e+50$ & $...$ & $...$ & $0$ \\
100906A& $1.727$ & $2.6060140e+53$ & $5.1760976e+52$ & $2.35$ & $1.47313\pm0.05$ & $1$ \\
100901A& $1.408$ & $3.3777869e+52$ & $2.6105526e+51$ & $1.1$ & $1.1\pm0.2$ & $1$ \\
100814A& $1.4392$ & $9.3933130e+52$ & $9.9955859e+51$ & $1.75$ & $1.33636\pm0.07$ & $1$ \\
100802A& $3.1$ & $4.1739812e+52$ & $1.6711393e+52$ & $1.24$ & $1.1625\pm0.27$ & $1$ \\
100728B& $2.106$ & $4.8620742e+52$ & $3.6503314e+52$ & $1.25$ & $1.16667\pm0.09$ & $1$ \\
100728A& $1.5670$ & $9.4690119e+53$ & $3.9247296e+52$ & $2.37$ & $1.47685\pm0.38$ & $1$ \\
100724A& $1.2890$ & $1.4860394e+51$ & $2.7429215e+51$ & $1.38$ & $1.38\pm0.21$ & $1$ \\
100621A& $0.5426$ & $4.3871766e+52$ & $3.1958388e+51$ & $4.11$ & $1.21392\pm0.11$ & $1$ \\
100615A& $1.3978$ & $7.1521988e+52$ & $1.8810050e+52$ & $1.87$ & $1.36829\pm0.21$ & $1$ \\
100606A& $1.5545$ & $2.9411088e+53$ & $4.8160657e+52$ & $1.75$ & $1.33636\pm0.14$ & $1$ \\
100518A& $4$ & $5.5154036e+52$ & $4.9521156e+52$ & $...$ & $...$ & $0$ \\
100513A& $4.772$ & $1.3952819e+53$ & $2.8013301e+52$ & $1.15$ & $1.12326\pm0.16$ & $1$ \\
100508A& $0.5201$ & $2.8693894e+51$ & $2.2369195e+50$ & $...$ & $...$ & $0$ \\
100425A& $1.755$ & $9.4185364e+51$ & $4.2312295e+51$ & $1.175$ & $1.13448\pm0.34$ & $1$ \\
100424A& $2.4656$ & $4.5401228e+52$ & $3.0277871e+51$ & $...$ & $...$ & $0$ \\
100418A& $0.6235$ & $7.6628711e+50$ & $2.1475553e+50$ & $1.12$ & $1.10943\pm0.12$ & $1$ \\
100414A& $1.368$ & $5.6293755e+53$ & $3.2986995e+52$ & $...$ & $...$ & $0$ \\
100316D& $0.0592$ & $5.7396503e+48$ & $1.1315130e+47$ & $...$ & $...$ & $0$ \\
100316B& $1.180$ & $1.6489192e+51$ & $1.3303074e+51$ & $1.31$ & $1.19091\pm0.12$ & $1$ \\
100302A& $4.813$ & $2.8206935e+52$ & $2.0434558e+52$ & $1.25$ & $1.16667\pm0.34$ & $1$ \\
100219A& $4.6667$ & $5.5763567e+52$ & $3.0171783e+52$ & $1.17$ & $1.13226\pm0.1$ & $1$ \\
091208B& $1.0633$ & $2.8049919e+52$ & $2.0298703e+52$ & $1.8125$ & $1.5225\pm0.16$ & $1$ \\
091127A& $0.4904$ & $1.8626071e+52$ & $6.2383126e+51$ & $2.25$ & $1.70243\pm0.03$ & $1$ \\
091109A& $3.076$ & $1.4248573e+53$ & $3.5058787e+52$ & $...$ & $...$ & $0$ \\
091029A& $2.752$ & $9.5034024e+52$ & $1.7189666e+52$ & $...$ & $...$ & $0$ \\
091024A& $1.092$ & $5.1508245e+52$ & $1.0148987e+52$ & $...$ & $...$ & $0$ \\
091020A& $1.71$ & $6.8451170e+52$ & $1.8099910e+52$ & $1.6$ & $1.09268\pm0.06$ & $1$ \\
091018A& $0.9710$ & $7.0667531e+51$ & $4.1785711e+51$ & $2.3125$ & $1.3875\pm0.12$ & $1$ \\
091003A& $0.8969$ & $7.1707843e+52$ & $2.9274666e+52$ & $...$ & $...$ & $0$ \\
090927A& $1.37$ & $1.8282907e+51$ & $4.5879533e+51$ & $1.475$ & $...$ & $1$ \\
090926B& $1.2427$ & $4.4799495e+52$ & $3.8927965e+51$ & $1.5$ & $1.09565\pm0.05$ & $1$ \\
090926A& $2.1062$ & $1.9832293e+54$ & $6.5531284e+53$ & $...$ & $...$ & $0$ \\
090902B& $1.822$ & $3.0471058e+54$ & $7.8036630e+53$ & $...$ & $...$ & $0$ \\
090814A& $0.696$ & $3.6764254e+51$ & $2.1111366e+50$ & $...$ & $...$ & $0$ \\
090812A& $2.452$ & $4.4523105e+53$ & $8.1381486e+52$ & $1.5$ & $1.10526\pm0.1$ & $1$ \\
090809A& $2.737$ & $2.4814919e+52$ & $2.1554239e+52$ & $1.3$ & $...$ & $1$ \\
090726A& $2.71$ & $3.1681798e+52$ & $5.4079709e+51$ & $...$ & $...$ & $0$ \\
090715B& $3.00$ & $2.0983716e+53$ & $8.1227288e+52$ & $1.5625$ & $1.09375\pm0.07$ & $1$ \\
090709A& $1.7$ & $4.0875025e+52$ & $2.4577569e+51$ & $2.5$ & $1.27273\pm0.03$ & $1$ \\
090618A& $0.54$ & $2.8004938e+53$ & $1.2555784e+52$ & $7.5$ & $1.23336\pm0.03$ & $1$ \\
090530A& $1.266$ & $1.2696336e+52$ & $5.3293269e+51$ & $1.5$ & $1.3125\pm0.09$ & $1$ \\
090529A& $2.625$ & $2.1863139e+52$ & $3.0014850e+51$ & $...$ & $...$ & $0$ \\
090519A& $3.85$ & $2.6629949e+53$ & $1.0303792e+53$ & $...$ & $...$ & $0$ \\
090516A& $4.109$ & $7.3085617e+53$ & $8.6563951e+52$ & $...$ & $...$ & $0$ \\
090429B& $9.2$ & $6.0949332e+52$ & $1.9404051e+53$ & $1.3325$ & $1.25\pm0.12$ & $1$ \\
090424A& $0.544$ & $4.1371760e+52$ & $1.6471143e+52$ & $11.25$ & $1.18125\pm0.11$ & $1$ \\
090423A& $8.23$ & $7.8948141e+52$ & $1.1437631e+53$ & $1.3125$ & $1.21702\pm0.11$ & $1$ \\
090418A& $1.608$ & $1.6208777e+53$ & $1.2398685e+52$ & $...$ & $...$ & $0$ \\
090417B& $0.345$ & $1.5666212e+51$ & $1.6856844e+49$ & $...$ & $...$ & $0$ \\
090407A& $1.4478$ & $1.4144214e+52$ & $1.4509500e+51$ & $1.1375$ & $1.0736\pm0.07$ & $1$ \\
090328A& $0.7357$ & $9.2304540e+52$ & $1.3589252e+52$ & $...$ & $...$ & $0$ \\
090323A& $3.5832$ & $3.9644160e+54$ & $3.2394370e+53$ & $...$ & $...$ & $0$ \\
090313A& $3.375$ & $6.8020897e+52$ & $1.1626059e+52$ & $...$ & $...$ & $0$ \\
090205A& $4.6497$ & $1.5374740e+52$ & $1.3482579e+52$ & $1.187$ & $...$ & $1$ \\
090201A& $2.1000$ & $8.0038575e+53$ & $2.6953466e+53$ & $2$ & $1.2\pm0.14$ & $1$ \\
090113A& $1.7494$ & $1.6616931e+52$ & $1.2540848e+52$ & $1.5$ & $1.18868\pm0.16$ & $1$ \\
090102A& $1.547$ & $2.3508670e+53$ & $4.8004486e+52$ & $...$ & $...$ & $0$ \\
081230A& $2.03$ & $1.7313072e+52$ & $3.0616189e+51$ & $...$ & $...$ & $0$ \\
081228A& $3.44$ & $4.4768834e+51$ & $8.1172601e+51$ & $1.35484$ & $1.176\pm0.34$ & $1$ \\
081222A& $2.77$ & $2.4034230e+53$ & $1.2212816e+53$ & $2.3125$ & $1.19907\pm0.12$ & $1$ \\
081221A& $2.2590$ & $3.9462215e+53$ & $8.3021276e+52$ & $3.75$ & $1.20229\pm0.16$ & $1$ \\
081210A& $2.0631$ & $6.7121312e+52$ & $2.4742813e+52$ & $1.45$ & $1.218\pm0.06$ & $1$ \\
081203A& $2.05$ & $3.3822417e+53$ & $3.2740339e+52$ & $1.5$ & $1.15596\pm0.12$ & $1$ \\
081128A& $4$ & $1.4195376e+53$ & $2.5911611e+52$ & $1.1875$ & $1.09615\pm0.23$ & $1$ \\
081121A& $2.512$ & $2.8375606e+53$ & $8.6457708e+52$ & $1.14118$ & $1.10706\pm0.34$ & $1$ \\
081118A& $2.58$ & $3.7992073e+52$ & $4.1194145e+51$ & $...$ & $...$ & $0$ \\
081109A& $0.9785$ & $3.3091949e+52$ & $3.4559130e+51$ & $1.31429$ & $1.07333\pm0.1$ & $1$ \\
081029A& $3.8479$ & $2.0341676e+53$ & $2.0294838e+52$ & $...$ & $...$ & $0$ \\
081028A& $3.038$ & $3.5080114e+53$ & $1.7131302e+52$ & $...$ & $...$ & $0$ \\
081008A& $1.967$ & $1.3029506e+53$ & $1.3255802e+52$ & $1.3125$ & $1.16053\pm0.25$ & $1$ \\
081007A& $0.5295$ & $1.4797417e+51$ & $4.5325496e+50$ & $1.35$ & $1.26\pm0.03$ & $1$ \\
080928A& $1.6919$ & $1.3708649e+52$ & $1.0153389e+52$ & $1.375$ & $1.21579\pm0.07$ & $1$ \\
080916C& $4.35$ & $2.7181075e+54$ & $7.0134960e+53$ & $...$ & $...$ & $0$ \\
080916A& $0.6887$ & $1.8086470e+52$ & $2.5486208e+51$ & $1.5$ & $1.14545\pm0.03$ & $1$ \\
080913A& $6.7$ & $6.3720057e+52$ & $1.2513551e+53$ & $1.256$ & $1.186\pm0.09$ & $1$ \\
080906A& $2.0$ & $9.3992576e+52$ & $6.6199120e+51$ & $1.23529$ & $1.1025\pm0.27$ & $1$ \\
080905B& $2.3739$ & $4.6881162e+52$ & $1.7804066e+52$ & $1.2625$ & $1.11632\pm0.09$ & $1$ \\
080825B& $4.31$ & $3.5940676e+53$ & $2.9567534e+53$ & $...$ & $...$ & $0$ \\
080810A& $3.3604$ & $3.5364850e+53$ & $1.0534185e+53$ & $...$ & $...$ & $0$ \\
080805A& $1.5052$ & $4.4648592e+52$ & $4.1328767e+51$ & $1.225$ & $1.11848\pm0.14$ & $1$ \\
080804A& $2.2059$ & $1.5546458e+53$ & $4.2916063e+52$ & $1.5$ & $1.09565\pm0.11$ & $1$ \\
080721A& $2.5914$ & $1.1960634e+54$ & $1.0046853e+54$ & $4.8125$ & $1.33858\pm0.07$ & $1$ \\
080710A& $0.8454$ & $9.3389662e+51$ & $1.0528554e+51$ & $1.11446$ & $1.1037\pm0.01$ & $1$ \\
080707A& $1.2322$ & $4.7939787e+51$ & $1.5436752e+51$ & $1.25$ & $1.10526\pm0.21$ & $1$ \\
080703A& $...$ & $5.8740749e+51$ & $7.3991245e+51$ & $...$ & $...$ & $0$ \\
080607A& $3.0368$ & $1.7552252e+54$ & $2.1343758e+54$ & $5.60417$ & $1.20191\pm0.07$ & $1$ \\
080605A& $1.6408$ & $2.3136072e+53$ & $3.2369663e+53$ & $1.42$ & $1.11269\pm0.43$ & $1$ \\
080604A& $1.4171$ & $9.4921771e+51$ & $8.5514698e+50$ & $...$ & $...$ & $0$ \\
080603B& $2.6892$ & $9.5590203e+52$ & $1.1833413e+53$ & $1.65$ & $1.1088\pm0.19$ & $1$ \\
080603A& $1.688$ & $1.8762905e+52$ & $2.3944618e+51$ & $...$ & $...$ & $0$ \\
080602A& $1.8204$ & $8.7340914e+52$ & $5.9717894e+52$ & $1.25$ & $1.07143\pm0.16$ & $1$ \\
080523A& $3$ & $4.2466396e+52$ & $7.7291421e+51$ & $1.1$ & $1.07442\pm0.29$ & $1$ \\
080520A& $1.5457$ & $1.3510256e+51$ & $1.7098984e+51$ & $1.325$ & $...$ & $1$ \\
080517A& $0.089$ & $3.3740448e+49$ & $3.2947838e+48$ & $...$ & $...$ & $0$ \\
080515A& $2.47$ & $5.4263908e+52$ & $2.2181828e+52$ & $1.125$ & $1.0678\pm0.34$ & $1$ \\
080514B& $1.8$ & $2.5760460e+53$ & $4.6225271e+53$ & $...$ & $...$ & $0$ \\
080430A& $0.767$ & $4.5687980e+51$ & $1.3439085e+51$ & $1.4625$ & $1.11682\pm0.12$ & $1$ \\
080413B& $1.1012$ & $2.3721599e+52$ & $2.1471186e+52$ & $2.375$ & $1.53462\pm0.16$ & $1$ \\
080413A& $2.4330$ & $1.7426652e+53$ & $5.9825698e+52$ & $1.75$ & $1.13077\pm0.06$ & $1$ \\
080411A& $1.0301$ & $2.3503784e+53$ & $9.7098954e+52$ & $6.85$ & $1.13045\pm0.03$ & $1$ \\
080330A& $1.5119$ & $5.7708526e+51$ & $2.0984474e+51$ & $1.1875$ & $1.10833\pm0.23$ & $1$ \\
080325A& $1.78$ & $9.5986868e+52$ & $6.0175521e+51$ & $...$ & $...$ & $0$ \\
080320A& $...$ & $6.3380906e+51$ & $3.3006865e+51$ & $1.125$ & $1.08621\pm0.05$ & $1$ \\
080319C& $1.9492$ & $1.3627224e+53$ & $8.9756346e+52$ & $1.525$ & $1.08559\pm0.34$ & $1$ \\
080319B& $0.9382$ & $1.3329219e+54$ & $9.8009238e+52$ & $8$ & $1.10818\pm0.27$ & $1$ \\
080319A& $2.43$ & $1.7716543e+53$ & $2.2395303e+52$ & $1.17949$ & $1.07333\pm0.1$ & $1$ \\
080310A& $2.4274$ & $7.4258415e+52$ & $7.9741960e+51$ & $1.1875$ & $1.07258\pm0.07$ & $1$ \\
080307A& $...$ & $1.9065949e+52$ & $1.9603370e+51$ & $...$ & $...$ & $0$ \\
080212A& $...$ & $5.7578347e+52$ & $5.4185702e+51$ & $...$ & $...$ & $0$ \\
080210A& $2.6419$ & $6.3298328e+52$ & $1.5370847e+52$ & $1.225$ & $1.09468\pm0.03$ & $1$ \\
080207A& $2.0856$ & $1.5562192e+53$ & $5.7990757e+51$ & $...$ & $...$ & $0$ \\
080205A& $2.72$ & $7.2184603e+52$ & $1.0968947e+52$ & $1.1875$ & $1.09016\pm0.07$ & $1$ \\
080129A& $4.349$ & $1.1970941e+53$ & $1.2684855e+52$ & $...$ & $...$ & $0$ \\
071122A& $1.14$ & $4.6162024e+51$ & $5.1104681e+50$ & $...$ & $...$ & $0$ \\
071117A& $1.3308$ & $4.0903286e+52$ & $1.0872379e+53$ & $2.4$ & $1.44\pm0.16$ & $1$ \\
071112C& $0.8227$ & $4.1372216e+52$ & $1.8333820e+52$ & $...$ & $...$ & $0$ \\
071031A& $2.692$ & $3.7856631e+52$ & $4.2507204e+51$ & $1.125$ & $1.07386\pm0.09$ & $1$ \\
071025A& $4.8$ & $5.6063097e+53$ & $5.9287583e+52$ & $1.25$ & $1.09375\pm0.38$ & $1$ \\
071021A& $2.4515$ & $4.2959975e+52$ & $6.2368264e+51$ & $1.125$ & $1.08621\pm0.14$ & $1$ \\
071020A& $2.1462$ & $9.3826365e+52$ & $2.3125641e+53$ & $2.25$ & $...$ & $1$ \\
071010B& $0.947$ & $1.7206817e+52$ & $6.2377591e+51$ & $2.25$ & $1.35\pm0.24$ & $1$ \\
071010A& $0.98$ & $1.1676156e+51$ & $5.1502254e+50$ & $1.10526$ & $1.08088\pm0.29$ & $1$ \\
071003A& $1.60435$ & $3.4719932e+53$ & $2.0736068e+53$ & $1.575$ & $1.18125\pm0.11$ & $1$ \\
070810A& $2.17$ & $1.5704482e+52$ & $9.3622150e+51$ & $1.4$ & $1.176\pm0.14$ & $1$ \\
070808A& $...$ & $3.8897130e+52$ & $1.6633936e+52$ & $1.4125$ & $1.1865\pm0.43$ & $1$ \\
070802A& $2.4538$ & $8.6058381e+51$ & $3.1451717e+51$ & $...$ & $...$ & $0$ \\
070721B& $3.6298$ & $4.4753633e+53$ & $9.1377691e+52$ & $1.375$ & $1.1\pm0.16$ & $1$ \\
070714A& $1.58$ & $2.9457416e+51$ & $4.6090404e+51$ & $1.50495$ & $1.50495\pm0.21$ & $1$ \\
070621A& $5.5$ & $5.5519282e+53$ & $1.7372473e+53$ & $...$ & $...$ & $0$ \\
070612A& $0.617$ & $2.9463866e+52$ & $6.5729792e+50$ & $1.125$ & $1.09884\pm0.06$ & $1$ \\
070611A& $2.0394$ & $9.9161791e+51$ & $5.0380419e+51$ & $1.14375$ & $1.08559\pm0.12$ & $1$ \\
070529A& $2.4996$ & $1.5196412e+53$ & $2.6085971e+52$ & $...$ & $...$ & $0$ \\
070521A& $2.0865$ & $2.4712069e+53$ & $1.7361771e+53$ & $2.2875$ & $1.22389\pm0.05$ & $1$ \\
070518A& $1.161$ & $1.2322460e+51$ & $6.7331338e+50$ & $1.2$ & $1.12\pm0.1$ & $1$ \\
070508A& $0.82$ & $9.5957298e+52$ & $3.6512114e+52$ & $4.375$ & $1.17038\pm0.25$ & $1$ \\
070506A& $2.3090$ & $6.1087518e+51$ & $7.0997048e+51$ & $1.33333$ & $...$ & $1$ \\
070419B& $1.9586$ & $1.7844103e+53$ & $8.2091868e+51$ & $1.2375$ & $1.09421\pm0.16$ & $1$ \\
070419A& $0.9705$ & $4.1927148e+51$ & $8.6316733e+49$ & $...$ & $...$ & $0$ \\
070411A& $2.9538$ & $1.1822420e+53$ & $1.2173051e+52$ & $1.1125$ & $1.07414\pm0.09$ & $1$ \\
070330A& $...$ & $3.7283449e+51$ & $3.3349759e+51$ & $1.2125$ & $1.08351\pm0.38$ & $1$ \\
070328A& $2.0627$ & $5.2913221e+53$ & $1.2447092e+53$ & $1.725$ & $1.22797\pm0.14$ & $1$ \\
070318A& $0.8401$ & $1.7913945e+52$ & $2.0269993e+51$ & $1.31875$ & $1.08603\pm0.11$ & $1$ \\
070306A& $1.4965$ & $7.9147385e+52$ & $1.1914416e+52$ & $1.375$ & $1.08962\pm0.24$ & $1$ \\
070224A& $1.9922$ & $7.6620241e+51$ & $1.3990866e+51$ & $1.10625$ & $1.08684\pm0.29$ & $1$ \\
070223A& $1.6295$ & $2.4928967e+52$ & $1.8944456e+51$ & $...$ & $...$ & $0$ \\
070208A& $1.165$ & $3.3972989e+51$ & $9.9656545e+50$ & $1.16176$ & $1.09145\pm0.01$ & $1$ \\
070129A& $2.3384$ & $7.9041501e+52$ & $3.1153226e+51$ & $...$ & $...$ & $0$ \\
070125A& $1.547$ & $9.2131735e+53$ & $3.0343905e+53$ & $...$ & $...$ & $0$ \\
070110A& $2.3523$ & $5.7915995e+52$ & $5.9315767e+51$ & $...$ & $...$ & $0$ \\
070103A& $2.6208$ & $1.0879549e+52$ & $8.0657232e+51$ & $...$ & $...$ & $0$ \\
061222B& $3.355$ & $1.0839994e+53$ & $1.8093001e+52$ & $...$ & $...$ & $0$ \\
061222A& $2.088$ & $3.1111770e+53$ & $2.0406514e+53$ & $2.625$ & $1.55282\pm0.32$ & $1$ \\
061202A& $2.2543$ & $1.1395621e+53$ & $2.2451000e+52$ & $1.425$ & $1.08818\pm0.43$ & $1$ \\
061126A& $1.1588$ & $9.0535221e+52$ & $6.1748822e+52$ & $2.125$ & $1.275\pm0.19$ & $1$ \\
061121A& $1.3145$ & $2.6413304e+53$ & $1.3800882e+53$ & $4.8125$ & $1.3475\pm0.16$ & $1$ \\
061110B& $3.4344$ & $2.4782742e+53$ & $3.5004099e+52$ & $...$ & $...$ & $0$ \\
061110A& $0.7578$ & $4.6355035e+51$ & $2.0911536e+50$ & $1.325$ & $1.07019\pm0.29$ & $1$ \\
061021A& $0.3453$ & $5.4454205e+51$ & $2.0337085e+51$ & $2.0625$ & $1.28333\pm0.34$ & $1$ \\
061007A& $1.2622$ & $9.8416430e+53$ & $1.7435478e+53$ & $3.625$ & $1.19882\pm0.16$ & $1$ \\
060927A& $5.4636$ & $1.0975733e+53$ & $1.2051305e+53$ & $1.4625$ & $1.10676\pm0.12$ & $1$ \\
060926A& $3.2090$ & $1.3859510e+52$ & $1.5878204e+52$ & $1.2125$ & $...$ & $1$ \\
060923C& $...$ & $3.4500803e+52$ & $3.4940304e+51$ & $...$ & $...$ & $0$ \\
060923B& $1.5094$ & $7.8543219e+51$ & $2.9765572e+51$ & $...$ & $...$ & $0$ \\
060923A& $2.6$ & $3.2174964e+52$ & $1.4083859e+52$ & $1.25$ & $1.09375\pm0.23$ & $1$ \\
060912A& $0.9362$ & $7.6184994e+51$ & $7.2071118e+51$ & $1.9375$ & $1.40302\pm0.34$ & $1$ \\
060908A& $1.8836$ & $6.3284158e+52$ & $1.6126170e+52$ & $1.6$ & $1.12\pm0.1$ & $1$ \\
060906A& $3.6856$ & $1.2202450e+53$ & $3.2190896e+52$ & $...$ & $...$ & $0$ \\
060904B& $0.7029$ & $6.1461282e+51$ & $1.3320671e+51$ & $1.5$ & $1.18868\pm0.07$ & $1$ \\
060814A& $1.9223$ & $3.5075505e+53$ & $8.1162620e+52$ & $2.15278$ & $1.10941\pm0.09$ & $1$ \\
060807A& $...$ & $2.3099135e+52$ & $5.5948921e+51$ & $1.125$ & $1.08\pm0.07$ & $1$ \\
060805A& $2.3633$ & $1.9985472e+51$ & $2.0257219e+51$ & $...$ & $...$ & $0$ \\
060729A& $0.5429$ & $4.8623700e+51$ & $2.5536922e+50$ & $1.26829$ & $1.10303\pm0.16$ & $1$ \\
060719A& $1.5318$ & $1.9218133e+52$ & $4.7901958e+51$ & $1.375$ & $1.11058\pm0.27$ & $1$ \\
060714A& $2.7108$ & $9.6596707e+52$ & $1.0934948e+52$ & $...$ & $...$ & $0$ \\
060708A& $1.92$ & $1.1041213e+52$ & $9.9932260e+51$ & $1.4375$ & $1.2075\pm0.38$ & $1$ \\
060707A& $3.4246$ & $7.4972620e+52$ & $1.4959067e+52$ & $1.16216$ & $1.075\pm0.14$ & $1$ \\
060614A& $0.125$ & $2.1277555e+51$ & $2.6336827e+50$ & $2.5625$ & $2.2625\pm0.23$ & $1$ \\
060607A& $3.0749$ & $1.7174221e+53$ & $3.4718244e+52$ & $1.25$ & $1.07143\pm0.11$ & $1$ \\
060605A& $3.773$ & $5.4347537e+52$ & $1.4278230e+52$ & $1.21333$ & $1.11105\pm0.24$ & $1$ \\
060604A& $2.1355$ & $9.1378858e+51$ & $1.5501311e+51$ & $...$ & $...$ & $0$ \\
060602A& $0.787$ & $1.5399615e+52$ & $6.3242679e+50$ & $...$ & $...$ & $0$ \\
060526A& $3.2213$ & $5.6342323e+52$ & $2.0164615e+52$ & $1.35$ & $1.09038\pm0.29$ & $1$ \\
060522A& $5.11$ & $1.3495589e+53$ & $3.3061197e+52$ & $...$ & $...$ & $0$ \\
060512A& $0.4428$ & $3.2506240e+50$ & $9.7288108e+49$ & $1.15$ & $1.07333\pm0.11$ & $1$ \\
060510B& $4.9$ & $3.5858709e+53$ & $2.3920822e+52$ & $...$ & $...$ & $0$ \\
060505A& $0.0889$ & $9.2378497e+49$ & $2.5114909e+49$ & $1.58$ & $1.26667\pm0.25$ & $1$ \\
060502A& $1.5026$ & $4.9338917e+52$ & $8.9559537e+51$ & $1.3125$ & $1.1025\pm0.32$ & $1$ \\
060418A& $1.4901$ & $1.1625983e+53$ & $1.7700526e+52$ & $1.9375$ & $1.3125\pm0.29$ & $1$ \\
060319A& $1.172$ & $2.3018185e+51$ & $1.1418914e+51$ & $1.2375$ & $1.155\pm0.16$ & $1$ \\
060306A& $1.5597$ & $2.9687890e+52$ & $1.5675535e+52$ & $2.25$ & $1.512\pm0.12$ & $1$ \\
060223A& $4.406$ & $5.5266943e+52$ & $4.4592999e+52$ & $1.44737$ & $1.19814\pm0.05$ & $1$ \\
060218A& $0.03351$ & $9.3333895e+48$ & $8.6535438e+46$ & $...$ & $...$ & $0$ \\
060210A& $3.9122$ & $6.4850934e+53$ & $9.4990902e+52$ & $1.58333$ & $1.1644\pm0.1$ & $1$ \\
060206A& $4.0559$ & $5.5576582e+52$ & $6.6288907e+52$ & $1.5625$ & $...$ & $1$ \\
060204B& $2.3393$ & $8.3146259e+52$ & $9.7604032e+51$ & $1.25641$ & $1.07187\pm0.07$ & $1$ \\
060202A& $0.785$ & $8.6632343e+51$ & $2.8767925e+50$ & $...$ & $...$ & $0$ \\
060124A& $2.3$ & $2.1053479e+53$ & $1.2923597e+53$ & $3.375$ & $1.33726\pm0.2$ & $1$ \\
060123A& $0.56$ & $5.4277835e+50$ & $7.7711608e+48$ & $...$ & $...$ & $0$ \\
060115A& $3.5328$ & $1.4710756e+53$ & $2.6724218e+52$ & $1.15$ & $1.07333\pm0.07$ & $1$ \\
060111A& $2.32$ & $3.1790248e+52$ & $1.1697752e+52$ & $1.52941$ & $1.1375\pm0.16$ & $1$ \\
060108A& $2.03$ & $7.6912649e+51$ & $3.0715078e+51$ & $1.20513$ & $1.09666\pm0.38$ & $1$ \\
051117B& $0.4805$ & $3.3404745e+50$ & $1.0738958e+50$ & $1.15$ & $1.07675\pm0.29$ & $1$ \\
051111A& $1.55$ & $1.1236570e+53$ & $1.6529158e+52$ & $1.34375$ & $1.075\pm0.01$ & $1$ \\
051109B& $0.080$ & $6.7805663e+48$ & $1.1340947e+48$ & $1.1625$ & $1.085\pm0.21$ & $1$ \\
051109A& $2.346$ & $8.2773433e+52$ & $4.0159186e+52$ & $1.4375$ & $1.11806\pm0.32$ & $1$ \\
051022A& $0.8061$ & $6.0610610e+53$ & $4.1942078e+52$ & $...$ & $...$ & $0$ \\
051016B& $0.9358$ & $9.4879294e+50$ & $8.7512084e+50$ & $1.3$ & $1.15121\pm0.43$ & $1$ \\
051008A& $2.77$ & $6.2173122e+53$ & $2.3112013e+53$ & $1.8125$ & $1.17115\pm0.16$ & $1$ \\
051006A& $1.059$ & $1.2886256e+52$ & $2.7111250e+51$ & $1.275$ & $1.08182\pm0.29$ & $1$ \\
051001A& $2.4295$ & $4.9351298e+52$ & $2.9732935e+51$ & $1.09589$ & $1.06329\pm0.34$ & $1$ \\
050922C& $2.1992$ & $9.5330479e+52$ & $1.8800215e+53$ & $3.28571$ & $...$ & $1$ \\
050922B& $4.9$ & $2.0372373e+53$ & $4.6347149e+52$ & $1.26923$ & $1.07165\pm0.12$ & $1$ \\
050915A& $2.5275$ & $4.8429145e+52$ & $1.4846271e+52$ & $1.25714$ & $1.07442\pm0.06$ & $1$ \\
050908A& $3.3467$ & $2.3361435e+52$ & $1.0268558e+52$ & $1.125$ & $1.07386\pm0.23$ & $1$ \\
050904A& $6.295$ & $1.2252347e+54$ & $1.0267954e+53$ & $...$ & $...$ & $0$ \\
050826A& $0.296$ & $6.2733891e+50$ & $6.7723918e+49$ & $1.14375$ & $1.0675\pm0.34$ & $1$ \\
050824A& $0.8277$ & $1.7166067e+51$ & $3.2251971e+50$ & $...$ & $...$ & $0$ \\
050822A& $1.434$ & $3.2497875e+52$ & $3.9591747e+51$ & $1.2875$ & $1.10357\pm0.1$ & $1$ \\
050820A& $2.61469$ & $2.5944552e+53$ & $5.9775012e+52$ & $1.325$ & $1.13571\pm0.2$ & $1$ \\
050819A& $2.5042$ & $1.7313442e+52$ & $3.6023011e+51$ & $...$ & $...$ & $0$ \\
050814A& $5.3$ & $1.9833042e+53$ & $3.2482647e+52$ & $...$ & $...$ & $0$ \\
050803A& $4.3$ & $2.6551152e+53$ & $5.4943286e+52$ & $1.33977$ & $1.44367\pm0.38$ & $1$ \\
050802A& $1.7102$ & $4.4119336e+52$ & $1.3759985e+52$ & $1.175$ & $1.08462\pm0.03$ & $1$ \\
050801A& $1.38$ & $3.2305448e+51$ & $2.3465816e+51$ & $1.3875$ & $1.12067\pm0.07$ & $1$ \\
050730A& $3.96855$ & $2.0573220e+53$ & $1.9836602e+52$ & $1.16471$ & $1.08281\pm0.03$ & $1$ \\
050726A& $3.5$ & $4.2523539e+53$ & $1.2573507e+53$ & $1.12821$ & $1.07442\pm0.16$ & $1$ \\
050714B& $2.4383$ & $1.4348087e+52$ & $3.1647603e+51$ & $...$ & $...$ & $0$ \\
050713A& $3.6$ & $3.0904075e+53$ & $1.9809005e+53$ & $1.875$ & $1.1413\pm0.14$ & $1$ \\
050525A& $0.6063$ & $2.8447353e+52$ & $1.9298367e+52$ & $9.375$ & $1.82943\pm0.11$ & $1$ \\
050505A& $4.2748$ & $2.8977052e+53$ & $9.8634148e+52$ & $...$ & $...$ & $0$ \\
050502B& $5.2$ & $5.4990526e+52$ & $7.7618542e+52$ & $1.4359$ & $1.15295\pm0.21$ & $1$ \\
050502A& $3.793$ & $9.1660075e+52$ & $6.3212480e+52$ & $...$ & $...$ & $0$ \\
050416A& $0.6542$ & $1.2166116e+51$ & $9.7680797e+50$ & $1.53846$ & $...$ & $1$ \\
050408A& $1.2356$ & $2.3251283e+52$ & $...$ & $...$ & $...$ & $0$ \\
050401A& $2.8983$ & $4.1953788e+53$ & $2.0761332e+53$ & $1.5125$ & $1.10478\pm0.14$ & $1$ \\
050319A& $3.2425$ & $5.9217276e+52$ & $1.8528160e+52$ & $1.1875$ & $1.12079\pm0.19$ & $1$ \\
050318A& $1.4436$ & $1.2290230e+52$ & $5.6238939e+51$ & $1.5625$ & $1.17188\pm0.16$ & $1$ \\
050315A& $1.9500$ & $6.3428132e+52$ & $6.7557958e+51$ & $1.31641$ & $1.07586\pm0.29$ & $1$ \\
050223A& $0.584$ & $4.3600187e+51$ & $3.1817159e+50$ & $...$ & $...$ & $0$ \\
050219A& $0.211$ & $1.0528378e+51$ & $9.6873980e+49$ & $1.75$ & $1.176\pm0.34$ & $1$ \\
050215B& $2.62$ & $6.9535556e+51$ & $6.3796821e+51$ & $...$ & $...$ & $0$ \\
050128A& $5.5$ & $5.4185840e+53$ & $4.2376943e+53$ & $2.525$ & $1.23314\pm0.16$ & $1$ \\
050126A& $1.29002$ & $1.5942904e+52$ & $2.7268776e+51$ & $...$ & $...$ & $0$ \\
041219A& $0.31$ & $6.8846662e+52$ & $3.7435819e+51$ & $...$ & $...$ & $0$ \\
041006A& $0.716$ & $2.1103570e+52$ & $...$ & $...$ & $...$ & $0$ \\
040924A& $0.858$ & $9.2083233e+51$ & $2.0869299e+52$ & $...$ & $...$ & $0$ \\
040912A& $1.563$ & $8.4731910e+51$ & $...$ & $...$ & $...$ & $0$ \\
031203A& $0.1055$ & $6.8367417e+49$ & $1.7825514e+49$ & $...$ & $...$ & $0$ \\
030528A& $0.782$ & $2.2240206e+52$ & $1.2523546e+51$ & $...$ & $...$ & $0$ \\
030429A& $2.658$ & $1.7037366e+52$ & $7.4713614e+51$ & $...$ & $...$ & $0$ \\
030329A& $0.1685$ & $1.5536881e+52$ & $1.6487712e+51$ & $...$ & $...$ & $0$ \\
030328A& $1.5216$ & $3.5901169e+53$ & $1.4038892e+52$ & $...$ & $...$ & $0$ \\
030323A& $3.3736$ & $4.1435139e+52$ & $3.5389721e+52$ & $...$ & $...$ & $0$ \\
030226A& $1.986$ & $7.4612360e+52$ & $5.7559211e+51$ & $...$ & $...$ & $0$ \\
030115A& $2$ & $3.0132426e+52$ & $1.1088805e+52$ & $...$ & $...$ & $0$ \\
021211A& $1.006$ & $1.3420022e+52$ & $8.6209390e+51$ & $...$ & $...$ & $0$ \\
021004A& $2.3351$ & $4.3277032e+52$ & $6.6812030e+51$ & $...$ & $...$ & $0$ \\
020903A& $0.251$ & $2.0329623e+49$ & $6.3553778e+48$ & $...$ & $...$ & $0$ \\
020819B& $0.41$ & $1.6188284e+52$ & $2.0484405e+51$ & $...$ & $...$ & $0$ \\
020813A& $1.255$ & $1.3410511e+54$ & $7.3620474e+52$ & $...$ & $...$ & $0$ \\
020427A& $...$ & $1.5174889e+52$ & $2.3547242e+51$ & $...$ & $...$ & $0$ \\
020410A& $...$ & $3.1036079e+52$ & $1.6626471e+50$ & $...$ & $...$ & $0$ \\
020405A& $0.6908$ & $1.0712022e+53$ & $1.3777051e+52$ & $...$ & $...$ & $0$ \\
020331A& $...$ & $9.3092035e+52$ & $8.3236722e+51$ & $...$ & $...$ & $0$ \\
020322A& $...$ & $2.3006791e+52$ & $1.8188899e+52$ & $...$ & $...$ & $0$ \\
020305A& $2.8$ & $3.0862328e+53$ & $1.2454754e+53$ & $...$ & $...$ & $0$ \\
020127A& $1.9$ & $3.3595138e+52$ & $1.4276180e+52$ & $...$ & $...$ & $0$ \\
020124A& $3.198$ & $2.0916205e+53$ & $5.3304294e+52$ & $...$ & $...$ & $0$ \\
011211A& $2.14$ & $3.2338819e+52$ & $2.6326195e+51$ & $...$ & $...$ & $0$ \\
011121A& $0.36$ & $6.4222263e+52$ & $5.8553978e+51$ & $...$ & $...$ & $0$ \\
011030A& $3$ & $1.3496552e+53$ & $3.3741380e+51$ & $...$ & $...$ & $0$ \\
010921A& $0.4509$ & $1.5121289e+52$ & $1.7027655e+51$ & $...$ & $...$ & $0$ \\
010222A& $1.47688$ & $1.3583639e+54$ & $3.1280798e+53$ & $...$ & $...$ & $0$ \\
000926A& $2.0379$ & $7.6611917e+51$ & $1.9335268e+52$ & $...$ & $...$ & $0$ \\
000911A& $1.0585$ & $6.5286452e+53$ & $1.1686275e+53$ & $...$ & $...$ & $0$ \\
000418A& $1.1181$ & $1.0927409e+51$ & $1.1572673e+51$ & $...$ & $...$ & $0$ \\
000301C& $2.0404$ & $1.4137054e+53$ & $5.8167660e+51$ & $...$ & $...$ & $0$ \\
000214A& $...$ & $3.0799661e+53$ & $2.6027882e+53$ & $...$ & $...$ & $0$ \\
000210A& $0.846$ & $1.5402148e+53$ & $9.7440087e+52$ & $...$ & $...$ & $0$ \\
000131A& $4.5$ & $1.6091077e+54$ & $4.1427458e+53$ & $...$ & $...$ & $0$ \\
991216A& $1.02$ & $5.9990380e+53$ & $3.3340703e+53$ & $...$ & $...$ & $0$ \\
991208A& $0.7063$ & $2.6608965e+53$ & $4.7256055e+52$ & $...$ & $...$ & $0$ \\
990712A& $0.4331$ & $8.2140242e+51$ & $2.3543036e+51$ & $...$ & $...$ & $0$ \\
990705A& $0.8424$ & $2.4856450e+53$ & $2.2592458e+52$ & $...$ & $...$ & $0$ \\
990510A& $1.619$ & $1.9618455e+53$ & $6.6794953e+52$ & $...$ & $...$ & $0$ \\
990506A& $1.30658$ & $8.6570353e+53$ & $1.0003553e+53$ & $...$ & $...$ & $0$ \\
990308A& $...$ & $6.3224788e+52$ & $5.1426750e+52$ & $...$ & $...$ & $0$ \\
990123A& $1.6004$ & $3.9029937e+54$ & $5.7512954e+53$ & $...$ & $...$ & $0$ \\
981226A& $1.11$ & $5.4992087e+51$ & $7.4021245e+50$ & $...$ & $...$ & $0$ \\
980703A& $0.966$ & $1.3349163e+53$ & $1.1714416e+52$ & $...$ & $...$ & $0$ \\
980613A& $1.0969$ & $5.9439268e+51$ & $1.9942112e+51$ & $...$ & $...$ & $0$ \\
980519A& $...$ & $1.6401123e+53$ & $2.5541425e+53$ & $...$ & $...$ & $0$ \\
980425A& $0.0085$ & $9.4044560e+47$ & $4.7069075e+46$ & $...$ & $...$ & $0$ \\
980329A& $3.5$ & $2.4119407e+54$ & $5.1763959e+53$ & $...$ & $...$ & $0$ \\
980326A& $...$ & $1.7681436e+52$ & $1.7327807e+52$ & $...$ & $...$ & $0$ \\
971214A& $3.42$ & $2.8690117e+53$ & $9.7989789e+52$ & $...$ & $...$ & $0$ \\
970828A& $0.9578$ & $2.9962477e+53$ & $2.4480205e+52$ & $...$ & $...$ & $0$ \\
970508A& $0.835$ & $8.1226675e+51$ & $2.8154068e+51$ & $...$ & $...$ & $0$ \\
970228A& $0.695$ & $2.7519720e+52$ & $1.5689993e+52$ & $...$ & $...$ & $0$ \\
\hline
&SGRB&\\\hline
130603B& $0.356$ & $2.0184818e+51$ & $4.1470627e+52$ & $...$ & $...$ & $0$ \\
101224A& $...$ & $2.3377336e+50$ & $4.6214040e+50$ & $1.18$ & $1.02\pm0.01$ & $1$ \\
101219A& $0.718$ & $4.4889062e+51$ & $5.9981762e+52$ & $1.21$ & $1.04\pm0.02$ & $1$ \\
100816A& $0.8048$ & $7.9292300e+51$ & $9.0248326e+51$ & $1.78$ & $1.25\pm0.13$ & $1$ \\
100625A& $0.452$ & $9.1729595e+50$ & $1.6544728e+51$ & $...$ & $...$ & $1$ \\
100206A& $0.4068$ & $5.8146168e+50$ & $7.8630003e+50$ & $...$ & $...$ & $1$ \\
100117A& $0.92$ & $1.3177021e+51$ & $2.2221897e+51$ & $1.5$ & $1.13\pm0.06$ & $1$ \\
091109B& $...$ & $6.8707691e+51$ & $1.0359006e+52$ & $1.44$ & $1.06\pm0.03$ & $1$ \\
090515A& $...$ & $2.9009521e+49$ & $9.9408221e+50$ & $...$ & $...$ & $1$ \\
090510A& $0.903$ & $2.8315761e+52$ & $5.5685475e+52$ & $1.19$ & $1.03\pm0.01$ & $1$ \\
090426A& $2.609$ & $5.4996454e+51$ & $1.8767983e+52$ & $1.63$ & $1.06\pm0.03$ & $1$ \\
090305A& $...$ & $2.1668124e+51$ & $3.6835811e+51$ & $1.14$ & $1.04\pm0.02$ & $1$ \\
080905A& $0.1218$ & $4.3038781e+49$ & $3.0525878e+49$ & $...$ & $...$ & $1$ \\
080503A& $...$ & $...$ & $...$ & $1.3$ & $1.05\pm0.03$ & $1$ \\
080123A& $0.495$ & $7.4317979e+50$ & $2.0899903e+50$ & $1.1$ & $1.02\pm0.01$ & $0$ \\
071227A& $0.383$ & $1.0437688e+51$ & $3.1577267e+51$ & $...$ & $...$ & $1$ \\
070809A& $0.2187$ & $3.1788889e+49$ & $4.0789369e+49$ & $3$ & $1.38\pm0.19$ & $1$ \\
070724A& $0.457$ & $3.6821432e+49$ & $5.8840648e+49$ & $4.38$ & $1.75\pm0.38$ & $1$ \\
070714B& $0.923$ & $8.3606812e+51$ & $6.1510289e+51$ & $...$ & $...$ & $1$ \\
070707A& $...$ & $6.8773278e+50$ & $1.0315992e+51$ & $...$ & $...$ & $0$ \\
070429B& $0.904$ & $3.9860381e+50$ & $8.5234985e+50$ & $1.18$ & $1.03\pm0.01$ & $1$ \\
061217A& $0.827$ & $2.3431408e+51$ & $1.6880324e+52$ & $1.16$ & $1.04\pm0.02$ & $1$ \\
061210A& $0.41$ & $1.6610068e+51$ & $1.0680942e+51$ & $...$ & $...$ & $1$ \\
061201A& $0.111$ & $1.9644644e+50$ & $1.3062361e+51$ & $1.1$ & $1.03\pm0.01$ & $1$ \\
061006A& $0.4377$ & $2.3249221e+51$ & $1.9942888e+52$ & $1.25$ & $1.09\pm0.04$ & $1$ \\
060801A& $1.131$ & $2.3496415e+52$ & $8.9618292e+52$ & $4.63$ & $1.25\pm0.13$ & $1$ \\
060502B& $0.287$ & $2.1773702e+50$ & $3.5457363e+50$ & $...$ & $...$ & $1$ \\
060313A& $...$ & $1.2770348e+52$ & $9.4428632e+52$ & $1.94$ & $1.94\pm0.16$ & $1$ \\
060121A& $...$ & $3.9109172e+51$ & $2.0426446e+52$ & $1.81$ & $1.09\pm0.04$ & $0$ \\
051227A& $0.8$ & $2.7951385e+51$ & $5.6004036e+50$ & $4.75$ & $1.38\pm0.19$ & $1$ \\
051221A& $0.5465$ & $3.1228093e+51$ & $6.9422979e+52$ & $3.13$ & $1.25\pm0.13$ & $1$ \\
051210A& $1.4$ & $6.2686753e+51$ & $1.4502529e+52$ & $...$ & $...$ & $1$ \\
050724A& $0.258$ & $3.5790924e+50$ & $1.0819476e+50$ & $2.13$ & $1.19\pm0.09$ & $1$ \\
050709A& $0.16$ & $3.5820132e+49$ & $5.2977976e+50$ & $1.23$ & $1.03\pm0.01$ & $0$ \\
050509B& $0.226$ & $6.9883382e+48$ & $2.2031235e+49$ & $1.23$ & $1.04\pm0.02$ & $1$ \\
\enddata
\tablecomments{References.
(1) \citet{2010ApJ...725.1965L};
}
\end{deluxetable}

